Robotic Grasping of Fully-Occluded Objects using RF Perception

We present the design, implementation, and evaluation of RF-Grasp, a robotic system that can grasp fully-occluded objects in unknown and unstructured environments. Unlike prior systems that are constrained by the line-of-sight perception of vision and infrared sensors, RF-Grasp employs RF (Radio Frequency) perception to identify and locate target objects through occlusions, and perform efficient exploration and complex manipulation tasks in non-line-of-sight settings. RF-Grasp relies on an eye-in-hand camera and batteryless RFID tags attached to objects of interest. It introduces two main innovations: (1) an RF-visual servoing controller that uses the RFID's location to selectively explore the environment and plan an efficient trajectory toward an occluded target, and (2) an RF-visual deep reinforcement learning network that can learn and execute efficient, complex policies for decluttering and grasping. We implemented and evaluated an end-to-end physical prototype of RF-Grasp. We demonstrate it improves success rate and efficiency by up to 40-50% over a state-of-the-art baseline. We also demonstrate RF-Grasp in novel tasks such mechanical search of fully-occluded objects behind obstacles, opening up new possibilities for robotic manipulation. Qualitative results (videos) available at rfgrasp.media.mit.edu

==> abstract-3.tex <==
We consider the problem of grasping fully occluded objects in unknown
and unstructured environments. Existing solutions to this problem
either require an expensive process of active exploration to search
for objects or completely fail if the objects are behind occlusions.

We present \name, a system that leverages radio perception to design
efficient exploration controllers and learn complex manipulation
policies in highly cluttered and non-line-of-sight settings.  The
system relies on an eye-in-hand camera and batteryless RFIDs attached
to objects of interest. Since RF (radio frequency) signals can
traverse many everyday occlusions, \name\ uses the RFID signals to
locate an object through occlusions. \name's design introduces two
main components that synergistically combine RF and visual features.
First, it introduces a radio-visual servoing controller that uses the
RFID's location to selectively explore the environment and plan an
efficient trajectory toward an occluded target object. The controller
can efficiently discover obstacles by biasing a gaussian belief space
planner using the RFID's location and can close the control loop by
tracking the RFID's (and thus the object's) movement.  Second, \name\
employs a radio-visual deep reinforcement learning network that can
learn efficient and complex policies for decluttering and grasping.
The network can focus on the region of interest using an RF-based
attention mechanism; it also incorporates a RF-based spatio-temporal
reward function that extends its learning horizon and allows it learn
and execute complex behaviors. 

We implemented \name\ using a UR5e robot, Intel RealSense camera, USRP
software radios, and off-the-shelf RFID tags.  Our real-world
experiments demonstrate that \name\ can reduce time-to-grasp by
XXX$\times$ in line-of-sight scenarios and XXX$\times$ in
non-line-of-sight scenarios against state-of-the-art baselines.


==> abstract-4.tex <==
We consider the problem of grasping fully-occluded objects in unknown and unstructured environments. Existing solutions to this problem require an expensive process of active exploration to search for objects and often fail if objects are under clutter or behind occlusions.

We present RF-Grasp, a system that leverages RF (Radio Frequency) perception to perform efficient exploration and complex manipulation tasks in highly cluttered and non-line-of-sight settings. Unlike visible light and infrared, RF signals can traverse many everyday occlusions, enabling RF-Grasp to identify and locate target objects through occlusions, and to guide its exploration, navigation, and manipulation.

RF-Grasp relies on an eye-in-hand camera and batteryless RFID tags attached to objects of interest. Its design introduces two main innovations: (1) an RF-visual servoing controller that uses the RFID’s location to selectively explore the environment and plan an efficient trajectory toward an occluded target object, and (2) an RF-visual deep reinforcement learning network that can learn and execute efficient, complex policies for decluttering and grasping.

We implemented and evaluated an end-to-end prototype of RF-Grasp using a UR5e robot, Intel RealSense camera, customized RFID micro-location system, and off-the-shelf RFID tags. We demonstrate the system performing novel grasping tasks in highly-challenging scenarios where it was not feasible before, opening up new possibilities for robotic manipulation.


==> conclusion-1.tex <==
\vspace{-0.1in}
\section{Conclusion}
\vspace{-0.08in}
%\fa{Failure modes? Limitations}
\name\ is a system that fuses RF-visual information to enable robotic grasping of fully-occluded objects. %It presents a first step toward RF-visual primitives for novel robotic tasks. 
As the work evolves, it can be extended to grasping at different angles and grippers, novel tasks that use RFIDs for semantic grasping and scene understanding, and more complex manipulation and assembly including human-robot interaction. 
%We hope this work motivates researchers to bridge RF and vision 

\vspace{0.02in}
\noindent
\footnotesize{\textbf{Acknowledgments.} 
We thank the anonymous reviewers and the Signal Kinetics group for their feedback. The research is sponsored by the National Science Foundation, NTT DATA, Toppan, Toppan Forms, and Abdul Latif Jameel Water and Food Systems Lab (J-WAFS).}


==> implementation-1.tex <==
\section{Implementation \& Evaluation}
\subsection{RFID Localization}
\textbf{Hardware.} We implemented the RFID localization system on three USRP N210s \cite{x} with SBX daughterboards \cite{x} all synchronized to the same external clock\cite{x}. One USRP handles in-band RX/TX; one handles out-of-band RX/TX; and the third provides an extra out-of-band RX channel for 2D trilateration. We used three MT-242025 antennas: One transmits in-band and out-of-band TX using a D-2-21-3W-S+ power combiner; one handles in-band and one out-of-band RX through a ZAPD-2-21-3W-S+ power splitter; and one is directly connected to USRP as an out-of-band receiver. All antennas are arranged in a single plane next to each other. The USRPs are connected to a NETGEAR GS110MX network switch, which in turn connected to a PC that runs Ubuntu 18.04 and has XXX.

\textbf{Software.} The system is implemented primarily in Python, using the Python 3 bindings for the USRP’s UHD driver (version 3.15.0.0) to control the radios. Some parts of the system such as decoding, channel estimation, and the Query-ACK turnaround are implemented in C++ for speeding up the system.

\subsection{Robot ?!}
\textbf{Hardware.} Our real-world setup consists of a UR5e robot arm, 2F-85 Robotiq gripper, and an Intel Real-Sense D415 depth camera mounted on the gripper. The RFID localization system is set up on a table in front of the robot arm 16cm below the robot base level. The robot is connected through Ethernet to a PC that runs Ubuntu 16.04 and has an Intel Core i9-9900K processor; RTX 2080 Ti, 11 GB graphic card; and 32 GB RAM. We also used a USB to RS485 interface to control the gripper from the PC.

\textbf{Software.} The robot is controlled using Universal Robots ROS Driver\cite{x} on ROS kinetic\cite{x}. We used Moveit!\cite{x} and OMPL\cite{x} for planning scene and inverse kinematic solver. The TSDF volume is created using Yak \cite{x}. We used Point Cloud Library \cite{x} for extracting clusters and occlusion from TSDF volume. To solve the SQP for trajectory optimization, we used FORCES\cite{x}. The code is implemented in both C++ and Python.

\subsection{Simulation}
The system is simulated with the help of three different environments: 1) VREP\cite{x} to simulate the depth camera visual data, and robot and gripper's physical interactions with objects in the environment. We used Bullet Physics 2.83 as the physics engine. 2) Gazebo\cite{x} for predicting the robot state. This module takes into account gravity, inertia, and crashing into the ground and other obstacles. 3) Rviz is a 3D visualization tool to visualize the robot trajectory, obstacles in the environment, occluded areas, and their mean and co-variances. In the simulated system, we used the VREP remote API to get each object's location to simulate the RFID localization system in the real world. 

\subsection{Baselines}
We implemented four baselines:
\begin{itemize}
    \item \textit{Random Trajectory Sampling:} In this baseline, an initial trajectory toward the average of the centers of occlusions is created. Then, a random vector, drawn from a uniform distribution, is added to the control signal. From a population of 100 samples, the trajectory that minimizes the objective function is chosen for execution. In each iteration, the system plans for the next 4 steps or a maximum of 0.5-meter travel.
    
    \item \textit{Active Exploration using Trajectory
    Optimization\cite{x}:} represents a system for exploring the environment with the goal of minimizing the uncertainties. This system has no knowledge of items position. 
    
    \item \textit{Obstacle Avoidance with RF-guidance:} uses the occlusion frontiers extracted in the initial position to plan the robot's movements toward the item located using RFID. The system perceives the frontiers as walls with which collision must be avoided.
    
    \item \textit{Visual Pushing for Grasping (VPG)\cite{x}:} represents a state-of-the-art system for grasping in clutter. This baseline de-clutters the workspace by pushing the object to make space for the gripper finger to perform grasping.
\end{itemize}

\subsection{Evaluation}
We evaluated \name by executing a series of tests in which the robot must explore the environment to find and grasp an item initially hidden from it. The robot workspace is on top of a table with dimensions of $0.8 \times 0.8 \times XXX$ that is 15cm below the robot's base. We tested the system in three different scenarios with different levels of clutter and occlusion. For each test, we ran the system for n times ($n \in \sim 6-10$) and evaluated the performance by the following metrics: 1) Average Traveled Distance: the distance that the robot's end-effector moves from the initial position until there is a line-of-sight to the item of interest or the system stops exploring without completing the task  2) Task completion rate: the percentage of trials that reach the stopping criteria meaning that there was a line of sight to the item of interest. 3) Grasping efficiency: it is the number of successful grasps of intended objects over the total grasping attempts.

The robot arm is placed in a similar initial position in each run where there are two separated regions of workspace hidden from the wrist-mounted camera. In all three scenarios, there is one item of interest behind one occlusion frontier. In the first scenario, there are two separate sheets occluding two separate regions. In the second scenario, there are three occlusion frontiers, two of which share one occluded area. In the third scenario, there are four occlusion frontiers, three of which share one occluded region.

WE NEED A FIGURE.


==> implementation-2.tex <==
\section{Implementation \& Evaluation}

\fa{If we're short on space, I'm wondering if we can cut this significantly.}

\subsection{RFID Localization}
\textbf{Hardware.} We implemented the RFID localization system on three USRP N210s \cite{usrp} with SBX daughterboards \cite{sbx} all synchronized to the same external clock \cite{clock}. One USRP handles in-band RX/TX; one handles out-of-band RX/TX; and the third provides an extra out-of-band RX channel for 2D trilateration. We used three MT-242025 antennas: One transmits in-band and out-of-band TX using a D-2-21-3W-S+ power combiner; one handles in-band and one out-of-band RX through a ZAPD-2-21-3W-S+ power splitter; and one is directly connected to USRP as an out-of-band receiver. All antennas are arranged in a single plane next to each other. The USRPs are connected to a NETGEAR GS110MX network switch, which in turn connected to a PC that runs Ubuntu 18.04 and has XXX.

\textbf{Software.} The system is implemented primarily in Python, using the Python 3 bindings for the USRP’s UHD driver (version 3.15.0.0) to control the radios. Some parts of the system such as decoding, channel estimation, and the Query-ACK turnaround are implemented in C++ for speeding up the system.

\subsection{Robot ?!}
\textbf{Hardware.} Our real-world setup consists of a UR5e robot arm, 2F-85 Robotiq gripper, and an Intel Real-Sense D415 depth camera mounted on the gripper. The RFID localization system is set up on a table in front of the robot arm 16cm below the robot base level. The robot is connected through Ethernet to a PC that runs Ubuntu 16.04 and has an Intel Core i9-9900K processor; RTX 2080 Ti, 11 GB graphic card; and 32 GB RAM. We also used a USB to RS485 interface to control the gripper from the PC.

\textbf{Software.} The robot is controlled using Universal Robots ROS Driver \cite{URD} on ROS kinetic \cite{ros}. We used Moveit! \cite{moveit} and OMPL \cite{OMPL} for planning scene and inverse kinematic solver. The TSDF volume is created using Yak \cite{yak}. We used Point Cloud Library  \cite{PCL} for extracting clusters and occlusion from TSDF volume. To solve the SQP for trajectory optimization, we used FORCES \cite{forces}. The code is implemented in both C++ and Python.

\subsection{Simulation}
\fa{Are we reporting the simulation results?}

The system is simulated with the help of three different environments: 1) VREP \cite{vrep} to simulate the depth camera visual data, and robot and gripper's physical interactions with objects in the environment. We used Bullet Physics 2.83 as the physics engine. 2) Gazebo \cite{gazebo} for predicting the robot state. This module takes into account gravity, inertia, and crashing into the ground and other obstacles. 3) Rviz  \cite{rviz} is a 3D visualization tool to visualize the robot trajectory, obstacles in the environment, occluded areas, and their mean and co-variances. In the simulated system, we used the VREP remote API to get each object's location to simulate the RFID localization system. 

\subsection{Baseline}

Vision-based semantic grasping systems requires large datasets of items images and an extensive training process. As a result, implementing the state of the art semantic grasping systems for a baseline is beyond the scope of this paper. We implemented a simpler baseline with a similar performance of a vision-based semantic grasping system for our evaluation. The baseline looks for and tries grasping the green item in a workspace with non-green objects.

\textit{Active Exploration using Trajectory
    Optimization\cite{BerkeleyGraspOcclusion} + color-based attention:} 
  
Similar to our system, the baseline extracts the occluded regions from the TSDF volume and models them with 3D Gaussian distributions. The robot arm explores the environment with the goal of minimizing the covariances that represent the uncertainties. In each iteration of exploration, the system plans for the next 4 steps or a maximum of 0.5-meter travel.
This system has no knowledge of items position. It stops exploration as a green item is seen by the wrist-mounted camera, estimates the location of the item, and tries grasping the item of interest by focusing the attention of the grasping network on the green item.


\subsection{Evaluation}

\fa{Clean up}

We evaluated \name\ by executing a series of tests in which the robot must explore the environment to find and grasp an item initially hidden from it. The robot workspace is on top of a table with dimensions of $0.8 \times 0.8 \times XXX$ that is 15cm below the robot's base. We evaluated the performance of the system by the following metrics: 1) Average Traveled Distance: the distance that the robot's end-effector moves from the initial position until the item of interest is grasped. 2) Task completion rate: the percentage of trials that resulted in successful grasp of tagged items (or green item for baseline) before 10 grasping attempt and 5 meter of traveled distance in exploration phase. 
%3) Grasping efficiency: it is the number of successful grasps of intended objects over the total grasping attempts.

We first evaluate our system qualitatively in challenging scenarios where there is no baseline capable of completing the task. First, in a cluttered scenario, we randomly placed more than 20 blocks along with tagged item in the workspace and covered them with \textcolor{blue}{paper cover}. Because of the cover, there is no line of sight to the item from wrist-mounted camera or antennas to the item. Secondly, we tested \name\ in a cluttered singlr obstacle scenario, where there is an obstacle in the workspace that occludes an area from the wrist-camera. The item of interest along with 5 random block are placed in the initially occluded region. These items are also covered by \textcolor{blue}{paper cover}, and there is no line of sight to the item. Lastly, we tested \name\ in a cluttered multi-obstacle scenario, where there are two boxes which occluded two regions from camera, and we put the tagged item in one of the boxes. We also put 5 more items in each box and covered them with \textcolor{blue}{paper cover}. Similarly, there is no line of sight to object from wrist-mounted camera or antennas to objects.


We evaluated the baseline and our system quantitatively in 6  more scenarios with 0-5 occlusions and 1-15 objects. The robot arm is placed in a similar initial position in each trials. In five of theses scenarios, there are 1-5 separated regions of workspace hidden from the wrist-mounted camera, and the item of interest is not in line of sight of the camera in these 5 scenarios. In the scenario with no occlusion, there is no need for exploration since there is no occlusion in the work space as the item of interest is in the line-of-sight of the wrist mounted camera. 
% \begin{table}[h]
%     \begin{center}
%     \begin{tabular}{ |c|c |c | } 
%      \hline
%       Scenario & \# occlusions & \#  objects\\ [2ex]
%      \hline
%      A &  1  &   1 \\[1ex]
%      B &  2  &   5 \\[1ex]
%      C &  3  &   10 \\[1ex]
%      D &  4  &   13 \\[1ex]
%      E &  5  &   15 \\[1ex]
%      O &  0  &   5 \\[1ex]
%      \hline
%     \end{tabular}
%     \end{center}
%     \label{tab:tab1}
%     \caption{\textbf{Summary of Scenarios.} The table shows number of graspable toy blocks and occluded regions in scenarios that we quantitatively compared \name\ to the baseline.}
% \end{table}


==> implementation-3.tex <==
\section{Implementation \& Evaluation}

%\fa{If we're short on space, I'm wondering if we can cut this significantly.}

\subsection{Physical Prototype.}
Our physical setup consists of a UR5e robot arm, 2F-85 Robotiq gripper, and an Intel Real-Sense D415 depth camera mounted on the gripper. The RF perception module is implemented as an RFID localization system on software radios (we refer the reader to~\cite{TurboTrack} for implementation details). The RFID localization system is set up on a table in front of the robot arm 16cm below the robot base level. The robot is connected through Ethernet to a PC that runs Ubuntu 16.04 and has an Intel Core i9-9900K processor; RTX 2080 Ti, 11 GB graphic card; and 32 GB RAM. We also used a USB to RS485 interface to control the gripper from the PC.

The robot is controlled using Universal Robots ROS Driver~\cite{URD} on ROS kinetic~\cite{ros}. We used Moveit!~\cite{moveit} and OMPL~\cite{OMPL} for planning scene and inverse kinematic solver. The TSDF volume is created using Yak~\cite{yak}. We used Point Cloud Library~\cite{PCL} for extracting clusters and occlusion from TSDF volume. To solve the SQP for trajectory optimization, we used FORCES~\cite{forces}. The code is implemented in both C++ and Python.

Objects of interest are tagged with off-the-shelf RFIDs such as the Alien tag~\cite{Alien}. The system continuously identifies the tags in the environment, tracks their location, and feeds their location, as well as the RGB-D input to the perception modules as shown in Fig.~\ref{fig:overview}. The system also performs coordinate transformation between the RFID localization system's fixed-mount frame and the eye-in-hand camera frame of reference by using the robot's pose.

\subsection{Simulation}
We also built a full simulation for our system, for training and development purposes. The simulation is implemented using a combination of three environments: 1) VREP~\cite{vrep} to simulate the depth camera visual data, and robot and gripper's physical interactions with objects in the environment. We used Bullet Physics 2.83 as the physics engine. 2) Gazebo~\cite{gazebo} for predicting the robot state. This module takes into account gravity, inertia, and crashing into the ground and other obstacles. 3) Rviz ~\cite{rviz} is a 3D visualization tool to visualize the robot trajectory, obstacles in the environment, occluded areas, and their mean and co-variances. In the simulated system, we used the VREP remote API to get each object's location to simulate the RFID localization system. Note that only VREP is used to train the deep-reinforcement learning network, while Gazebo, Rviz, \textcolor{red}{and VREP} were used to develop and visualize the different steps of RF-Visual servoing.

\subsection{Baseline}
Since prior work does not deal with the generalized mechanical search problem where the target objects are both behind an occlusion \texit{and} dense clutter, we built a baseline by combining two state-of-the-art past systems. The first component of the baseline performs efficient active exploration and trajectory optimization using Gaussian Belief Space Planning~\cite{BerkeleyGraspOcclusion}. The system uses a similar objective function as Eq.~\ref{eq:obj1}, but without the RF-biasing and guidance. It also performs similar steps (TSDF, frontier extraction, etc) to efficiently explore the environment, but unlike \name, it does not have a mechanism to obtain the target object's location. The second component is a color-based attention mechanism~\cite{graspinvisible} which estimates the location of the item using a unique color,\footnote{Without loss of generalizity, the baseline looks for and tries grasping the green item in a workspace with non-green objects.} and tries grasping the item of interest by focusing the attention of the grasping network on the colored item of interest. For fairness to the baseline, we only compare it to our system in scenarios where the object is only partially (or not) occluded, but not in scenarios where it is fully occluded. \textcolor{red}{\sout{The baseline has an exploration termination criterion similar to Eq.~\ref{eq:criterion}.} The baseline stops as it detects more than 100 green pixels in its field of view.}

% In each iteration of exploration, the system plans for the next 4 steps or a maximum of 0.5-meter travel.
%This system has no knowledge of items position. It stops exploration as a green item is seen by the wrist-mounted camera, estimates the location of the item, and tries grasping the item of interest by focusing the attention of the grasping network on the green item.


\subsection{Evaluation Metrics}

We evaluated \name\ through a series of tests in which the robot must explore the environment to find and grasp an item initially hidden from it. The robot workspace is on top of a table with dimensions of 0.8m$\times$1.2m that is 15cm below the robot's base. We evaluated the performance of the system by the following metrics: 1) Average Traveled Distance: the distance that the robot's end-effector moves from the initial position until the item of interest is grasped. 2) Task completion rate: the percentage of trials that resulted in successful grasp of tagged items (or green item for baseline) before 10 grasping attempt and 5 meter of traveled distance in exploration phase. 
%3) Grasping efficiency: it is the number of successful grasps of intended objects over the total grasping attempts.


% \begin{table}[h]
%     \begin{center}
%     \begin{tabular}{ |c|c |c | } 
%      \hline
%       Scenario & \# occlusions & \#  objects\\ [2ex]
%      \hline
%      A &  1  &   1 \\[1ex]
%      B &  2  &   5 \\[1ex]
%      C &  3  &   10 \\[1ex]
%      D &  4  &   13 \\[1ex]
%      E &  5  &   15 \\[1ex]
%      O &  0  &   5 \\[1ex]
%      \hline
%     \end{tabular}
%     \end{center}
%     \label{tab:tab1}
%     \caption{\textbf{Summary of Scenarios.} The table shows number of graspable toy blocks and occluded regions in scenarios that we quantitatively compared \name\ to the baseline.}
% \end{table}


==> intro-3.tex <==
\section{Introduction} 

Recent years have witnessed a surge in robotic grasping and
manipulation systems~\cite{XXX,XXX,XXX}. Multiple advances have been
made in both accuracy and robustness~\cite{XXX,XXX}. State-of-the-art
robotic grasping systems can achieve over 80-90\% success rate even in
cluttered environments~\cite{MVPclutter,PushGrasp}. Yet, today’s
systems require objects to be visible to their cameras to attain such
high success rates. If an object of interest is fully occluded, these
systems cannot perceive it and either completely fail~\cite{XXX} or
resort to an expensive process of active
exploration~\cite{BerkeleyGraspOcclusion,XXX}.

In this paper, we ask whether we can extend efficient robotic grasping
to visually occluded environments. Our idea is to augment robotic
systems with radio perception. Unlike visible light and infrared,
radio frequency (RF) signals can traverse many everyday occlusions
like cardboard boxes, wooden dividers, opaque plastic covers, and
colored glass. Thus, augmenting robotic systems with radio perception
would enable them to perceive visually-occluded objects and plan
efficient grasping and manipulation tasks in non-line-of-sight
settings. 

Transforming this idea into a practical system faces multiple
challenges.
Unlike cameras, radio sensors cannot produce high-resolution images
with pixel-wise precision~\cite{RFCapture}. Moreover, existing
learning models for robotic grasping and exploration are mostly based
on vision and are not designed to incorporate RF features. This
problem is exacerbated by the fact that RF signals reflect off
different objects in the environment before arriving at the receiver
leading to a common problem called the multipath effect, which makes
it difficult to associate an RF signal with a specific location.

We present \name\ (Radio-Visual Grasping), a robotic system that
combines radio and vision perception to efficiently grasp objects in
both line-of-sight and non-line-of-sight settings. \name\ relies on an
eye-in-hand camera and on passive RFID (Radio Frequency
IDentification) tags placed on objects of interest as shown in
Fig.~\ref{fig:intro-fig}. Passive RFIDs are
batteryless tags (3-5 cents each) which have been widely adopted by
many industries as replacements to barcodes. RFIDs harvest energy from
existing radio signals to power up and transmit
their identifiers, enabling a radio-equipped robot to uniquely
identify them from a distance and through occlusions. \name\ uses the
RFID’s signal in order to sense and identify the tagged item, even if
it is fully occluded, and subsequently guide the eye-in-hand camera’s
active exploration around occlusions. 
%
Architecturally, \name\ consists of two main components:

\vspace{0.05in}
\noindent
\textbf{(a) Radio-Visual Servoing:} % Controller:}
% RF-Guided Active Exploration and Trajectory Planning:} 
The first component of \name's design is a radio-visual controller
that enables it to localize the object of interest through occlusions
and plan an efficient trajectory for grasping. To locate the target
object, \name\ queries the associated RFID and uses the RFID's
response to compute the time-of-flight from multiple antennas and
perform trilateration. But obtaining the RFID's location is not enough
to guide the robot toward grasping since the object of interest may be
occluded by dividers that are transparent to RF signals. Thus, the
robot needs to reduce uncertainty about the layout of obstacles in the
environment and identify viable paths for grasping the target object.


\begin{figure*}[t]
	\centering
	\begin{tabular}{ccc}
%	\begin{minipage}{.63\columnwidth}
%		\centering
		\epsfig{file=image1_e.jpeg,width=0.31\textwidth, height= 0.19\textwidth}
		&
		\epsfig{file=image2_e.jpeg,width=0.31\textwidth, height= 0.19\textwidth}
		&
		\epsfig{file=image3_e.jpeg,width=0.31\textwidth, height= 0.19\textwidth}\\
		
		\footnotesize{(a) Object of interest is occluded}
		&
		\footnotesize{(b) Radio-Visual Servoing}
		&
		\footnotesize{(c) Grasping item of interest}\vspace{+0.2cm} \\ 
		
		\epsfig{file=fig_1_Color.png ,width=0.155\textwidth, height= 0.09\textwidth}\hspace{0.5mm}\epsfig{file=fig_1_depth.png ,width=0.155\textwidth, height= 0.09\textwidth}
		&
		\epsfig{file=fig_2_Color.png ,width=0.155\textwidth, height= 0.09\textwidth}\hspace{0.5mm}\epsfig{file=fig_2_depth.png ,width=0.155\textwidth, height= 0.09\textwidth}
		&
		\epsfig{file=fig_3_Color.png ,width=0.155\textwidth, height= 0.09\textwidth}\hspace{0.5mm}\epsfig{file=fig_3_depth.png ,width=0.155\textwidth, height= 0.09\textwidth}\\
		\footnotesize{(d) Camera Field-of-view (FOV) in RGB and depth}
		&
		\footnotesize{(e) Camera FOV during planning} 
		&
		\footnotesize{(f) Camera FOV after grasping RFID-tagged object} \vspace{0.1cm}		
\end{tabular}
\caption{\name\ uses Radio-Visual Servoing and Learning to Grasp Occluded Objects}
\label{fig:intro-fig}
\end{figure*}



To deal with this uncertainty, \name\ leverages an eye-in-hand camera
to perform selective active exploration. It builds on prior work in
gaussian belief planning~\cite{BerkeleyGraspOcclusion,XXX}, and
extends it by  biasing the belief space and constraining the
optimization problem using the RFID-computed position. Specifically,
\name\ encodes unknown (occluded) regions as a mixture of Gaussians,
and applies higher weights to gaussians near the RFID's location thus
encouraging the exploration of those regions. This can be formulated
as an optimization problem, which \name\ further constrains by
imposing penalties on trajectories that deviate from the direct
line-of-sight path from the gripper’s current position to that of the
RFID. This enables \name\ to perform selective exploration of the
belief space and plan an optimal trajectory toward the object of
interest as we describe in detail in~\xref{sec:servoing}.

\vspace{0.05in}
\noindent
\textbf{(b) Radio-Visual Learning of Manipulation Policies:}
%\textbf{(b) Radio-Visual Deep Reinforcement Learning:}
%\textbf{(b) RF-based Attention for Decluttering and Grasping:} 
While RF-guided trajectory planning enables the robot to intelligently
explore and servo the robotic arm toward the object of interest, the
robot still needs a grasping policy once the object of interest is
within reach. Designing such policies is known to be challenging in
highly cluttered environments~\cite{PushGrasp,XXX}. An object of
interest may still be buried under a pile or stacked close to other
objects, to the extent that it may be infeasible to grasp it without
actively manipulating the environment. State-of-the-art systems deal
with this challenge by learning policies that aim to grasp
\textit{all} objects in the environment and do not have mechanisms for
focusing on the target~\cite{PushGrasp}. This makes them inefficient
in scenarios where the robot needs to grasp a specific object or a
subset of objects in the environment.

To learn efficient and targeted grasping policies, \name\ encodes the
RFID’s location (obtained earlier) as an
attention mechanism in the reinforcement learning problem. Such
attention mechanism allows the robot to focus on the area of interest,
thus reducing the time-to-pick up the target object. The attention
mechanism is implemented as a convolutional layer that folds in the
probability distribution corresponding to the RFID’s location.
Attention mechanisms, however, run the risk of over-emphasizing the
region of interest while discouraging policies that may achieve higher
efficiency by performing actions further away from the attention
domain~\cite{XXX}. For example,
it may be necessary to push further away objects in order to make room
for grasping the target object. In order to balance
attention with effectiveness, \name\ employs a spatio-temporal reward
function. Specifically, rather than offering no rewards to successful
actions executed further away from the attention domain, this function
discounts rewards by their spatial and temporal distance to the attention
region. As a result, \name's approach extends the learning horizon
beyond a single time step or the immediate vicinity of the
object of interest.  In~\xref{sec:learning}, we show how this mechanism
can teach robots to learn attention-based synergies between pushing
and grasping for removing clutter and picking up the
object of interest.

We implemented our design using a UR5e robotic arm, USRP software
radios (for RF localization), and an Intel RealSense XXX camera. (more
implementation details) Our experimental results show that \name\ can
reduce pick-up time of an object of interest by as much as XXX in
line-of-sight and by XXX in non-line-of-sight scenarios due to
reducing the active exploration and the attention mechanism.
Qualitative results (videos) are available at: XXX




\vspace{0.05in}
\noindent
\textbf{Contributions:} \name\ is the first system that bridges RF and
vision perception to enable robot object manipulation in fully
occluded environments.  The design introduces multiple innovations
including radio-visual servoing, RF-biased gaussian belief space
planning, and radio-visual deep reinforcement learning of manipulation
policies.
 % can grasp fully-occluded RFID-tagged objects using radio-visual
%servoing and learning.  
%The design multiple innovations including an RF-biased
%guassian belief space planning controller and a radio-visual deep
%reinforcement learning network of manipulation policies that
%incorporates RF-based attention spatio-temporal reward function. 
The paper also presents a prototype implementation and evaluation of
the system demonstrating its efficiency and its ability to perform
previously-infeasible tasks such directly grasping up target object
from under a pile.

In comparison to vision-only systems, \name's design has the drawback
of requiring the target object(s) to be tagged with RFIDs. Despite
this limitation, we argue that the system can enable many applications
given the widespread adoption of RFIDs (tens of billions of manufactured
objects are annually tagged with RFIDs~\cite{XXX} and entire countries
like Japan have announced that all future manufactured items must be
tagged with RFIDs~\cite{XXX}). More fundamentally, we hope that this
work will motivate further research on bridging RF and vision to
enable efficient and complex robotic tasks.

% should we argue bridging as a contribution?


==> intro-6.tex <==
\section{Introduction} 

Object grasping and manipulation are fundamental robotic problems that
have seen significant advances over the past few
years~\cite{XXX,XXX,XXX}. State-of-the-art robotic grasping systems
can achieve high success rates even in cluttered
environments~\cite{MVPclutter,PushGrasp}. Recently, the problem of
semantic grasping has received mounting interest from academia and
industry~\cite{semantic1,semantic2}. Rather than grasping
\textit{any} object, semantic grasping requires a robot to grasp a
\textit{specific} object or one belonging to a certain (semantic)
class.  Such targeted grasping is an important enabler for various
high-level complex tasks such as sorting, packaging, and assembly.

In this paper, we ask the following question: Can we enable semantic
grasping of invisible objects? This problem arises frequently in
unstructured environments. For example, a robot may need to fetch a
target item hidden behind clutter, inside containers, or on high
shelves. Alternatively, it may need to collect a certain class of
objects from within a pile and declare task completion once all such
objects have been collected. However, if the target object is
invisible to the camera, the robot cannot recognize and grasp it. As a
result, semantic grasping remains infeasible today  in fully-occluded
environments.

% This
%problem is common in unstructured environments at homes, warehouses,
%or factories. 

We present \name,\footnote{\name\ stands for Radio and Visual
Learning.} a system that enables robotic grasping of invisible
objects, as shown in Fig.~\ref{fig:intro-fig}. The system can learn,
plan, and execute, efficient grasping policies in line-of-sight,
non-line-of-sight, and highly cluttered environments.  At the heart of
\name's design is a radio perception module that can identify and
locate objects through occlusions. Unlike visible light, radio signals
can traverse many everyday occlusions including cardboard boxes,
wooden dividers, opaque plastic covers, and colored glass. By placing
batteryless radio stickers (RFIDs)\footnote{RFIDs (Radio Frequency
Identifiers) are passive 3-5 cent tags which have been adopted by many
industries as replacement to barcodes as they enable reading and
uniquely identifying objects from a distance. Please refer to
section~\ref{sec:related} for a background on RFIDs.} on objects of
interest, \name\ can perceive them through occlusions and plan
efficient grasping and manipulation tasks.

% grasp planner
% uniquely identify

Designing a robotic system that leverages RFIDs for grasping is
challenging for many reasons. First, unlike cameras, a radio
perception module cannot produce high-resolution images with
pixel-wise precision~\cite{RFCapture}; this makes it difficult to
determine grasping affordances. Second, existing learning models for
robotic grasping and exploration are primarily based on vision and are
not designed to incorporate RF features. Moreover, the fact that
occlusions are transparent to radio signals enables \name\ to locate
an RFID through occlusions but also prevents it from recognizing these
occlusions as obstacles and identifying viable paths around them to
grasp the object of interest.

% RFIDs harvest energy from
%existing radio signals to power up and transmit
%their identifiers, enabling a radio-equipped robot to uniquely
%identify them from a distance and through occlusions. \name\ uses the
%RFID’s signal in order to sense and identify the tagged item, even if
%it is fully occluded, and subsequently guide the eye-in-hand camera’s
%active exploration around occlusions. 
%
%Architecturally, \name\ consists of two main components:

To overcome these challenges, \name\ introduces two key primitives
that fuse information from its radio perception module and an
eye-in-hand camera:
% via two key primitives:

\begin{figure*}[h!]
	\centering
	\begin{tabular}{cccc}
%	\begin{minipage}{.63\columnwidth}
%		\centering
		\epsfig{file=res_3p_1.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_2.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_3.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_4.jpeg,width=0.23\textwidth}
		\\
		
		\footnotesize{(a) Localization through obstacles}
		&
		\footnotesize{(b) RF-Guided Exploration }
		&
		\footnotesize{(c) RF-Guided Exploration}  
		& 
		\footnotesize{(d) Decluttering}
		\\ [1ex] 
		
		\epsfig{file=res_3p_5.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_6.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_7.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_8.jpeg,width=0.23\textwidth}
		\\
		
		\footnotesize{(e) Decluttering}
		&
		\footnotesize{(f) Grasping attempt,}
		&
		\footnotesize{(g) Grasping again after }
		&
	    \footnotesize{(h) Grasp success confirmation}
		\\
		&
		\footnotesize{box slipped in the process}
		&
		\footnotesize{updating RFID location }
		&
	    \footnotesize{by RFID location change}
		\\
\end{tabular}
\caption {\textbf{Multi-Obstacle \& Clutter Scenario. } a) In the initial state, an RFID tagged item is occluded under clutter inside one of the boxes. There is no line-of-sight to the item from camera or antennas. b) The robot explores the environment using RF-guided exploration. c) \name\ performs another iteration of exploration, and the stopping criteria is met. As a result, \name moves to grasping phase d) The robot grasps an item. However, since the RFID location doesn't change, it concludes that the recently grasped item is a clutter. e) The robot removes more clutter.  
f) Robot tries grasping the tagged item. However, it misses the item as the box slippes in the process and changes the item location. e) \name\ updates the tagged item location, and tries grasping again. g) The robot confirms that it grasped the item of interest because the RFID location changes with accordingly.}
\label{fig:intro-fig}
\end{figure*}

\vspace{0.05in}
\noindent
\textbf{(a) Radio-Visual Servoing:} % Controller:}
% RF-Guided Active Exploration and Trajectory Planning:} 
\name's first key primitive is a radio-visual controller that enables
it to localize the objects of interest through occlusions and plan an
efficient trajectory for grasping. To locate the target objects,
\name\ sends a radio query and obtains responses from RFIDs on all the
objects belonging to the semantic class. For simplicity, let us focus
on a single object and its corresponding RFID. \name\ uses the RFID's
radio signal to trilaterate the object's position. Once the position
has been identified, \name\ uses the eye-in-hand camera to servo the
robotic arm towards it. 

A key difficulty in this process is that the environment is not known
a priori and the direct path may be occluded by obstacles. Thus,
\name\ needs to actively explore the environment as it tries to
determine an optimal path around obstacles and toward the target
object. To perform efficient active exploration, \name\ encodes
unknown regions using a mixture of Gaussian and biases its belief
space by applying weights derived from the computed RFID position.
In~\xref{sec:servoing}, we explain this process in detail and describe
how this formulation allows \name\ to adapt recent advances in
Gaussian Belief Planning to the radio-visual servoing problem.




% \begin{figure*}[t]
% 	\centering
% 	\begin{tabular}{ccc}
% %	\begin{minipage}{.63\columnwidth}
% %		\centering
% 		\epsfig{file=image1_e.jpeg,width=0.31\textwidth, height= 0.19\textwidth}
% 		&
% 		\epsfig{file=image2_e.jpeg,width=0.31\textwidth, height= 0.19\textwidth}
% 		&
% 		\epsfig{file=image3_e.jpeg,width=0.31\textwidth, height= 0.19\textwidth}\\
		
% 		\footnotesize{(a) Object of interest is occluded}
% 		&
% 		\footnotesize{(b) Radio-Visual Servoing}
% 		&
% 		\footnotesize{(c) Grasping item of interest}\vspace{+0.2cm} \\ 
		
% 		\epsfig{file=fig_1_Color.png ,width=0.155\textwidth, height= 0.09\textwidth}\hspace{0.5mm}\epsfig{file=fig_1_depth.png ,width=0.155\textwidth, height= 0.09\textwidth}
% 		&
% 		\epsfig{file=fig_2_Color.png ,width=0.155\textwidth, height= 0.09\textwidth}\hspace{0.5mm}\epsfig{file=fig_2_depth.png ,width=0.155\textwidth, height= 0.09\textwidth}
% 		&
% 		\epsfig{file=fig_3_Color.png ,width=0.155\textwidth, height= 0.09\textwidth}\hspace{0.5mm}\epsfig{file=fig_3_depth.png ,width=0.155\textwidth, height= 0.09\textwidth}\\
% 		\footnotesize{(d) Camera Field-of-view (FOV) in RGB and depth}
% 		&
% 		\footnotesize{(e) Camera FOV during planning} 
% 		&
% 		\footnotesize{(f) Camera FOV after grasping RFID-tagged object} \vspace{0.1cm}		
% \end{tabular}
% \caption{\name\ uses Radio-Visual Servoing and Learning to Grasp Occluded Objects}
% \label{fig:intro-fig}
% \end{figure*}


\vspace{0.05in}
\noindent
%\textbf{(b) Radio-Visual Learning of Manipulation Policies:}
%\textbf{(b) Radio-Visual Deep Reinforcement Learning:}
\textbf{(b) RF-based Attention for Decluttering and Grasping:} The
above primitive enables the robot to intelligently explore the
environment and servo the robotic arm closer to the object of
interest. Once the object is within reach, \name\ still needs to grasp
it.  Designing grasping policies is known to be challenging
in highly cluttered environments~\cite{PushGrasp,XXX}, especially if
the target object is buried under a pile or stacked close
to other objects. In some scenarios, it may be infeasible to grasp the
object without actively manipulating the environment.

To learn efficient and targeted grasping policies, \name\ encodes the
RFID’s location (obtained earlier) as an attention mechanism in a
reinforcement learning problem. The attention mechanism allows the
robot to focus on the area of interest (near the RFID) and manipulate
the environment around it to facilitate grasping. For example, the
robot may still need to declutter the environment by pushing away
nearby objects to make room for grasping the object of interest.  In
section~\ref{sec:learning}, we describe this primitive in detail and
explain how \name\ trains the reinforcement learning problem by
designing a spatio-temporal reward function centered around the RFID's
position.

We implemented our design using a UR5e robotic arm~\cite{XXX} equipped
with an Intel RealSense~\cite{XXX} eye-in-hand camera. \name's radio
perception module is implemented on USRP X310 software radios by
adapting recent advances in fine-grained RFID positioning, and the
objects of interest are tagged with off-the-shelf RFID
stickers~\cite{Alien}. \name's gaussian belief space planner is
implemented using KinectFusion~\cite{XXX} and TCL~\cite{XXX}. The RF
attention-based reinforcement learning component is trained in
simulation by seeding it with synthetic positioning information from
the radio perception module.

Our empirical evaluation of \name\ demonstrates that it can
semantically grasp invisible objects, a task that was previously
impossible. We implemented a baseline by combining two
state-of-the-art systems for active
exploration~\cite{BerkeleyGraspOcclusion} and grasp affordance
planning~\cite{PushGrasp}. In comparison to this baseline, \name\ can
reduce the pick up time for an object of interest by as much as XXX in
line-of-sight and by XXX in non-line-of-sight scenarios.  Qualitative
results (videos) are available at: XXX


\vspace{0.05in}
\noindent
\textbf{Contributions:} \name\ is the first system that bridges RF and
vision perception to enable robotic grasping of invisible
objects. The design introduces two key primitives -- radio-visual
servoing and RF-based attention for decluttering and grasping -- that
together enable it to learn, plan, and execute efficient grasping
policies.  The paper also presents a prototype implementation and
evaluation of the system demonstrating its efficiency and its ability
to perform previously-infeasible tasks such directly grasping up
target object from under a pile.

In comparison to vision-only systems, \name's design has the drawback
of requiring the target object(s) to be tagged with RFIDs. Despite
this limitation, we argue that the system can enable many applications
given the widespread adoption of RFIDs.
% (tens of billions of manufactured
%objects are annually tagged with RFIDs~\cite{XXX} and entire countries
%like Japan have announced that all future manufactured items must be
%tagged with RFIDs~\cite{XXX}). 
More fundamentally, we hope that this work will motivate further
research on bridging RF and vision to enable efficient and complex
robotic tasks.



==> intro-7.tex <==
\section{Introduction}




\begin{figure}[h!]
	\centering
	\begin{tabular}{c}
		\epsfig{file=intro.jpeg,width=0.45\textwidth}
		\\
		\footnotesize{(a) Target object is fully-occluded in an unstructured environment.}
		\\
		%\epsfig{file=intro_2.jpeg,width=0.4\textwidth}
		%\\
		%\footnotesize{(b) }
		%\\
		\epsfig{file=intro_1.jpeg,width=0.45\textwidth}
		\\
		\footnotesize{(b) \name\ is successful in grasping the target object.}
		\\
\end{tabular}
\caption {\textbf{RF-Grasp can grasp fully-occluded objects.} (a) Even though the camera and RF sensor have no line-of-sight to the object, \name\ uses RF perception to identify and locate the target object through occlusions. (b) It employs \textiti{RF-visual servoing} and \textit{RF-visual manipulation} to efficiently maneuver toward the object, declutter its  vicinity, grasp it, and pick it up.}
\label{fig:intro-fig}
\end{figure}







Object grasping and manipulation are fundamental robotic problems that
have seen significant advances over the past few
years. State-of-the-art robotic grasping systems
can achieve high success rates even in cluttered
environments~\cite{MVPclutter,PushGrasp}. Recently, the problem of
semantic grasping has received mounting interest from academia and
industry~\cite{semantic1,ICRA2019search}. Rather than grasping
\textit{any} object, semantic grasping requires a robot to grasp a
\textit{specific} object or one belonging to a certain (semantic)
class.  Such targeted grasping is an important enabler for various
high-level complex tasks such as retrieving a specific tool or target object, or selectively sorting objects (from a semantic class) into a bin.
%sorting (all objects, packaging, and assembly

In this paper, we ask the following question: \textit{Can we enable semantic
grasping of fully-occluded objects?} This problem arises frequently in
unstructured environments such as warehouses and home environments. For example, a robot may need to fetch a
target item or a tool hidden behind clutter, inside containers, or on high
shelves. Alternatively, it may need to collect a certain class of
objects from within a pile and declare task completion once all such
objects have been collected. However, if the target object is
invisible to the camera, the robot cannot recognize, locate, and/or grasp it. This is why today's approaches for dealing with such a problem either require  partial view to the object of interest or must peform an expensive process of active exploration and manipulation of the environment to search for the target object(s)~\cite{ICRA2019search,BerkeleyGraspOcclusion}. 
%As a
%result, efficient semantic grasping remains largely infeasible today in %fully-occluded environments. 

We present \name,\footnote{\name\ stands for RF-guided gasping.} a system that enables robotic grasping of fully-occluded
objects, as shown in Fig.~\ref{fig:intro-fig}. The system can learn,
plan, and execute, efficient grasping policies in line-of-sight,
non-line-of-sight, and highly cluttered environments.  At the heart of
\name's design is a RF (radio frequency) perception module that can identify and
locate objects through occlusions. Unlike visible light, RF signals
can traverse many everyday occlusions including cardboard boxes,
wooden dividers (and walls), opaque plastic covers, and colored glass. This ``see-through'' capability enables \name\ to identify and locate objects even when they are fully-occluded from its vision sensor.

\name\ relies on wireless and batteryless stickers, called RFIDs (Radio Frequency IDentifiers). RFIDs are passive 3-cent tags which have been widely adopted by many industries as barcode replacements~\cite{RFIDmarket}. A wireless device called a reader can read and uniquely identify RFIDs from up to 9~m and through occlusions, and existing RFID readers can read thousands of tags per second~\cite{Imping}. Moreover, recent advances in RFID systems have enabled locating these passive tags with centimeter-scale precision, through occlusions and in highly-cluttered environments~\cite{TurboTrack,RFind}. 

\name\ is also capable of learning novel manipulation tasks and reasoning methods. One such example involves scenarios where the RFID-tagged target object is hidden under clutter. Knowing where the object of interest is, \name\ can focus on decluttering in its near vicinity until the object is becomes (partially) visible for grasping. Moreover, on the reasoning front, \name\ is able to close the loop on task completion. This is because the RF perception module is capable of identifying and locating all RFID-tagged objects of interest; thus, it can know when the object of interest is picked up (by tracking the RFID's trajectory) as well as when all RFID-tagged objects from a semantic class have been sorted to the correct bin.

\begin{figure*}[h!]
	\centering
	\begin{tabular}{cccc}
%	\begin{minipage}{.63\columnwidth}
%		\centering
		\epsfig{file=res_3p_1.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_2.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_3.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_4.jpeg,width=0.23\textwidth}
		\\
		
		\footnotesize{(a) Localization through obstacles}
		&
		\footnotesize{(b) RF-Guided Exploration }
		&
		\footnotesize{(c) RF-Guided Exploration}  
		& 
		\footnotesize{(d) Decluttering}
		\\ [1ex] 
		
		\epsfig{file=res_3p_5.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_6.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_7.jpeg,width=0.23\textwidth}
		&
		\epsfig{file=res_3p_8.jpeg,width=0.23\textwidth}
		\\
		
		\footnotesize{(e) Decluttering}
		&
		\footnotesize{(f) Grasping attempt,}
		&
		\footnotesize{(g) Grasping again after }
		&
	    \footnotesize{(h) Grasp success confirmation}
		\\
		&
		\footnotesize{box slipped in the process}
		&
		\footnotesize{updating RFID location }
		&
	    \footnotesize{by RFID location change}
		\\
\end{tabular}
\caption {\textbf{Multi-Obstacle \& Clutter Scenario. } a) In the initial state, an RFID tagged item is occluded under clutter inside one of the boxes. There is no line-of-sight to the item from camera or antennas. b) The robot explores the environment using RF-guided exploration. c) \name\ performs another iteration of exploration, and the stopping criteria is met. As a result, \name moves to grasping phase d) The robot grasps an item. However, since the RFID location doesn't change, it concludes that the recently grasped item is a clutter. e) The robot removes more clutter.  
f) Robot tries grasping the tagged item. However, it misses the item as the box slippes in the process and changes the item location. e) \name\ updates the tagged item location, and tries grasping again. g) The robot confirms that it grasped the item of interest because the RFID location changes with accordingly.}
\label{fig:intro-fig}
\end{figure*}

Designing a robotic system that leverages RFIDs for grasping is
challenging for many reasons. First, unlike cameras, a radio
perception module cannot produce high-resolution images with
pixel-wise precision~\cite{RFCapture}; this makes it difficult to
determine grasping affordances. Second, existing learning models for
robotic grasping and exploration are primarily based on vision and are
not designed to incorporate RF features. Moreover, the fact that
occlusions are transparent to radio signals enables \name\ to locate
an RFID through occlusions but also prevents it from recognizing these
occlusions as obstacles and identifying viable paths around them to
grasp the object of interest.

To address these challenges, \name\ fuses RF and visual information to enable efficient robotic grasping of fully-occluded objects. The contributions of this paper are multi-fold:
\begin{Itemize}
    \item It presents the first system that bridges RF and vision perception \textit{(RF+RGDB)} to enable robotic grasping of fully-occluded objects.
    \item It introduces \textit{RF-visual servoing}, a novel controller that exploits RF and visual information to efficiently perform active exploration, obstacle avoidance, and navigation.
    \item It introduces \textit{RF-visual grasping}, a model-free deep reinforcement learning network that can learn efficient and complex policies for decluttering and grasping.
    \item It presents a prototype implementation and practical evaluation of the system, demonstrating its ability to perform previously infeasible tasks such as directly grasping target object from under a pile. 
\end{Itemize}


In comparison to vision-only systems, \name's design has the drawback
of requiring the target object(s) to be tagged with RFIDs. However, we believe that given the rate of adoption of RFIDs by many industries (with tens of billions deployed annually~\cite{RFIDmarket}), the system can have immediate practical impact. Fundamentally, we hope that this work will motivate further research on bridging RF and vision to enable novel robotic tasks.

%Despite
%this limitation, we argue that the system can enable many applications
%given the widespread adoption of RFIDs.
% (tens of billions of manufactured
%objects are annually tagged with RFIDs~\cite{XXX} and entire countries
%like Japan have announced that all future manufactured items must be
%tagged with RFIDs~\cite{XXX}). 
%More fundamentally, we hope that this work will motivate further
%research on bridging RF and vision to enable efficient and complex
%robotic tasks.


==> intro-8.tex <==
\section{Introduction}


\begin{figure}[h!]
	\centering
	\begin{tabular}{c}
		\epsfig{file=intro.jpeg,width=0.45\textwidth}
		\\
		\footnotesize{(a) Target object is fully-occluded in an unstructured environment.}
		\\
		%\epsfig{file=intro_2.jpeg,width=0.4\textwidth}
		%\\
		%\footnotesize{(b) }
		%\\
		\epsfig{file=intro_1.jpeg,width=0.45\textwidth}
		\\
		\footnotesize{(b) \name\ is successful in grasping the target object.}
		\\
\end{tabular}
\caption {\textbf{RF-Grasp can grasp fully-occluded objects.} (a) Even though the camera and RF sensor have no line-of-sight to the object, \name\ uses RF perception to identify and locate the target object through occlusions. (b) It employs \textit{RF-visual servoing} and \textit{RF-visual manipulation} to efficiently maneuver toward the object, declutter its  vicinity, grasp it, and pick it up.}
\label{fig:intro-fig}
\end{figure}

Mechanical search refers to the robotic task of searching for and retrieving a target object that is partially or fully occluded~\cite{IROS2019Xray,ICRA2019search,objectfinding,graspinvisible}. This problem arises frequently in unstructured environments such as warehouses and homes. For example, a warehouse robot may need to retrieve a customer’s desired object from under a pile, or it may need to fetch a tool (e.g., screwdriver) required to perform higher-order robotic tasks such as assembly.

To address this problem, the past few years have seen significant advances in learning models that can either recognize the target object through partial occlusions or actively explore the environment, searching for the object of interest. Recent proposals have also considered the geometry of the obstacles~\cite{BerkeleyGraspOcclusion,objectfinding} or pile~\cite{IROS2019Xray,ICRA2019search} to more efficiently explore and declutter the environment. However, existing mechanical search systems are inherently constrained by their vision sensors, which can only perceive objects in their direct line-of-sight. If the object of interest is behind an obstacle, they need to actively explore the environment searching for it, a process that can be very expensive~\cite{BerkeleyGraspOcclusion}. Moreover, these systems cannot generalize to \textit{extended mechanical search}, where the robot needs to prioritize retrieving \textit{all} objects belonging to a certain class (e.g., all erasers from a box) and sort them into a separate bin. Unless the robot knows the number of objects a priori, it is infeasible to declare task completion before extensively exploring and decluttering the environment.

In this paper, we draw on recent advances in RF (radio frequency) perception~\cite{TurboTrack,RFCapture} to enable highly-efficient and extended mechanical in unstructured environments. Unlike visible light and infrared, RF signals can traverse many everyday occlusions including cardboard boxes, wooden dividers (and walls), opaque plastic covers, and colored glass. This “see through” capability enables a robot to identify and locate objects tagged with passive RF stickers,\footnote{The stickers are batteryless RFIDs (Radio Frequency IDentifiers), which are 3-cent tags that have been widely adopted by many industries as barcode replacements.} even when they are fully occluded from its vision sensor. The key challenge with RF perception, however, is that unlike vision, it cannot produce high-resolution images with pixel-wise precision. Moreover, because standard (visual) occlusions are transparent to RF signals, a robot can neither perceive them using RF sensing nor reason about the collision avoidance and decluttering steps that may be necessary prior to grasping the target object.

%, a task that is necessary  needs other mechanism for  to plan or perform obstacle avoidance and decluttering.

We present RF-Grasp (shown in Fig.~\ref{fig:intro-fig}), the first robotic system that fuses RF and vision information (RF+RGBD) to enable efficient and generalized mechanical search, across line-of-sight, non-line-of-sight, and highly cluttered environments. This paper provides four contributions:
 \begin{Itemize}
    \item It presents the first system that bridges RF and vision perception \textit{(RF+RGBD)} to enable mechanical search and extended mechanical search.
    \item It introduces \textit{RF-visual servoing}, a novel controller that performs RF-guided active exploration and navigation to avoid obstacles and maneuver toward the target object.
    \item It introduces \textit{RF-visual grasping}, a model-free deep reinforcement learning network that employs RF-based attention to vision input in order to learn and execute efficient and complex policies for decluttering and grasping.
    \item It presents a prototype implementation and practical evaluation of the system and a baseline across over 100 physical experiments, demonstrating \name's ability to efficiently perform mechanical search as well as previously infeasible tasks such as retrieving all objects of interest.
\end{Itemize}

In comparison to vision-only systems, \name's design has the drawback
of requiring the target object(s) to be tagged with RFIDs. However, we believe that given the rate of adoption of RFIDs by many industries (with tens of billions deployed annually~\cite{RFIDmarket}), the system can have immediate practical impact. Fundamentally, we hope that this work will motivate further research on bridging RF and vision to enable novel and more efficient robotic tasks.


==> intro-9.tex <==
\vspace{-0.1in}
\section{Introduction}
\vspace{-0.05in}

% \begin{figure}[t]
% 	\centering
% 	\begin{tabular}{c}
% 		\epsfig{file=intro.jpeg,width=0.35\textwidth}
% 		\\
% 		\footnotesize{(a) Target object is fully-occluded in an unstructured environment.}
% 		\\
% 		%\epsfig{file=intro_2.jpeg,width=0.4\textwidth}
% 		%\\
% 		%\footnotesize{(b) }
% 		%\\
% 		\epsfig{file=intro_1.jpeg,width=0.35\textwidth}
% 		\\
% 		\footnotesize{(b) \name\ is successful in grasping the target object.}
% 		\\
% \end{tabular}

%\setlength{\tabcolsep}{0pt}
\begin{figure}[t]
	\centering
	\setlength{\tabcolsep}{0pt}
	\begin{tabular}{cc}
	\multicolumn{2}{c}{
		\epsfig{file=intro.jpeg,width=0.4\textwidth}}
		\\
	\multicolumn{2}{c}{
		\footnotesize{(a) Target object is fully-occluded in an unstructured environment.}}
		\\
		%\epsfig{file=intro_2.jpeg,width=0.4\textwidth}
		%\\
		%\footnotesize{(b) }
		%\\
		\epsfig{file=intro_1.jpeg,width=0.22\textwidth}
		&
		\epsfig{file=intro_2.jpeg,width=0.22\textwidth}
		\\
		\footnotesize{(b) Decluttering}
		& 
		\footnotesize{(c) Successful Grasping}
\end{tabular}

%\setlength{\tabcolsep}{12pt}

% 	\begin{tabular}{cc}
% 	\multirow{ 2}{*}{
% 		\epsfig{file=intro.jpeg,width=0.35\textwidth}}
% 		& \epsfig{file=intro_1.jpeg,width=0.1\textwidth}
% 		\\
% 		& \footnotesize{(b) }
% % 		\\
% % 		& \epsfig{file=intro_1.jpeg,width=0.1\textwidth}
% % 		\\
% % 		\footnotesize{(a) Target object is fully-occluded in an unstructured environment.}
% % 	    &
% % 		\footnotesize{(c) \name\ is successful in grasping the target object.}
% 		\\
% \end{tabular}

\caption {\textbf{RF-Grasp grasping fully-occluded objects.} (a) Even though the camera and RF sensor have no line-of-sight to the object, \name\ uses RF perception to identify and locate the target object through occlusions. (b) It employs \textit{RF-visual servoing} and \textit{RF-visual manipulation} to efficiently maneuver toward the object and declutter its  vicinity. (c) Successful pick-up.}
\label{fig:intro-fig}
\vspace{-0.15in}
\end{figure}



Mechanical search is a fundamental problem in robotics~\cite{IROS2019Xray,ICRA2019search,objectfinding,graspinvisible}. It refers to the robotic task of searching for and retrieving a target object that is partially or fully occluded. This problem arises frequently in unstructured environments such as warehouses, hospitals, agile manufacturing plants, and homes. For example, a warehouse robot may need to retrieve an e-commerce customer’s desired item from under a pile. Similarly, a mobile robot may need to retrieve a desired tool (e.g., screwdriver) from behind an obstacle to perform a complex task such as furniture assembly~\cite{ikeabot}.
%
%it may need to fetch a tool (e.g., screwdriver) required to perform higher-order robotic tasks such as assembly.
%

To address this problem, the past few years have seen significant advances in learning models that can either recognize the target object through partial occlusions or actively explore the environment, searching for the object of interest. Recent proposals have also considered the geometry of obstacles or pile~\cite{IROS2019Xray,ICRA2019search,BerkeleyGraspOcclusion}, and demonstrated remarkable results in efficiently exploring and decluttering the environment. %, demonstrating remarkable results.

However, existing mechanical search systems are inherently constrained by their vision sensors, which can only perceive objects in their direct line-of-sight. If the object of interest is behind an obstacle, they need to actively explore the environment searching for it, a process that can be very expensive and often fails~\cite{BerkeleyGraspOcclusion}. Moreover, these systems are typically limited to a single pile or pick-up bin~\cite{IROS2019Xray,objectfinding}, and cannot generalize to \textit{extended mechanical search} problems. One such example involves robots that need to prioritize retrieving \textit{all} objects belonging to a certain class (e.g., all plastic bottles from a box) and sort them into a separate bin; unless the robot knows the number of objects a priori, it is infeasible to declare task completion before extensively exploring and decluttering the environment.

In this paper, we draw on recent advances in RF (radio frequency) perception~\cite{TurboTrack,RFCapture} to enable highly-efficient as well as extended mechanical search in unstructured environments. Unlike visible light and infrared, RF signals can traverse many everyday occlusions including cardboard boxes, wooden dividers (and walls), opaque plastic covers, and colored glass. This “see through” capability enables a robot to identify and locate objects tagged with passive RF stickers,\footnote{The stickers are batteryless RFIDs (Radio Frequency IDentifiers), which are 3-cent tags widely adopted by many industries as barcode replacements.} even when they are fully occluded from its vision sensor. The key challenge with RF perception, however, is that unlike vision, it cannot produce high-resolution images with pixel-wise precision. Moreover, because standard (visual) occlusions are transparent to RF signals, a robot can neither perceive them using RF sensing nor reason about the collision avoidance and decluttering steps that may be necessary prior to grasping the target object.

%, a task that is necessary  needs other mechanism for  to plan or perform obstacle avoidance and decluttering.

We present RF-Grasp (shown in Fig.~\ref{fig:intro-fig}), the first robotic system that fuses RF and vision information (RF+RGB-D) to enable efficient and generalized mechanical search, across line-of-sight, non-line-of-sight, and highly cluttered environments. This paper provides three main contributions:
 \begin{Itemize}
    \item It presents the first system that bridges RF and vision perception \textit{(RF+RGB-D)} to enable mechanical search and extended mechanical search.
    \item It introduces two novel primitives: (1) \textit{RF-visual servoing}, a novel controller that performs RF-guided active exploration and navigation to avoid obstacles and maneuver toward the target object, and (2) \textit{RF-visual grasping}, a model-free deep reinforcement learning network that employs RF-based attention to learn and execute efficient and complex policies for decluttering and grasping.
    \item It presents an end-to-end prototype implementation and evaluation of \name. The implementation is built using a UR5e robot, Intel RealSense D415 depth camera, and a customized RF localization system on software radios. The system is evaluated in over 100 physical experiments and compared to a baseline that combines two prior systems~\cite{BerkeleyGraspOcclusion,graspinvisible}. The evaluation demonstrates that \name\ improves success rate by up to 40\% and efficiency by up to 50\% in challenging environments. Moreover, it demonstrates that \name\ can perform novel mechanical search tasks of fully-occluded objects across settings with obstacles, multiple piles, and multiple target objects.
\end{Itemize}

In comparison to vision-only systems, \name's design requires the target object(s) to be tagged with RF stickers (RFIDs). However, we believe that given the widespread adoption of RFIDs by many industries (with tens of billions deployed annually~\cite{RFIDmarket}), the system can already have significant practical impact. More generally, we hope that this work motivates new research that bridges RF and vision perception to enable novel (and efficient) robotic tasks.

==> learning-1.tex <==
\section{Radio-Visual Learning of Manipulation
Policies}\label{sec:learning}

Things to cover: Attention mechanism, reward function, full framework\\


In this section, we describe how \name$_$ performs grasping of tagged item. We use an off-policy Q-learning approach to find an optimal policy maximizing the expected sum of future rewards that are calculated from a spatio-temporal reward function. 

The grasping problem is to maximize the action-value function $Q(s_i,a_i)$ that estimates the expected reward of taking the action $a_i$ at the state of $s_i$. Q-learning can be defined simply as : 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$
Where $R_{t+1}$ is the reward that system receives after action $a_t$. The aim of the network is to learn Q-function by minimizing: $$ \delta_t = [R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\subsection{States}
Our grasping network's state consist of a RGB height-map, a depth height-map, and a probability map of RFID location. We get the RGB-D data from a wrist-mounted camera, and project the pointcloud to a height-map whose boundaries are defined by the workspace limit of setup and the surrounding area of RFID tagged object. RFID-localization system provides the probability map of RFID location.\\
% For each state, the inputs are rotated to produce 16 different orientations. These 16 different groups of inputs are fed separately to the grasp (push) network, producing 16 outputs. The output that contains the pixel with highest value of all shows the proper gripper direction for performing grasp (push).

\subsection{Actions}
% \subsubsection{Pushing}
% The output of the push network is 16 probability maps. The push starting point is the pixel with highest probability of successful push in one of the 16 outputs (aka directions). A 10-cm push is executed from the chosen point in one of the 16 directions.  The robot gets the height of the action-point from depth height-map, and pushes the blocks by the finger tips of the closed gripper.
% \subsubsection{Grasping}
The grasping action can happen in eight different directions anywhere in the work space. For each state, the inputs are rotated to produce 16 different orientations. Then, they are fed separately to the grasping network, producing 16 outputs. The point with the highest value, action-point, represents the best position for middle point of gripper to performing a grasping action. The rotation of the output sets rotation of the gripper. \textcolor{red}{WHAT?!} Since the gripper is symmetrical, these 16 direction of gripper maps to 8 different direction of grasping. The robot gets the height of the action-point from depth height-map, moves the gripper above the intended action-point, lowers the gripper to put the block between its fingers, and then closes the gripper.

\subsection{Fully Convolutional Attention-based Learning}

\subsubsection{Network Architecture}

 We trained a feed-forward fully convolutional networks (FCNs) that takes the state representatives and outputs pixel-wise map of Q values. The output is then mapped to the workspace in post-processing. The FCN has two input streams: 1) three channels of RGB height-map data, 2) three channels consisting of depth height-map, RFID probability map, and multiplication of a binary mask by the depth map. The binary mask shows the immediate vicinity of RFID tagged object with 1 and other places with 0. \\
Each input stream goes through a 121-layer DenseNet whose initial weights were taken from the pre-trained model in \cite{PushGrasp}. Then, the output of two streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. When testing, the probability map of RFID is also dotted with the output of last CNN layer to focus the attention of the network on the RFID.\\
To learn orientation influence on grasping, network inputs are rotated into 16 directions and fed separately to the network. The output contains 16 maps for grasp, from which we choose the position and rotation with highest probability of success.\\

\begin{figure*}[ht]
	\begin{center}
		\includegraphics[width =\textwidth, height= 0.345\textwidth]{net.jpeg}
		\caption{Network overview}
		\label{net}
	\end{center}
\end{figure*}

\subsubsection{Pre-process Attention}
Before feeding the RGB height-map and depth height-map to the network, they are cropped to create a 11cm$\times$11cm square around the most probable location of RFID. This early-stage attention mechanism, enabled by RFID localization, allows the network to focus more on the vicinity of the object of interest and calculates with higher resolution and less computational complexity. 

\subsubsection{Mid-process Attention }
The pre-trained 121-layer DenseNet input is a 4-dimensional tensor with 3 channels. The first stream gets the $11cm\times11cm$ cropped RGB height-map around the RFID location as input. The second stream gets the $11cm\times11cm$ cropped depth height-map around the RFID location, a probability 2-D mask of the RFID's position, and  the multiplication of the cropped depth height-map by the binary mask of $5\times5$ centered at RFID's most probable location.\\ 


\subsubsection{Post-processing Attention}
Grasping network produces a 2-d matrix, elements of which are  the Q value estimations of performing the action at the represented area by that matrix element. To focus the attention of grasping system on the area containing the object of interest, we multiply the grasping Q-values by a Gaussian mask centered at the most probable RFID location while testing the system. In this case, the probability of grasping the item of interest increases.\\ 


\subsection{Reward}
Rewards are calculated from a spatio-temporal reward function.  Reward with a $\gamma$-discount sum is given by: 
$$R=\sum_{i=t}^{\infty}\gamma R(s_i, s_{i+1}, \dist(\text{apoint}_i,\text{target}_i))$$
where $apoint_i$ (action point $i$) refers to the position that action was performed, and $target_i$ is the position of RFID-tagged object. 
Reward function rewards successful grasp near the item of interest ($\text{target}$) more than successful grasps of items which are far from the item of interest. The future discount, $\gamma$, is set to be $0.2$.



\subsection{Training Details}
We used Huber loss function for training our network to reduce sensitivity to outliers.
$$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
$$L_i = \begin{cases} 
\frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
|  \delta_i | - \frac{1}{2}, \text{ Otherwise}
\end{cases}
$$ 
The networks were trained by stochastic gradient descent with learning rates of $10^{-4}$, momentum of $0.9$, and weight decay of $2^{-5}$.


\subsection{Experience Replay}
We use Prioritized Approbatory experience replay in the training process \textcolor{red}{(I coined the word)}to bias the network toward grasps in the vicinity of RFID location. In every iteration a threshold is defined   $\text{tr}=0.05 + \min(0.05\times\text{\#iteration},4)$. Among those action with a reward above the threshold, a stochastic rank-based prioritization is performed. The prioritization is estimated by a power-law distribution. 















==> learning-2.tex <==
\section{Radio-Visual Learning of Manipulation
Policies}\label{sec:learning}

\begin{figure*}[ht]
	\begin{center}
		\includegraphics[width =\textwidth, height= 0.345\textwidth]{net.jpeg}
		\caption{\textbf{Network Overview.} Using RFID location, \name\ crops out the RGB-D data near the tagged object location, and feeds the cropped RGB-D data and RFID location probability as input to the Deep-NN that outputs the Q-value estimations. The rotated inputs in 16 different directions are separately fed to DNN to estimate Q-values of different grasping rotations.}
		\label{fig:net}
	\end{center}
\end{figure*}

Things to cover: Attention mechanism, reward function, full framework\\


In this section, we describe how \name\ solves the problem of semantic grasping of fully occluded items. The goal of system is to grasp a requested tagged item, localized at $\mathbf{p}=(x_p,y_p,z_p)$ in an environment containing occluded regions, obstacles, and other objects. We frame the problem as a  Markov decision process (MDP) defined by a a 4-tuple $(S,A,T,R)$.

We use an off-policy Q-learning approach to find an optimal policy maximizing the expected sum of future rewards that are calculated from a spatio-temporal reward function. 

The grasping problem is to maximize the action-value function $Q(s_i,a_i)$ that estimates the expected reward of taking the action $a_i$ at the state of $s_i$. Q-learning can be defined simply as : 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$
Where $R_{t+1}$ is the reward that system receives after action $a_t$. The aim of the network is to learn Q-function by minimizing: $$ \delta_t = [R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\subsection{States}
Our grasping network's state consist of a RGB height-map, a depth height-map, and a probability map of RFID location. We get the RGB-D data from a wrist-mounted camera, and project the pointcloud to a height-map whose boundaries are defined by the surrounding area of RFID tagged object. RFID-localization system provides the probability map of RFID location.
% For each state, the inputs are rotated to produce 16 different orientations. These 16 different groups of inputs are fed separately to the grasp (push) network, producing 16 outputs. The output that contains the pixel with highest value of all shows the proper gripper direction for performing grasp (push).
\subsection{Actions}
% \subsubsection{Pushing}
% The output of the push network is 16 probability maps. The push starting point is the pixel with highest probability of successful push in one of the 16 outputs (aka directions). A 10-cm push is executed from the chosen point in one of the 16 directions.  The robot gets the height of the action-point from depth height-map, and pushes the blocks by the finger tips of the closed gripper.
% \subsubsection{Grasping}
The grasping action can happen in eight different directions anywhere in the work space. For each state, the inputs are rotated to produce 16 different orientations. Then, they are fed separately to the grasping network, producing 16 outputs. The point with the highest value, action-point, represents the best position for middle point of gripper to perform grasping. The rotation of the output sets rotation of the gripper. \textcolor{red}{WHAT?!} Since the gripper is symmetrical, these 16 directions of gripper maps to 8 different direction of grasping. The robot gets the height of the action-point from depth height-map, moves the gripper above the intended action-point, lowers the gripper to put the block between its fingers, and then closes the gripper.

\subsection{Fully Convolutional Attention-based Learning}

\subsubsection{Network Architecture}

We trained a feed-forward fully convolutional networks (FCNs) that takes the state representatives and outputs pixel-wise map of Q values.The overview of the architecture is presented in Figure \ref{fig:net}. The output is then mapped to the workspace in post-processing. The FCN has two input streams: 1) three channels of RGB height-map data, 2) three channels including two copies of depth height-map and RFID probability map. The binary mask shows the immediate vicinity of RFID tagged object with 1 and other places with 0. \\
Each input stream goes through a 121-layer DenseNet whose initial weights were taken from the pre-trained model in \cite{PushGrasp}. Then, the output of two streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. When testing, the probability map of RFID is also dotted with the output of last CNN layer to focus the attention of the network on the RFID.\\
To learn orientation's influence on grasping, network inputs are rotated into 16 directions and fed separately to the network. The output contains 16 maps for grasp, from which we choose the position and rotation with highest probability of success.

\subsubsection{Pre-process Attention}
The RGB height-map and depth height-map are cropped to create a 11cm$\times$11cm square around the most probable location of RFID. This early-stage attention mechanism, enabled by RFID localization, allows the network to focus more on the vicinity of the object of interest and calculates with higher resolution and less computational complexity. 

% \subsubsection{Mid-process Attention }
% The pre-trained 121-layer DenseNet input is a 4-dimensional tensor with 3 channels. The first stream gets the $11cm\times11cm$ cropped RGB height-map around the RFID location as input. The second stream gets the $11cm\times11cm$ cropped depth height-map around the RFID location, a probability 2-D mask of the RFID's position, and  the multiplication of the cropped depth height-map by the binary mask of $5\times5$ centered at RFID's most probable location.\\ 

\subsubsection{Post-processing Attention}
Grasping network produces a 2-d matrix, whose elements are  the Q value estimations of grasping at the position represented by the matrix element. To focus the attention of system, we dot the Q-values matrix by a Gaussian mask centered at the most probable RFID location while testing the system. In this case, the probability of grasping the item of interest increases.

\subsection{Grasp Success Assessment and Rewards}

When the robot closes its gripper, and move in Z direction for 10 cm, the RFID location system updates the tagged-item location. If the tagged-item has also moved 10cm in Z direction, the grasp is announced successful. Otherwise, \name\ concludes it has grasped a clutter/cover that was on or near the tagged-item and puts it aside. The robot then returns to previous locations and tries grasping again.  

Rewards are calculated from a spatio-temporal reward function.  Reward with a $\gamma$-discount sum is given by: 
$$R=\sum_{i=t}^{\infty}\gamma^{i-t} r(s_i, s_{i+1}, a_i)$$
where $apoint_i$ (action point $i$) refers to the position that action was performed, and $target_i$ is the position of RFID-tagged object. 
Reward function rewards successful grasp near the item of interest ($\text{target}$) more than successful grasps of items which are far from the item of interest. The future discount, $\gamma$, is set to be $0.2$.



\subsection{Training Details}
We used Huber loss function for training our network to reduce sensitivity to outliers.
% $$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
% $$L_i = \begin{cases} 
% \frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
% |  \delta_i | - \frac{1}{2}, \text{ Otherwise}
% \end{cases}
% $$ 
The networks were trained by stochastic gradient descent with learning rates of $10^{-4}$, momentum of $0.9$, and weight decay of $2^{-5}$.


\subsection{Experience Replay}
We use Prioritized experience replay in the training process. We defined a threshold as $\text{tr}=0.05 + \min(0.05\times\text{\#iteration},4)$ to bias the network toward grasps in the vicinity of RFID location. Among those experiences with a reward above the threshold, a stochastic rank-based prioritization is performed. The prioritization is estimated by a power-law distribution. 












==> learning-3.tex <==
\section{Radio-Visual Learning of Grasping
Policies}\label{sec:grasping}

\begin{figure}
	\begin{center}
		\includegraphics[width =0.48\textwidth]{Grasping_Paper/figures/Net_new.jpeg}
		\caption{\textbf{RF-Visual Grasping.} Using the RFID's location, \name\ crops out the RGB-D data near the tagged object location, and feeds the cropped RGB-D data and RFID location probability as input to the Deep-NN that outputs the Q-value estimations. The rotated inputs in 16 different directions are separately fed to DNN to estimate Q-values of different grasping rotations.}
		\label{fig:net}
	\end{center}
\end{figure}

%Things to cover: Attention mechanism, reward function, full %framework

The above primitive enables the robot to intelligently explore the environment and servo the robotic arm closer to the object of interest. Once the object is within reach, \name\ still needs to grasp it. In this section, we describe how \name\ exploits RF-based attention to learn efficient grasping policies. 

\subsection{Problem Statement}

The goal of system is to grasp a requested tagged item, localized at $\mathbf{p}=(x_p,y_p,z_p)$ in an explored environment that previously contained occluded regions. We frame the grasping phase problem as a Markov Decision Process (MDP) defined by a a 4-tuple $\mathcal{(S,A,T,R)}$.

\begin{itemize}
    \item \textbf{States $\mathcal{(S)}$:} State can be represented by the robot joint state $\mathbf{x}_t^R$, RFID tagged item location $\mathbf{p}_t$, and RGB-D data from wrist-mounted camera.
    
    \item \textbf{Actions $\mathcal{(A)}$:} Grasping action $a_t$ happens at position $(x_{a_t},y_{a_t},z_{a_t})$ with gripper rotation of $\theta_{a_t}$. 
    
    \item \textbf{Transition Function $\mathcal{(T)}$:} the transition model is $T(s_{t+1} | s_t , a_t )$. Next states are determined by executing action and waiting until objects come to rest. 
    
    \item \textbf{Reward $\mathcal{(R)}$:} Reward is $r_t = r(s_t, s_{t+1}, a_t) \in [0,5]$. It is equal to 5 if it grasps the requested item, and 0 if it does not grasp anything. Any other grasp is rewarded $(0,5)$ depending of distance from requested item.
\end{itemize}
\noindent
Given the problem definition, the objective is to find an optimal policy maximizing the expected sum of future rewards, given the current state. Similar to prior work on unsupervised grasping, we use a Deep Q-Network (DQN, an off-policy Q-learning approach) to achieve this.

The action-value function $Q(s_i,a_i)$ estimates the expected reward of taking the action $a_i$ at the state of $s_i$. Q-learning can be defined simply as : 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$
Where $R_{t+1}$ is the reward that system receives after action $a_t$. The aim of the network is to learn Q-function by minimizing: $$ \delta_t = [R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\subsection{Spatio-Temporal Reward Function}

\name\ uses RFID tags' location to assess the performance of the system and to reward accordingly. Rewards are calculated from a spatio-temporal reward function where it rewards successful grasp of the item of interest the highest. For grasping other items, the nearer they were located to the requested item, the higher will be the reward value. Reward with a $\gamma$-discount sum is given by: 
$$R_t=\sum_{i=t}^{\infty}\gamma^{i-t} r_t(s_i, s_{i+1}, a_i)$$ Where $\gamma$ is the discount factor for future rewards. To asses the system grasping performance, the robot moves for 10 cm in Z direction after it closes its gripper. The RFID location system updates the tagged-item locations; If the tagged-item has also moved 10cm in Z direction, the grasp is announced successful. Otherwise, \name\ concludes it has grasped a clutter/cover that was on or near the tagged-item and puts it aside. 



\subsection{Deep Reinforcement Learning with RF-based Attention}
To learn efficient grasping policies of potentially-cluttered objects, \name\ extends prior work on deep reinforcement networks for learning grasping policies by folding RF-based attention. 

The overall architecture of the network is shown in Fig.~\ref{fig:net} and consists of feed-forward fully convolutional networks (FCNs). The networks takes the state representatives (RGB-D and RFID 3D position) as input, and outputs pixel-wise map of Q values. The output is then mapped to the workspace in post-processing. The network determines the optimal grasping point as the one having the highest probability acrosss the output affordance map.

\name\ incorporates RF-attention into the network through three main strategies:
\begin{itemize}
    \item \textit{Pre-processing Attention (RF-based Mask).} The RGB height-map and depth height-map are cropped to create a 11cm$\times$11cm square around the most probable location of RFID. This early-stage attention mechanism, enabled by RFID localization, allows the network to focus more on the vicinity of the object of interest and calculates with higher resolution and less computational complexity. 
    \text \textit{Intra-network attention layer (RF kernel).}
    \item \textit{Post-Processing Attention.}

Grasping network produces a 2-d matrix, whose elements are  the Q value estimations of grasping at the position represented by the matrix element. To focus the attention of system, we dot the Q-values matrix by a Gaussian mask centered at the most probable RFID location while testing the system. In this case, the probability of grasping the item of interest increases.

To discover optimal grasping affordances, the inputs to the network are rotated into 16 directions and fed separately to the network. The output contains 16 maps for grasp, from which we choose the position and rotation with highest probability of success.
\end{itemize}

The FCN has two input streams: 1) three channels of RGB height-map data, 2) three channels including two copies of depth height-map and RFID probability map. The binary mask shows the immediate vicinity of RFID tagged object with 1 and other places with 0. 

Each input stream goes through a 121-layer DenseNet whose initial weights were taken from the pre-trained model in \cite{PushGrasp}. Then, the output of two streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. When testing, the probability map of RFID is also dotted with the output of last CNN layer to focus the attention of the network on the RFID.


\subsubsection{Pre-process Attention}
The RGB height-map and depth height-map are cropped to create a 11cm$\times$11cm square around the most probable location of RFID. This early-stage attention mechanism, enabled by RFID localization, allows the network to focus more on the vicinity of the object of interest and calculates with higher resolution and less computational complexity. 


\subsubsection{Post-processing Attention}
Grasping network produces a 2-d matrix, whose elements are  the Q value estimations of grasping at the position represented by the matrix element. To focus the attention of system, we dot the Q-values matrix by a Gaussian mask centered at the most probable RFID location while testing the system. In this case, the probability of grasping the item of interest increases.

To discover optimal grasping affordances, the inputs to the network are rotated into 16 directions and fed separately to the network. The output contains 16 maps for grasp, from which we choose the position and rotation with highest probability of success.

\subsection{Training Details}
We used Huber loss function for training our network to reduce sensitivity to outliers.
% $$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
% $$L_i = \begin{cases} 
% \frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
% |  \delta_i | - \frac{1}{2}, \text{ Otherwise}
% \end{cases}
% $$ 
The networks were trained by stochastic gradient descent with learning rates of $10^{-4}$, momentum of $0.9$, and weight decay of $2^{-5}$. The reward discount factor was also set to be 0.2.


\subsection{Experience Replay}
We use Prioritized experience replay in the training process. We defined a threshold as $\text{tr}=0.05 + \min(0.05\times\text{\#iteration},4)$ to bias the network toward grasps in the vicinity of RFID location. Among those experiences with a reward above the threshold, a stochastic rank-based prioritization is performed. The prioritization is estimated by a power-law distribution. 












==> learning-4.tex <==
\section{Radio-Visual Learning of Grasping
Policies}\label{sec:grasping}

\begin{figure}
	\begin{center}
		\includegraphics[width =0.48\textwidth]{Grasping_Paper/figures/Net_new.jpeg}
		\caption{\textbf{RF-Visual Grasping.} Using the RFID's location, \name\ crops out the RGB-D data near the tagged object location, and feeds the cropped RGB-D data and RFID location probability as input to the Deep-NN that outputs the Q-value estimations. The rotated inputs in 16 different directions are separately fed to DNN to estimate Q-values of different grasping rotations.}
		\label{fig:net}
	\end{center}
\end{figure}

%Things to cover: Attention mechanism, reward function, full %framework

The above primitive enables \name\ to intelligently explore the environment and servo the robotic arm around obstacles, and closer to the object of interest, but the robot still needs to grasp it. 
Below, we describe how \name\ exploits RF-based attention to learn efficient grasping policies. 

\subsection{The Grasping Sub-problem}

We formulate the grasping sub-problem as a Markov Decision Process (MDP). Here, the action $a_t$ is grasping with a parallel jaw gripper at position $\mathbf{g_t}= (x_{a_t},y_{a_t},z_{a_t})$ with gripper rotation of $\theta_{a_t}$. The goal is to learning the optimal policy $\pi*$ to grasp the item of interest either directly or after manipulating the environment.

This can be cast as a deep reinforcement learning problem where the robot aims to maximize the future reward (by grasping the target object). Similar to prior work on unsupervised grasping, we use a Deep Q-Network (DQN, an off-policy Q-learning approach) to solve this problem. The action-value function $Q(s_t,a_t)$ estimates the expected reward at the state  $s_t$ when taking the action $a_t$ according to the policy $\pi(s_t)$.  Q-learning can be defined as: 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$
Where $r_{t}$ is the reward that system receives after action $a_t$. $\alpha$ is the learning rate, and $\gamma$ is the discount factor. The aim of the network is to the learn Q-function by minimizing: $$ \delta_t = [r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$



The goal of system is to grasp a requested tagged item, localized at $\mathbf{p}=(x_p,y_p,z_p)$ in a cluttered environment. We frame the grasping phase problem as a Markov Decision Process (MDP) defined by a a 4-tuple $\mathcal{(S,A,T,R)}$.

\begin{itemize}
    \item \textbf{States $\mathcal{(S)}$:} State can be represented by the robot joint state $\mathbf{x}_t^R$, RFID tagged item location $\mathbf{p}_t$, and RGB-D heightmaps obtained from the wrist-mounted camera.\footnote{The heightmaps are computed by extracting 3D point cloud from RGB-D images and projecting the images orthographally upwards parallel to the table top. The RGB and depth heightmap represent color and height from tabletop respectively.}
    
    \item \textbf{Actions $\mathcal{(A)}$:} Grasping action $a_t$ happens at position $\mathbf{g_t}= (x_{a_t},y_{a_t},z_{a_t})$ with gripper rotation of $\theta_{a_t}$. 
    
    \item \textbf{Transition Function $\mathcal{(T)}$:} the transition model is $T(s_{t+1} | s_t , a_t )$. Next states are determined by executing action and waiting until objects come to rest. 
    
    \item \textbf{Reward $\mathcal{(R)}$:} Reward is $r_t = r(s_t, s_{t+1}, a_t) \in [0,5]$. It is equal to 5 if it grasps the requested item, and 0 if it does not grasp anything. Any other grasp is rewarded $(0,4.5)$ depending of distance from requested item.
\end{itemize}
\noindent
Given the problem definition, the objective is to find an optimal policy $\pi*$ maximizing the expected sum of future rewards, given the current state. Similar to prior work on unsupervised grasping, we use a Deep Q-Network (DQN, an off-policy Q-learning approach) to achieve this.

The action-value function $Q(s_t,a_t)$ estimates the expected reward at the state  $s_t$ when taking the action $a_t$ according to the policy $\pi(s_t)$.  Q-learning can be defined as: 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$
Where $r_{t}$ is the reward that system receives after action $a_t$. $\alpha$ is the learning rate, and $\gamma$ is the discount factor. The aim of the network is to the learn Q-function by minimizing: $$ \delta_t = [r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\subsection{Spatio-Temporal Reward Function}

\name\ uses RFID tags' location to assess the performance of the system and to reward accordingly. Rewards are calculated from a spatio-temporal function where successful grasp of items of interest are rewarded the highest. In the case of grasping other items, the nearer they were located to the requested item, the higher are the reward values. The reward function is as follows:
$$r(s_t, s_{t+1}, a_t) = \begin{cases}
      5 & \text{\footnotesize{Grasped requested item}}\\
      \max{(\frac{\varrho}{||\mathbf{p}_t - \mathbf{g}_t||},4.5)}& \text{\footnotesize{Grasped another item}}\\
      0 & \text{\footnotesize{Otherwise}}
    \end{cases}$$
where $\varrho$ is a constant\footnote{In  our  implementation, $\varrho$ is set to 0.035.}. As the robot pose changes after grasping, the RFID location system updates the tagged-item location. If the tagged-item moves with robot the end-effector, the grasp is announced successful. Otherwise, \name\ concludes it has grasped a clutter/cover that was on or near the tagged-item, and puts it aside. 



\subsection{Deep Reinforcement Learning with RF-based Attention}
\name\ trains a deep reinforcement learning entirely in simulation, and folds in RF-based attention into the network. The overall architecture of the network is shown in Fig.~\ref{fig:net} and consists of feed-forward fully convolutional networks (FCNs). The networks take the state representatives (RGB-D and RFID 3D position) as input, and output pixel-wise map of Q values. 
The network determines the optimal grasping policy as the one having the highest Q across the output affordance map.

\name\ incorporates RF-based attention through two main strategies (and at three different layers):
\begin{itemize}
    \item \textit{RF-based Binary Mask (pre-processing attention).} The RGB and depth heightmaps are cropped to a N$\times$N region around the most probable location of RFID.\footnote{In our implementation, it is set to 11cm$\times$11cm.} This early-stage attention mechanism, enabled by RFID localization, allows the network to focus more on the vicinity of the target object and compute the affordance map with higher resolution and/or less computational complexity. 
    \item \textit{RF Kernel.} The RFID location is also used to construct an RF kernel, which consists of a 2D Gaussian centered around the RFID location, and whose standard deviation allows accounting for RF localization errors. The 2D kernel is fed into the network alongside depth heightmap. It is also multiplied by the output of DQN's last layer to compute the final affordance map. Both of approaches serve serve as attention mechanisms to increase the probability of grasping the item of interest. We note that the multiplication by the kernel at the output is only used in testing but not in training, as it yielded better performance.
    %\item \textit{Post-Processing Attention.}
\end{itemize}

\name\ uses the above RF attention mechanisms to extend a state-of-the-art deep-reinforcement learning grasping network. The FCN has two input streams: 1) three channels of cropped RGB heightmap and  2) three channels including two copies of cropped depth heightmap and the RF kernel. To discover optimal grasping affordances, the inputs to the network are rotated into 16 directions and fed separately to the network. Each input stream goes through a 121-layer DenseNet whose initial weights were taken from the pre-trained model in \cite{PushGrasp}. Then, the output of two streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. The output contains 16 maps for grasp, from which \name\ chooses the position and rotation with highest probability of success.

\subsection{Training Details} 
We use Huber loss function for training our network to reduce sensitivity to outliers.  We fine-tuned the weight of the network by training for 500 iterations in simulation. The gradient is only backpropagated through the pixel of affordance map that we executed grasping according to its predicted value. The network is trained by stochastic gradient descent with learning rates of $10^{-4}$, momentum of $0.9$, and weight decay of $2^{-5}$. The reward discount factor is also set to be 0.2.
% $$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
% $$L_i = \begin{cases} 
% \frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
% |  \delta_i | - \frac{1}{2}, \text{ Otherwise}
% \end{cases}
% $$ 

In the training process, we used prioritized experience replay \cite{prioritized} to improve sample efficiency and stability. In experience replay, a fixed number of the most recent experiences are saved, and the network is trained on a batch of a chosen set of transitions. We define a threshold as $\text{tr}=0.05 + \min(0.05\times\text{\#iteration},4)$, to perform a stochastic rank-based prioritization among experiences with a reward above the threshold. The prioritization is estimated by a power-law distribution. 












==> learning-5.tex <==
\vspace{-0.05in}
\section{Radio-Visual Learning of Grasping
Policies}\label{sec:grasping}
\vspace{-0.05in}

\begin{figure}
	\begin{center}
		\includegraphics[width =0.48\textwidth]{Grasping_Paper/figures/Net_new.jpeg}
		\caption{\textbf{RF-Visual Grasping.} Using the RFID's location, \name\ crops out the RGB-D data near the tagged object location, and feeds the cropped RGB-D data and RFID location probability as input to the Deep-NN that outputs the Q-value estimations. The rotated inputs in 16 different directions are separately fed to DNN to estimate Q-values of different grasping rotations.}
		\label{fig:net}
	\end{center}
	\vspace{-0.1in}
\end{figure}

%Things to cover: Attention mechanism, reward function, full %framework

The above primitive enables \name\ to intelligently explore the environment and servo the robotic arm around obstacles, and closer to the object of interest, but the robot still needs to grasp it. 
Below, we describe how \name\ exploits RF-based attention to learn efficient grasping policies. 

\subsection{The Grasping Sub-problem}

We formulate the grasping sub-problem as a Markov Decision Process (MDP). Here, the action $a_t$ is grasping with a parallel jaw gripper at position $\mathbf{g_t}= (x_{a_t},y_{a_t},z_{a_t})$ with gripper rotation of $\theta_{a_t}$. The goal is to learning the optimal policy $\pi^*$ to grasp the item of interest either directly or after manipulating the environment.

This can be cast as a deep reinforcement learning problem where the robot aims to maximize the future reward (by grasping the target object). Similar to prior work on unsupervised grasping, we use a Deep Q-Network (DQN, an off-policy Q-learning approach) to solve this problem. The action-value function $Q(s_t,a_t)$ estimates the expected reward at the state  $s_t$ when taking the action $a_t$ according to the policy $\pi(s_t)$.  Q-learning can be defined as: 
\vspace{-0.1in} 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\vspace{-0.1in}
\noindent
where $r_{t}$ is the reward that system receives after action $a_t$. $\alpha$ is the learning rate, and $\gamma$ is the discount factor. The aim of the network is to the learn Q-function by minimizing: 
\vspace{-0.1in}
$$ \delta_t = [r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\subsection{Spatio-Temporal Reward Function}

We construct a spatio-temporal reward function to encourage the robot to grasp the target item or those in its near vicinity. The reward function $r(s_t, s_{t+1}, a_t)$ is 1 if the robot grasps the target object;  $\max{(\frac{\varrho}{||\mathbf{p}_t - \mathbf{g}_t||},1)}$ if it grasps another item; and 0 otherwise. In  our  implementation, $\varrho$ is a constant set to 0.035. Since RF perception tracks the RFID's location, it can determine whenever the grasp is successful/picked up.

%As the robot pose changes after grasping, the RFID location system updates the tagged-item location. If the tagged-item moves with robot the end-effector, the grasp is announced successful. Otherwise, \name\ concludes it has grasped a clutter/cover that was on or near the tagged-item, and puts it aside. 

\subsection{Deep Reinforcement Learning with RF-based Attention}
\name\ trains a deep reinforcement learning network entirely in simulation, and folds RF-based attention into the network. The overall network architecture is shown in Fig.~\ref{fig:net} and consists of feed-forward fully convolutional networks (FCNs). The networks take state representations (RGB-D and RFID 3D position) as input, and outputs pixel-wise map of Q values. 
The network selects the optimal grasping policy as the one with the highest Q across the output affordance map.

\name\ incorporates RF-based attention through two main strategies (and at three different layers):
\begin{itemize}
    \item \textit{RF-based Binary Mask (pre-processing attention).} The RGB and depth heightmaps\footnote{The heightmaps are computed by extracting 3D point cloud from RGB-D images and projecting the images orthographally upwards parallel to the table top. The RGB and depth heightmap represent color and height from tabletop respectively.} are cropped to a N$\times$N region around the most probable location of RFID.\footnote{In our implementation, it is set to 11cm$\times$11cm.} This early-stage attention mechanism, enabled by RFID localization, allows the network to focus more on the vicinity of the target object and compute the affordance map with higher resolution and/or less computational complexity. 
    \item \textit{RF Kernel.} The RFID location is also used to construct an RF kernel, which consists of a 2D Gaussian centered around the RFID location, and whose standard deviation allows accounting for RF localization errors. The 2D kernel is fed into the network alongside depth heightmap. It is also multiplied by the output of DQN's last layer to compute the final affordance map. Both of approaches serve serve as attention mechanisms to increase the probability of grasping the item of interest. We note that the multiplication by the kernel at the output is only used in testing but not in training, as it yielded better performance.
    %\item \textit{Post-Processing Attention.}
\end{itemize}

\name\ uses the above RF attention mechanisms to extend a state-of-the-art deep-reinforcement learning grasping network. The FCN has two input streams: 1) three channels of cropped RGB heightmap and  2) three channels including two copies of cropped depth heightmap and the RF kernel. To discover optimal grasping affordances, the inputs to the network are rotated into 16 directions and fed separately to the network. Each input stream goes through a 121-layer DenseNet whose initial weights were taken from the pre-trained model in \cite{PushGrasp}. Then, the output of two streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. The output contains 16 maps for grasp, from which \name\ chooses the position and rotation with highest probability of success.

\vspace{0.05in}
\noindent
\textbf{Training Details.} 
We use Huber loss function for training our network to reduce sensitivity to outliers.  We fine-tuned the weight of the network by training for 500 iterations in simulation. The gradient is only backpropagated through the pixel of affordance map that we executed grasping according to its predicted value. The network is trained by stochastic gradient descent with learning rates  $10^{-4}$, momentum  $0.9$, and weight decay  $2^{-5}$. The reward discount factor is 0.2.
% $$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
% $$L_i = \begin{cases} 
% \frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
% |  \delta_i | - \frac{1}{2}, \text{ Otherwise}
% \end{cases}
% $$ 

In training, we used prioritized experience replay \cite{prioritized} to improve sample efficiency and stability. In experience replay, a fixed number of most recent experiences are saved, and the network is trained on a batch of a chosen set of transitions. We define a threshold as $\text{tr}=0.05 + \min(0.05\times\text{\#iteration},4)$, to perform a stochastic rank-based prioritization among experiences with a reward above the threshold. The prioritization is estimated by a power-law distribution. 












==> learning-6.tex <==
\vspace{-0.05in}
\section{Radio-Visual Learning of Grasping
Policies}\label{sec:grasping}
\vspace{-0.05in}

%Things to cover: Attention mechanism, reward function, full %framework

The above primitive enables \name\ to intelligently explore the environment and servo the robotic arm around obstacles, closer to the object of interest, but the robot still needs to grasp it. 
Below, we describe how \name\ exploits RF-based attention to learn efficient grasping policies. 

\vspace{-0.08in}
\subsection{The Grasping Sub-problem}
\vspace{-0.05in}
We formulate the grasping sub-problem as a Markov Decision Process (MDP). Here, the action $a_t$ is grasping with a parallel jaw gripper at position $\mathbf{g_t}= (x_{a_t},y_{a_t},z_{a_t})$ with gripper rotation of $\theta_{a_t}$. The goal is to learn the optimal policy $\pi^*$ to grasp the item of interest either directly or by manipulating the environment.

This can be cast as a deep reinforcement learning problem where the robot aims to maximize the future reward (by grasping the target object). Similar to prior work on unsupervised grasping~\cite{PushGrasp}, we use a Deep Q-Network (DQN, an off-policy Q-learning approach) to solve this problem. 

\textcolor{red}{REMOVE: The action-value function $Q(s_t,a_t)$ estimates the expected reward at the state  $s_t$ when taking the action $a_t$ according to the policy $\pi(s_t)$.  Q-learning can be defined as: }
\vspace{-0.08in} 
$$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

\vspace{-0.1in}
\noindent
\textcolor{red}{
where $r_{t}$ is the reward that system receives after action $a_t$. $\alpha$ is the learning rate, and $\gamma$ is the discount factor. The aim of the network is to the learn Q-function by minimizing: }
\vspace{-0.1in}
$$ \delta_t = [r_{t} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$


%As the robot pose changes after grasping, the RFID location system updates the tagged-item location. If the tagged-item moves with robot the end-effector, the grasp is announced successful. Otherwise, \name\ concludes it has grasped a clutter/cover that was on or near the tagged-item, and puts it aside. 

\begin{figure}
	\begin{center}
		\includegraphics[width =0.48\textwidth]{Grasping_Paper/figures/Net_new.jpeg}
		\vspace{-0.2in}
		\caption{\textbf{RF-Visual Grasping.} Using the RFID's location, \name\ crops out the RGB-D data near the tagged object location, and feeds the cropped RGB-D data and RFID location probability as input to the Deep-NN that outputs the Q-value estimations. The rotated inputs in 16 different directions are separately fed to DNN to estimate Q-values of different grasping rotations.}
		\label{fig:net}
	\end{center}
	\vspace{-0.12in}
\end{figure}

\vspace{-0.12in}
\subsection{RF-based Attention and Rewards}
\vspace{-0.05in}
\name\ trains a deep reinforcement learning network in simulation, and folds in RF information via reward and attention mechanisms. Fig.~\ref{fig:net} shows the overall architecture, consisting of feed-forward fully convolutional networks (FCNs). The networks take state representations (RGB-D and RFID position) as input, and output pixel-wise map of Q values. 
\name\ selects the optimal grasping policy as the one with the highest Q across the output affordance map.

\vspace{0.05in}
\noindent
\textbf{Spatio-Temporal Reward Function.}
We construct a spatio-temporal reward function to encourage the robot to grasp the target item or those in its near vicinity. The reward function $r(s_t, s_{t+1}, a_t)$ is 1 if the robot grasps the target object;  $\max{(\frac{\varrho}{||\mathbf{p}_t - \mathbf{g}_t||},1)}$ if it grasps another item; and 0 otherwise. In  our  implementation, $\varrho$ is a constant set to \textcolor{red}{0.0007. This way, any grasp within RFID accuracy will be rewarded 1}. Since RF perception tracks the RFID's location, it can determine whenever the grasp is successful (it is picked up).

\vspace{0.05in}
\noindent
\textbf{RF-based Attention.} 
\name\ incorporates RF-based attention through two main strategies (and at three layers):
\begin{itemize}
    \item \textit{RF-based Binary Mask.} The RGB and depth heightmaps\footnote{Heightmaps are computed by extracting 3D point cloud from RGB-D images and projecting the images orthographically, parallel to the table top.
    %The RGB and depth heightmap represent color and height from tabletop respectively.
    } are cropped to a square around the RFID's location (11cm$\times$11cm). This pre-processing attention mechanism allows the network to focus on the vicinity of the target object and compute the affordance map with higher resolution and/or less computational complexity. 
    \item \textit{RF Kernel.} The RFID location is also used to construct an RF kernel, a 2D Gaussian centered around $\mathbf{p}$, whose standard deviation accounts for RF localization errors. The kernel is fed to the network, and is multiplied by DQN's last layer to compute the final affordance map. This increases the probability of grasping the target item. %We note that the multiplication by the kernel at the output is only used in testing but not in training, as it yielded better results.
    %\item \textit{Post-Processing Attention.}
\end{itemize}

\name\ uses the above RF attention mechanisms to extend a state-of-the-art deep-reinforcement learning grasping network~\cite{PushGrasp}, as shown in Fig.~\ref{fig:net}. It consists of two 121-layer DenseNets: the first takes as input three channels of cropped RGB heightmaps; the second's input is the RF kernel plus two copies of cropped depth heightmap. To discover optimal grasping affordances, the inputs are rotated in 16 directions and fed separately to the network. Then, the outputs of both streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. The output contains 16 maps for grasp, from which \name\ chooses the position and rotation with highest probability of success.

\vspace{0.05in}
\noindent
\textbf{Training Details.} 
We use Huber loss function for training our network to reduce sensitivity to outliers.  The DenseNet initial weights were taken from the pre-trained model in \cite{PushGrasp}, and fine-tuned by training for 500 iterations in simulation. The gradient is only backpropagated through the pixel of affordance map that we executed grasping according to its predicted value. The network is trained by stochastic gradient descent with learning rates  $10^{-4}$, momentum  $0.9$, and weight decay  $2^{-5}$. The reward discount factor is 0.2.
% $$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
% $$L_i = \begin{cases} 
% \frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
% |  \delta_i | - \frac{1}{2}, \text{ Otherwise}
% \end{cases}
% $$ 

In training, we used prioritized experience replay~\cite{prioritized} to improve sample efficiency and stability. 
%In experience replay, a fixed number of most recent experiences are saved, and the network is trained on a batch of a chosen set of transitions. 
We define threshold $\rho_i=0.05 + \min(0.05\times\text{\#iteration},4)$, and performed stochastic rank-based prioritization among experiences with rewards $\ge\rho_i$. Prioritization is estimated by a power-law distribution. 












==> learning-7.tex <==
\vspace{-0.05in}
\section{Radio-Visual Learning of Grasping
Policies}\label{sec:grasping}
\vspace{-0.05in}

%Things to cover: Attention mechanism, reward function, full %framework

The above primitive enables \name\ to intelligently explore the environment and servo the robotic arm around obstacles, closer to the object of interest, but the robot still needs to grasp it. 
Below, we describe how \name\ exploits RF-based attention to learn efficient grasping policies. 

\vspace{-0.08in}
\subsection{The Grasping Sub-problem}
\vspace{-0.05in}
We formulate the grasping sub-problem as a Markov Decision Process (MDP). Here, the action $a_t$ is grasping with a parallel jaw gripper at position $\mathbf{g_t}= (x_{a_t},y_{a_t},z_{a_t})$ with gripper rotation of $\theta_{a_t}$. The goal is to learn the optimal policy $\pi^*$ to grasp the item of interest either directly or by manipulating the environment.

This can be cast as a deep reinforcement learning problem where the robot aims to maximize the future reward (by grasping the target object). Similar to prior work on unsupervised grasping~\cite{PushGrasp}, we use a Deep Q-Network (DQN, an off-policy Q-learning approach) to solve this problem. 

%As the robot pose changes after grasping, the RFID location system updates the tagged-item location. If the tagged-item moves with robot the end-effector, the grasp is announced successful. Otherwise, \name\ concludes it has grasped a clutter/cover that was on or near the tagged-item, and puts it aside. 

\begin{figure}
	\begin{center}
		\includegraphics[width =0.48\textwidth]{Grasping_Paper/figures/Net_new.jpeg}
		\vspace{-0.2in}
		\caption{\textbf{RF-Visual Grasping.} Using the RFID's location, \name\ crops out the RGB-D data near the tagged object location, and feeds the cropped RGB-D data and RFID location probability as input to the Deep-NN that outputs the Q-value estimations. The rotated inputs in 16 different directions are separately fed to DNN to estimate Q-values of different grasping rotations.}
		\label{fig:net}
	\end{center}
	\vspace{-0.12in}
\end{figure}

\vspace{-0.12in}
\subsection{RF-based Attention and Rewards}
\vspace{-0.05in}
\name\ trains a deep reinforcement learning network in simulation, and folds in RF information via reward and attention mechanisms. Fig.~\ref{fig:net} shows the overall architecture, consisting of feed-forward fully convolutional networks (FCNs). The networks take state representations (RGB-D and RFID position) as input, and output pixel-wise map of Q values. 
\name\ selects the optimal grasping policy as the one with the highest Q across the output affordance map.

\vspace{0.05in}
\noindent
\textbf{Spatio-Temporal Reward Function.}
We construct a spatio-temporal reward function to encourage the robot to grasp the target item or those in its near vicinity. The reward function $r(s_t, s_{t+1}, a_t)$ is 1 if the robot grasps the target object;  $\max{(\frac{\varrho}{||\mathbf{p}_t - \mathbf{g}_t||},1)}$ if it grasps another item; and 0 otherwise. \textcolor{red}{$\varrho$ is chosen based on the resolution of RFID positioning to provide the maximum reward when the grasp point is closest to the RFID position.}\footnote{ \textcolor{red}{In our implementation, $\varrho$ is set to 0.007.}}. Since RF perception tracks the RFID's location, it can determine whenever the grasp is successful (it is picked up).

\vspace{0.05in}
\noindent
\textbf{RF-based Attention.} 
\name\ incorporates RF-based attention through two main strategies (and at three layers):
\begin{itemize}
    \item \textit{RF-based Binary Mask.} The RGB and depth heightmaps\footnote{Heightmaps are computed by extracting 3D point cloud from RGB-D images and projecting the images orthographically, parallel to the table top.
    %The RGB and depth heightmap represent color and height from tabletop respectively.
    } are cropped to a square around the RFID's location\footnote{\textcolor{red}{The square is 11cm$\times$11cm in our implementation}}. This pre-processing attention mechanism allows the network to focus on the vicinity of the target object and compute the affordance map with higher resolution and/or less computational complexity. 
    \item \textit{RF Kernel.} The RFID location is also used to construct an RF kernel, a 2D Gaussian centered around $\mathbf{p}$, whose standard deviation accounts for RF localization errors. The kernel is fed to the network, and is multiplied by DQN's last layer to compute the final affordance map. This increases the probability of grasping the target item. %We note that the multiplication by the kernel at the output is only used in testing but not in training, as it yielded better results.
    %\item \textit{Post-Processing Attention.}
\end{itemize}

\name\ uses the above RF attention mechanisms to extend a state-of-the-art deep-reinforcement learning grasping network~\cite{PushGrasp}, as shown in Fig.~\ref{fig:net}. It consists of two 121-layer DenseNets: the first takes as input three channels of cropped RGB heightmaps; the second's input is the RF kernel plus two copies of cropped depth heightmap. To discover optimal grasping affordances, the inputs are rotated in 16 directions and fed separately to the network. Then, the outputs of both streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. The output contains 16 maps for grasp, from which \name\ chooses the position and rotation with highest probability of success.

\vspace{0.05in}
\noindent
\textbf{Training Details.} 
We use Huber loss function for training our network to reduce sensitivity to outliers.  The DenseNet initial weights were taken from the pre-trained model in \cite{PushGrasp}, and fine-tuned by training for 500 iterations in simulation. The gradient is only backpropagated through the pixel of affordance map that we executed grasping according to its predicted value. The network is trained by stochastic gradient descent with learning rates  $10^{-4}$, momentum  $0.9$, and weight decay  $2^{-5}$. The reward discount factor is 0.2.
% $$ \delta_i = {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i) $$
% $$L_i = \begin{cases} 
% \frac{1}{2}( \delta_i)^2, \text{   If } | \delta_i| < 1\\
% |  \delta_i | - \frac{1}{2}, \text{ Otherwise}
% \end{cases}
% $$ 

In training, we used prioritized experience replay~\cite{prioritized} to improve sample efficiency and stability. 
%In experience replay, a fixed number of most recent experiences are saved, and the network is trained on a batch of a chosen set of transitions. 
We define threshold $\rho_i=0.05 + \min(0.05\times\text{\#iteration},4)$, and performed stochastic rank-based prioritization among experiences with rewards $\ge\rho_i$. Prioritization is estimated by a power-law distribution. 












==> learning.tex <==
We use an off-policy Q-learning approach to find an optimal policy maximizing the expected sum of future rewards. Rewards are calculated from function  $\small{R_{a_t}(s_t, s_{t+1},\dist}\footnotesize{(\text{action},\text{target}))}$.  Future reward with a $\gamma$-discount sum is given by: 
$$R=\sum_{i=t}^{\infty}\gamma R_{a_i}(s_i, s_{i+1}, \dist(\text{action}_i,\text{target}_i))$$
where $a_i$ is the type of action: (push/grasp, $action_i$). $action_i$ refers to the position that action was performed, and $target_i$ is the position of the localized object. Reward function rewards successful grasp near the item of interest ($\text{target}$) more than successful grasps of items which are far from the item of interest by multiplying the function by $\frac{\beta}{\text{Euclidean distance}^2}$ where $\beta$ is a constant. The maximum reward, is given to grasping the item of interest. Other successful grasps are rewarded depending on their distance to the object of interest. \\
The problem is to maximize the action-value function $Q(s_i,a_i)$ that estimates the expected reward of taking the action $a_i$ at the state of $s_i$. Q-learning can be defined simply as : 
 
 $$ Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha [ R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$$

In this case, Q approximates the optimal action-value function. The aim of the network is to minimize $ \delta_t = [R_{t+1} +\gamma \max_{a} Q(s_{t+1},a) - Q(s_t,a_t)]$
\subsection{States}
Each state consist of a RGB height-map, a depth height-map, and a probability map of objects' location. The probability map of location comes from the exploration phase. We get the RGB-D data from a wrist-mounted camera, make a point cloud form it, and project it to a height-map whose boundaries are defined by the work space limit of setup. The working space is 44cm$\times$44cm.\\
For each state, the inputs are rotated to produce 16 different orientations. These 16 different groups of inputs are fed separately to the grasp (push) network, producing 16 outputs. The output that contains the pixel with highest value of all shows the proper gripper direction for performing grasp (push).

\subsection{Actions}
\subsubsection{Pushing}
The output of the push network is 16 probability maps. The push starting point is the pixel with highest probability of successful push in one of the 16 outputs (aka directions). A 10-cm push is executed from the chosen point in one of the 16 directions. The robot gets the height of the action-point from depth height-map, and pushes the blocks by the finger tips of the closed gripper.
\subsubsection{Grasping}
Similar to the push network, the grasp network output is 16 probability maps. The point with the highest value represents the middle point of gripper for performing grasping action. The orientations of the gripper is also defined by one of the 16 orientations. The robot gets the height of the action-point from depth height-map, moves the gripper above the intended action-point, lowers the gripper to put the block between its fingers, and then closes the gripper.

\subsection{Network Architecture}

For each push and grasp, we trained a separate feed-forward fully convolutional networks (FCNs) that takes the state representatives: RGB height-map, depth height-map, and probability map of object location. The output of each network is pixel-wise map of Q values that is mapped to the work space in post-processing. Each FCN has two input streams: 1) three channels of RGB height-map data, 2) three channels consisting of 2 copies of the depth height-map, and a location probability map. \\
Each input stream goes through a 121-layer DenseNet whose initial weights were taken from the pre-trained model on ImageNet. Then, the output of two streams are concatenated along channels. Two convolution layers with kernel size of $1\times1$ come after, producing the 2D map of the Q function estimation. In the last stage, the probability map of location is dotted with the output of last CNN layer to focus the attention of the network on the object. we multiply the grasping Q-values by a Gaussian mask centered at the most probable object location. In this case, the probability of grasping the item of interest increases.\\
To learn orientation's influence on the grasp and push success, network inputs are rotated into 16 directions and fed separately to the network. The output contains 16 maps for grasp and 16 maps for push, from which we choose the pixel and action with highest probability of success.

\begin{figure}
\centering
\includegraphics[scale=0.12]{Net.002.jpeg}
\caption{Network Architecture} \label{fig1}
\end{figure}

\subsection{Reward}
We reward the network based on the quality of its performance. The highest reward is given to grasping the item of interest ($R_{g_\text{intended}}=5$). Objects, which are very close to the object of interest, are considered indistinguishable from the intended object, or necessary to grasp to pave the way for grasping the intended object. Consequently, we reward these successful grasps four units ($R_{g_\text{very close}}=4$).\\
Other successful grasps are rewarded depending on their distance from the targeted item.  $$R_{grasp}=\frac{3.5\times 10^{-3}}{\text{Euclidean distance(action point, targeted item)}^2}$$\\
A Pushing network is rewarded if it induces enough changes in the work space (The number of pixels in depth height-map whose value changed exceeds a certain threshold). It also benefits from the discounted reward of future successful grasps.


\subsection{Training Details}
We used Huber loss function for training our network to reduce sensitivity to outliers.
$$\Loss_i = \begin{cases} 
\frac{1}{2}({R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i))^2, if |{R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i)| < 1\\
| {R^{\theta_i^-}}_{i+1} +\gamma \max_{a} Q^{\theta_i^-}(s_{i+1},a) - Q^{\theta_i^+}(s_i,a_i)| - \frac{1}{2}, Otherwise
\end{cases}
$$ 
We pass gradient only through the network that had the highest success probability, which the system performed according to its output. The networks were trained by stochastic gradient descent with learning rates of $10^{-4}$, momentum of $0.9$, and weight decay of $2^{-5}$. In simulation, We trained the system by dropping objects from random locations above the working space. The objects in simulations were 3D toy blocks models. 

\subsubsection{Experience Replay}
We use a modified experience replay in the training process to bias the network toward grasps in the vicinity of object location. In every iteration a threshold is defined   $\text{tr}=0.05 + \min(0.001\times\text{\#iteration},4)$. Among those action with a reward above the threshold, a stochastic rank-based prioritization is performed. The prioritization is estimated by a power-law distribution. The future discount is set to be $0.2$.




==> overview-1.tex <==

\section{Overview}

We consider the generalized mechanical search problem where a robot needs to extract target object(s) that is/are behind occlusions and/or under a pile. 

\fa{The overview section still needs to be massaged a bit to highlight high-level problem and the two key novel components.}

\name\ uses RGBD input to create a 3D model of the environment and extract occluded regions, and it plugs the location of the RFID-tagged object into the 3D model. If the object isn't within reach, it performs RF-guided active exploration and trajectory optimization to obtain a better view of the object by maneuvering around obstacles and closer to the object of interest. Once the target object is within reach (stopping criterion), the system moves to the grasping phase. Here, it applies RF-based attention to the RGBD information and relies on a model-free deep-reinforcement network to discover optimal grasping affordances. \name\ closes uses the RFID's location to close the loop on the grasping task and determine whether it has been successful or whether it needs to make another grasping attempt.

==> related-1.tex <==
\section{Background and Related Work}\label{sec:related}

Past works falls into several categories: a) Robotic navigation and localization using RFIDs, b) Vision based robotic grasping \\

a) \textbf{Robotic navigation and localization using RFIDs:} Radio frequency identification (RFID) is a relatively old technology, and recent advancements in chip manufacturing technology has made passive RFID tags available for 3 cent each. When these battery-less chips are interrogated wirelessly by an RFID reader, they harvest energy from transmitted RF waves by reader, and respond with their 96 bits identifier. Since RF signals can traverse walls and obstacles, RFID tags can be read in occlusion and NLOS scenarios. For instance, Ultra-High Frequency (UHF) RFID tags can communicate with a reader 6-8 meters away in NLOS. RFID tags has enabled applications such as item-level tagging, ID cards for access control, and contact-less payment systems. [RFID]

Researcher has recognized the potentials of using RFID for robotic applications. The wast majority of them focused on robotic navigation and localization. In early works on robot navigation, RFIDs were put on specific landmarks in the environment or followed a predefined pattern. Robot, knowing in advance the location of tags, navigates itself in in-door environment while carrying a RFID reader. It continuously senses the environment by reading the RFIDs to locate itself, or uses RFID tag data to plan its future steps. These previous methods require altering the environment and attaching tags in specific locations and have accuracies of fraction of a meter to a meter \cite{T4,T11,T12,T13,T14,T22,T34,T35}.

Some other similar approaches studied the problem of navigating to a specific object by sensing the RFID and Received Signal Strength (RSS) by moving toward the strong signal. These methods, while  enabling fuzzy localization, cannot be used for grasping \cite{T4,T5,T21,T29,T33}.
4
Some of the previous proposals tried to perform grasping using RSS in which a robot samples the environment when trying to approach the item of interest by moving toward the direction of strong signal. However, methods relying on RSS has been shown to have multi-meter accuracies as RSS needs a clear LOS. These methods cannot remove clutter to reach and grasp an occluded object; as a result, they require the object to be isolated from other objects and be in clear LOS. Consequently, none of theses methods can enable semantic grasping of occluded objects in cluttered environment \cite{T25,T28,T31}. 

While \name\ shares the vision of theses early systems, it is built on more recent advances in RFID positioning to develop techniques that enable grasping invisible object in unstructured clutter. Fine-grained RFID localization methods such as TurboTrack \cite{TurboTrack} and RFind \cite{RFind} focus on tracking RFID tags and have decimeter and centimeter positioning accuracy. Although these methods can localize and track an occluded RFID tagged item, they are unable to find a way to reach the occluded object and grasp it.

Two recent projects, RF-Compass \cite{RFCompass} and MobiTagbot \cite{MobiTag}, tried to enable more higher level tasks such as grasping and sorting. However, MobiTagbot \cite{MobiTag} can not perform object manipulation and its abilities are limited to checking the order of RFID tagged objects. RF-Compass \cite{RFCompass} can only works with large objects that one can put multiple RFID tags on them to reach the necessary accuracy for grasping. Therefore, their system cannot demonstrate grasping in practical scenarios.

Our system is built on these past works. It fuses the information provided by RFID tags localization with vision to enable robust servoing and grasping fully occluded objects in unstructured clutter. 

b)\textbf{Vision Based Robotic Grasping:} 
\name\ is also related to vision-based robotic grasping systems and semantic grasping, and directly builds on this area of past research \cite{PushGrasp,semantic1,MVPclutter,rpp}. Some of previous works, plans the robots actions and trajectory in order to relocated objects in the environment to generate a line of sight to item of interest  \cite{T36,T37,T38,T39,T47}, or performs grasping using tactile sensor \cite{T46}. However, these systems completely fail to plan a meaningful trajectory to reach an item in full occlusion and to perform semantic grasping. In contrary to previous works, \name\ can explore the environment to grasp a requested fully-occluded object. \name\ is built on prior work on active exploration, where the goal is to optimize the trajectory and explore the environment to minimize occlusions \cite{BerkeleyGraspOcclusion}. This past work is not able to perform semantic grasping, because it relies only on vision and cannot locate invisible objects. \name\ directly builds on this work and extends it to enable semantic grasping of invisible objects. 

==> related-2.tex <==
\section{Background \& Related Work}

\noindent
\textit{RFIDs and their Applications in Robotics.} RFID is a relatively mature technology that was introduced around two decades ago, and it has seen widespread adoption by many industries as barcode replacement over the past few years in retail, manufacturing, and warehousing~\cite{RFIDmarket}. Today's UHF (Ultra-High Frequency) RFIDs cost as little as 3-cents and don't require any batteries. A wireless device called a reader can read and uniquely identify RFIDs from up to 9~m and through occlusions, and existing RFID readers can read thousands of tags per second~\cite{Imping}. 

The vast majority of early research on RFIDs focused on tag and protocol design, security, and cost reduction. Due to their widespread adoption, the past few years have seen significant advances in RFID localization technologies~\cite{PinIt,RFCompass,RFind,TurboTrack,MobiTag}. Rather than simply using RFID tags as identifiers, these technologies can also locate the tags in the environment for location-based services, such as finding misplaced items. Researchers have considered various positioning techniques including received signal strength (RSS), angle of arrival (AoA), and time-of-flight. Recent advances in RF perception have enabled state-of-the-art RFID positioning systems to achieve centimeter-scale positioning even in cluttered and occluded environments. Our work builds directly on this line of work, and fuses it with vision to enable novel robotic tasks. We refer the interested reader to~\cite{TurboTrack} for a more detailed overview of the progress in RFID-positioning systems.

Recognizing the potential use of RFIDs in robotics, various researchers have also developed systems that leverage RFIDs as location markers to facilitate robotic navigation. Others have considered the use of RFIDs as markers to guide a mobile robot toward grasping; however, because RF signals are transparent to occlusions, these past systems could not tackle the mechanical search problem. Our work is similarly motivated to this line of work and demonstrates, for the first time how RF-visual information enables challenging robotic tasks like mechanical search.

\vspace{0.05in}
\noindent
\textit{Mechanical Search.}

\vspace{0.05in}
\noindent
\textit{Manipulation and Grasping in Clutter.}

==> related-3.tex <==
\vspace{-0.05in}
\section{Background \& Related Work}
\vspace{-0.05in}

\begin{figure}[t]
	\begin{center}
		\includegraphics[width =0.42\textwidth]{Grasping_Paper/figures/rfid.jpeg}
		\caption{\textbf{RFID-based Perception}. \name\ uses a customized reader that can identify and accurately localize RFID-tagged objects through occlusions.}
		\label{fig:rfid}
	\end{center}
	\vspace{-0.15in}
\end{figure}

\begin{figure*}[thp]
	\begin{center}
		\includegraphics[width =\textwidth]{Grasping_Paper/figures/overview_new.jpeg}
		\vspace{-0.2in}
		\caption{\textbf{System Overview.} \name\ uses RGB-D to create a 3D model of the environment and extract occluded regions, and it plugs the location of the RFID-tagged object into it. If the object is behind obstacles, it performs RF-guided active exploration and trajectory optimization to obtain a better view of the object by maneuvering around obstacles. Once a stopping criterion is met, it proceeds to the grasping phase. Here, it applies RF-based attention to the RGB-D information and relies on a model-free deep-reinforcement network to discover optimal grasping affordances. \name\ uses the RFID's location to close the loop on the grasping task and determine whether it has been successful or whether it needs to make another grasping attempt.}
	%	Once a grasping attempt is  made, \name\ uses the RFID's location (obtained from its RF perception module) to close the loop and determine whether the object of interest has been grasped (i.e., if it moved with the robotic arm) or whether the system needs to make another grasping attempt.}
		\label{fig:overview}
	\end{center}
	\vspace{-0.15in}
\end{figure*}

\noindent
\textbf{RFIDs and their Applications in Robotics.}
%
RFID is a relatively mature technology that has seen widespread adoption by many industries as barcode replacement over the past few years in retail, manufacturing, and warehousing~\cite{RFIDmarket}. Today's UHF (Ultra-High Frequency) RFIDs cost as little as 3-cents and don't require any batteries. A wireless device called a reader can read and uniquely identify RFIDs from up to 9~m and through occlusions (as shown in Fig.~\ref{fig:rfid}), and existing RFID readers can read thousands of tags per second~\cite{Imping}. 

%The vast majority of early research on RFIDs focused on tag and protocol design, security, and cost reduction. 
Due to their widespread adoption, the past few years have seen significant advances in RFID localization technologies~\cite{PinIt,RFCompass,RFind,TurboTrack,MobiTag}. Rather than simply using RFIDs as identifiers, these technologies can also locate the tags in the environment % Researchers have considered various positioning techniques including received signal strength (RSS), angle of arrival (AoA), and time-of-flight. 
%Recent advances in RF perception have enabled state-of-the-art RFID positioning systems to achieve
with centimeter-scale precision even in cluttered and occluded settings. We build directly on this work, and fuse it with vision to enable novel robotic tasks. 
%We refer the interested reader to~\cite{TurboTrack} for a more detailed overview of the progress in RFID-positioning systems.

Recognizing the potential for RFIDs in robotics, researchers have developed systems that leverage RFIDs as location markers to facilitate navigation~\cite{navigation1,navigation2,navigation3} and to guide a mobile robot toward grasping~\cite{RFCompass,T25,T28,T31,MobiTag,RFIDfusion}; however, because occlusions are transparent to RF, these systems could not perceive them and perform decluttering or obstacle avoidance. \name\ extends this work and demonstrates, for the first time, how RF-visual fusion enables challenging tasks like mechanical search.

\vspace{0.05in}
\noindent
\textbf{Mechanical Search and Grasping in Clutter.}
%\vspace{-0.05in}
%Robotic grasping in clutter is an important problem that has different forms. 
%
Object manipulation in cluttered environments has received significant attention and achieved remarkable success via supervised and unsupervised methods~\cite{PushGrasp,MVPclutter,rpp,graspocclusion}.
%grasping all items in a pile through various methods including manipulating the environment (e.g., by pushing and singulation) or multi-view perception
%These systems have achieved remarkable results via .
Our work is motivated by a similar desire to grasp in clutter and builds on this line of work but focuses on the problem of grasping a specific target object rather than \textit{any} object or \textit{all} objects.

The problem of recognizing and locating target objects in occlusions has also received considerable attention~\cite{semantic1}. Different techniques have been proposed including perceptual completion~\cite{occlusionaware} as well as active and interactive perception where a camera is moved to a more desirable vantage point for recognizing an object of interest~\cite{activeperception1,activeperception2,interactiveperception}. In contrast to this past work, which requires a (partial) line-of-sight to the object to recognize it, our work uses RF perception to directly identify and locate objects directly through occlusions, and without requiring any prior training.


\name\ is most related to recent prior work on mechanical search, where the goal is to search for and grasp a target object that may be partially or fully occluded~\cite{BerkeleyGraspOcclusion,IROS2019Xray,ICRA2019search,T36}; this includes both one-shot and multi-step procedures for search and retrieval~\cite{graspinvisible,objectfinding,T37,T38,T39}. Unlike \name, this prior work first needs to search for the object to identify its location, which does not scale well with the number and size of piles, or the number of target objects; in contrast, by exploiting RF perception, \name\ can recognize and locate RFID-tagged objects to perform highly efficient active exploration and manipulation.

It is worth noting that our work is also related to prior research that can recognize occluded objects without line-of-sight through tactile sensing~\cite{tactilerecognition}. Unlike \name, this past work needs to already be in direct contact with the object. 

%It is also worth noting that X-ray can traverse occlusions but is undesirable due to its harmful ionizing radiations, and other technologies like millimeter-waves and THz have been demonstrated to operate through occlusions but also have limited skin depth.

==> results-1.tex <==
 
\begin{table*}[t]
\begin{center}
\begin{tabular}{ |p {3cm} |p {3cm} |p {3cm} |p {3cm} |p {3cm} |p {3cm} | } 
 \hline
  Avg Traveled Distance & Random Sampling & Active Exploration & Obstacle  Avoidance & \hspace{1cm} \name \hspace{1cm} \\ [2ex]
 \hline

 Scenario 1 & 3.5432 \pm 1.6691 & 1.9191 \pm 0.9938 & 0.6246 \pm 0.0162 & cell6 \\[1ex]
 Scenario 2&  1.6117 \pm 0.5797 & 1.6117 \pm 0.5797 & 0.6377 \pm 0.0809 & cell6 \\ [1ex]
 Scenario 3&  0.7686 \pm 0.2480 & 0.7686 \pm 0.2480 & 1.6237 \pm 1.6935 & cell6 \\ [1ex]
 Total &      2.1314 \pm 1.6162 & 1.4331 \pm 0.7826 & 1.0026 & cell6 \\ [1ex]
 \hline
\end{tabular}
\end{center}
\end{table*}

\section{Results}
We first evaluated \name’s performance quantitatively and analyze the results in terms of the traveled distance, completion rate, and grasp efficiency.

\textbf{(a) Average Traveled Distance:} 
We recorded the robot's end-effector position through each trial, then computed the average traveled distance of end-effector in every scenario for our system and the baselines. Since the RFID location information is used in our cost function, the robot is guided in the direction of the tagged object. This reduces the traveled distance and the time which is spent on executing exploration in the environment, searching for the tagged item. We had three scenarios with two occluded region ($M=2$) and 2,3, or 4 occlusion frontiers. We ran $\sim 3$ trials per system and scenarios.

PUT THE FIGURE, EXPLAIN THE TREND

\textbf{(b) Completion Rate:} 
We are interested in evaluating \name’s completion rate which indicates how often our system successfully explores the environment until there is a Line-Of-Sight to RFID-tagged object.
We put the robot in an initial pose where the wrist-mounted camera can see one or two occlusion frontier. As a result, there is one or more occluded regions in the robot's workspace. The robot arm explores the environment trying to minimize its cost function. 

PUT THE TABLE, EXPLAIN THE TREND

\textbf{(c) Grasp Efficiency:} is defined as $\frac{\text{\# tagged objects}}{\text{\#grasping action attempts}}$. This metric indicated how attention mechanisms can improve the system's performance by the average number of grasp attempts before the object of interest is finally grasped. To evaluate this metric, We put the robot in the position depicted in figure XXX with the camera looking at a cluttered environment with 30 randomly placed objects. The location of the tagged object is published on a ROS topic and the grasping is initiated by focusing attention to the tagged item location. We performed XXX of trials with random position and orientation of block toys. The baseline, VPG, is tested in a similar scenario without the location information.

PUT THE FIGURE, EXPLAIN THE TREND





==> results-2.tex <==
 
\section{Results}

%\fa{Section needs smoothing English.}

%We first evaluated \name’s performance qualitatively and then quantitatively. We analyzed the quantitative results in terms of the traveled distance, completion rate, and grasp efficiency.

\subsection{Performance Results}

\begin{figure}[t]
\begin{tikzpicture}
\begin{axis}[ymin=0, ymax=5, height=5cm, width=0.45\textwidth, 
  ytick={0,1,...,5}, ytick align=outside, ytick pos=left,
  xtick={0,1,...,6}, xtick align=outside, xtick pos=left,
  xlabel= \footnotesize{\# occlusions},
  ylabel={\footnotesize{Avg. Traveled Distance [m]}},
  legend pos=north west,
  legend style={draw=none},
  yticklabel style={font=\small},
  xticklabel style={font=\small}]
\addplot+[
  blue, mark options={blue, scale=0.75}, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.95,    0.38
    1,  1.80,    0.68
    2,  2.43,    0.77
    3,  3.2,    1.57
    4,  3.42,    1.1
    5,  2.93,    0.96
    
};
\addplot+[
  red, mark options={red, scale=0.75},
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.96,    0.44
    1,  1.42,    0.22
    2,  1.40,    0.26
    3,  1.8,     0.37
    4,  1.82,    0.54
    5,  1.57,    0.45
    
};
\addlegendentry{\footnotesize{Baseline}}
\addlegendentry{\footnotesize{\name}}
\end{axis}
\end{tikzpicture}

\noindent
\caption{\textbf{Average Traveled Distance.} The figure plots the average traveled distance of the gripper's tip for baseline (blue) and \name\ (red) in scenarios with 0-5 occlusion. The error bars represent the standard deviation for traveled distance in each scenario.}
\label{fig:travel}
\end{figure}

\begin{figure*}[t]
	\centering
	\begin{tabular}{ccc}
%	\begin{minipage}{.63\columnwidth}
%		\centering
		\epsfig{file=res1.jpeg,width=0.3\textwidth}
		&
		\epsfig{file=res2.jpeg,width=0.3\textwidth}
		&
		\epsfig{file=res3.jpeg,width=0.3\textwidth}
		\\
		
		\footnotesize{(a) Clutter scenario}
		&
		\footnotesize{(b) Multi-obstacle and clutter scenario.  }
		&
		\footnotesize{(c) Sorting Scenario} \vspace{0.2cm}
		\\
\end{tabular}
\caption{\textbf{Generalized Mechanical Search.} We show 3 challenging tasks which the baseline cannot perform. (a) The first is grasping from under clutter. (b) The second is grasping in the presence of multiple piles and obstacles. (c) The third is a prioritized sorting task.}
\label{fig:res-qual-fig}
\end{figure*}

We evaluated the baseline and our system quantitatively in 6  more scenarios with 0-5 occlusions and 1-15 objects. The robot arm is placed in a similar initial position in each trials. In five of theses scenarios, there are 1-5 separated regions of workspace hidden from the wrist-mounted camera, and the item of interest is not in line of sight of the camera in these 5 scenarios. In the scenario with no occlusion, there is no need for exploration since there is no occlusion in the work space as the item of interest is in the line-of-sight of the wrist mounted camera. 

\noindent
\textbf{(a) Traveled Distance:} 
We recorded the robot's end-effector position and computed the average traveled distance of end-effector in every scenario for our system and the baseline. We had six scenarios with 0-5 occluded region ($M=0-5$) and ran $\sim 8-12$ trials per system and scenarios. 
We put the robot in an initial pose where the wrist-mounted camera can partially see a frontier. As a result, there is initially one or more occluded regions in the robot's workspace. It will find the other frontiers and occluded regions as it explores the environment to minimize its cost function. 

Figure \ref{fig:travel} plots the average traveled distance of gripper tip in each of the scenarios for both \name\ and the baseline. Our results show that \name\ travels shorter distances to grasp the requested item. The \name 's traveled distance is significantly lower than that of baseline in more complex scenarios with multiple occlusions. The robot is guided in the direction of the tagged object because the RFID tagged item location is used in our cost function. It reduces the traveled distance and the time which is spent on executing exploration in the environment searching for the tagged item. All the occluded regions are positioned in robots workspace and within its physical reach. Further, we note that the plots pleautu as the workspace of robot is limited by its arm size and mobility. 

\noindent
\textbf{(b) Task Completion Rate:}
We are interested in evaluating \name’s completion rate which indicates how often our system successfully explores the environment until there is a Line-Of-Sight to RFID-tagged object, and successfully performs grasping. For a trial to be considered completed, the system should find a line of sight to the item within 5 meters of traveled distance in exploration phase, and a successful grasp should happen within 10  grasp attempts. The experiments are the same as ones carried out for average traveled distance.
Table.\ref{tabCompletion} shows both \name\ and baseline's performance. \name\  was able to complete the task in 54 out of 54 trials, while the baseline were not able to complete the task in 8 out of 53 trials. The baseline completion rate decreases as the number of occlusions and complexity in experiments increases.

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lbababa}

& \multicolumn{6}{c}{\textbf{Scenario (M=\#occlusions, N=\#objects)}}\\
\cmidrule{2-7}
\textbf{System}& M=0 N=5 & M=1 N=1 & M=2 N=5 & M=3 N=10 & M=4 N=13 & M=5 N=15\\
\hline
Baseline &    $10_{/10}$  & $10_{/10}$ & $10_{/10}$  & $8_{/10}$  & $7_{/10}$  & $8_{/11}$  \\
RF-Grasp &    $10_{/10}$  &   $10_{/10}$   &  $10_{/10}$ &    $10_{/10}$ &  $10_{/10}$  &  $10_{/10}$ \\
\end{tabular}
\caption{\textbf{Completion rate.} In each scenario, M denotes number of occlusions, and N represents number of blocks. Baseline and \name\ were tested in 6 scenarios as presented above. The numbers are the number of \textit{successful} trials and the subscripts are the \textit{total} number of trials for the system in that scenario. }
\label{tabCompletion}
\end{table}

% \begin{table*}[h]
%     \begin{center}
%     \begin{tabular}{ |c|c|c|c|c|c|c| } 
%      \hline
%       \name & no occlusions & 1 occlusions & 2 occlusions & 3 occlusions & 4 occlusions & 5 occlusions\\ [1ex]
%      \hline
%      Total trials     &  5  &  9 &  10 & 11 & 10 & 9\\[1ex]
%      Successful trials & 5  &  9 &  10 & 11 & 10 & 9\\[1ex]
%      \hline
%      \hline
%      Baseline & no occlusions & 1 occlusions & 2 occlusions & 3 occlusions & 4 occlusions & 5 occlusions\\ [1ex]
%      \hline
%      Total trials &      5  & 9 & 8 &  9  &  10  & 12    \\[1ex]
%      Successful trials & 5  & 9 & 8 &  7  &  7  &  9  \\[1ex]
%      \hline
%     \end{tabular}
%     \end{center}
%     \label{tab:tab2}
%     \caption{\textbf{Completion Rate.} The table shows the total number of trials and successful trial in each scenario for \name\ and the baseline.}
% \end{table*}


% \begin{table*}[h]
% \begin{center}
% \begin{tabular}{|l||*{6}{c}}
% \backslashbox{System}{Scenario}
% & \rotatebox[origin=c]{60}{0 occlusion} & \rotatebox[origin=c]{60}{1 occlusion} & 2 & 3 & 4 & 5 \\\hline
% Baseline &&&&&&\\\hline
% \name\ &&&&&&\\\hline
% \end{tabular}
% \end{center}
% \end{table*}


% \begin{table*}[h]
% \begin{tabular}{|p{1.25cm}|p{0.01cm}p{0.5cm}p{0.01cm}p{0.5cm}p{0.01cm}p{0.5cm}p{0.01cm}p{0.5cm}p{0.01cm}p{0.5cm}p{0.01cm}p{0.5cm}|}
% &
% \begin{rotate}{60} 0 occlusion \end{rotate}&
% \begin{rotate}{60} \& 5 objects \end{rotate}&
% \begin{rotate}{60} 1 occlusion \end{rotate}&
% \begin{rotate}{60} \& 1 object \end{rotate}&
% \begin{rotate}{60} 2 occlusions \end{rotate}&
% \begin{rotate}{60} \& 5 objects \end{rotate}&
% \begin{rotate}{60} 3 occlusion \end{rotate}&
% \begin{rotate}{60} \& 10 objects \end{rotate}&
% \begin{rotate}{60} 4 occlusions \end{rotate}&
% \begin{rotate}{60} \& 13 objects \end{rotate}&
% \begin{rotate}{60} 5 occlusions \end{rotate}&
% \begin{rotate}{60} \& 15 objects \end{rotate}\\\hline
% baseline &    0  &&  2   && 4 &&   0 && 2  && 4 &\\ \hline
% \name\   &    0  &&  2   && 4 &&   0 && 2  && 4 & \\ \hline
% \end{tabular}
% \end{table*}


%\textbf{(b) Grasp Efficiency:} is defined as $\frac{\text{\# tagged objects}}{\text{\#grasping action attempts}}$. This metric indicated attention mechanisms performance since it gives the average number of grasp attempts before the object of interest is finally grasped. 

\subsection{Generalized Mechanical Search}

We have tested \name\ in several scenarios to show it is capable of grasping the requested item in full occlusion and clutter where it is impossible for other state of the art systems to perform. 

We first evaluate our system qualitatively in challenging scenarios where there is no baseline capable of completing the task. First, in a cluttered scenario, we randomly placed more than 20 blocks along with tagged item in the workspace and covered them with package filling sheets. Because of the cover, there is no line of sight to the item from wrist-mounted camera or antennas to the item. Secondly, we tested \name\ in a cluttered single obstacle scenario, where there is an obstacle in the workspace that occludes an area from the wrist-camera. The item of interest along with 5 random block are placed in the initially occluded region. These items are also covered by package filling sheets, and there is no line of sight to the item. Lastly, we tested \name\ in a cluttered multi-obstacle scenario, where there are two boxes which occluded two regions from camera, and we put the tagged item in one of the boxes. We also put 5 more items in each box and covered them with package filling sheets. Similarly, there is no line of sight to object from wrist-mounted camera or antennas to objects.

In the clutter scenario, we randomly placed more than 20 blocks next to a RFID-tagged item and covered them with paper cover as depicted in Figure \ref{fig:res-qual-fig}. Initially, there is no line of sight from camera or antennas to the tagged item. \name\ localizes the RFID and move directly above the covered item. The camera RGB-D data is fed to the grasping network and an action point and gripper orientation is chosen according to estimated Q-values. As the robot picks up the cover in step (c), it realizes it has picked up a clutter since the RFID location has not change. It puts the clutter aside and goes back above the tagged item location as depicted in step (d). The new RGB-D data is fed to grasping network, and \name\ tries grasping again. This time the RFID location changes with robot's end-effector movements, and \name\ confirms it has grasped the requested item. We tested \name\ in this scenario for 5 times. The average travelled distance was 2.68m with standard deviation of 0.98. \name\ was successful in all 5 trials.

In the cluttered multi-obstacle scenario, there are two boxes  occluding two regions from camera. We put 5 items in each box, and one tagged item in one of the boxes. All items are covered under clutter with paper covers, as depicted in Figure \ref{fig:intro-fig}. After RFID's location is found, \name\ realizes there is no line of sight to the tagged item location. So, the robot explores the environment using its RF-guided optimization. After several iterations of the exploration, \name's exploration stopping criteria is met, and it moves to the grasping phase. If the tagged item location changes in the middle of process, \name\ updates the RFID location instantly and tries grasping again. We tested \name\ in this scenario for 3 times. The average travelled distance was 4.13 with standard deviation of 1.91. \name\ was successful in all 3 trials.

\fa{Failure modes? Limitations}


% \begin{figure*}
% 	\centering
% 	\begin{tabular}{ccc}
% %	\begin{minipage}{.63\columnwidth}
% %		\centering
% 		\epsfig{file=res_1p_1.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_2.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_3.jpeg,width=0.3\textwidth}
% 		\\
		
% 		\footnotesize{(a) Localization through obstacles}
% 		&
% 		\footnotesize{(b) Moving directly  above  the  item.  }
% 		&
% 		\footnotesize{(c) Decluttering} \vspace{0.2cm}
% 		\\
		
% 		\epsfig{file=res_1p_4.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_5.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_6.jpeg,width=0.3\textwidth}
% 		\\
		
% 		\footnotesize{(d) Moving  directly  above  the  item.  }
% 		&
% 		\footnotesize{(e) Grasping attempt}
% 		&
% 		\footnotesize{(f)Grasp success confirmation}
% 		\\ 
% 		&
% 		&
% 		\footnotesize{by RFID location change}
% 		\\ 
% \end{tabular}
% \caption {\textbf{Scenario 1: Clutter} a) In the initial state, an RFID tagged item is occluded under clutter. There is no line-of-sight to the item from camera or antennas. b) The robot moves directly above the item. c) The robot grasps an item. However, since the RFID location doesn't change, it concludes that the recently grasped item is a clutter.  d)  The robot returns directly above the item to try again. e) \name\ attempts grasping another item. f) The robot confirms that it grasped the item of interest because the RFID location changes accordingly.}
% \label{fig:res-qual-fig}
% \end{figure*}
% \vspace{0.3cm}
% % \begin{figure*}
% % 	\centering
% % 	\begin{tabular}{cccc}
% % %	\begin{minipage}{.63\columnwidth}
% % %		\centering
% % 		\epsfig{file=res_1p_1.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_2.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_3.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_4.jpeg,width=0.23\textwidth}
% % 		\\
		
% % 		\footnotesize{(a)}
% % 		&
% % 		\footnotesize{(b) }
% % 		&
% % 		\footnotesize{(c)}  
% % 		& 
% % 		\footnotesize{(d)} 
% % 		\\
		
% % 		\epsfig{file=res_3_5.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_6.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_7.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_8.jpeg,width=0.23\textwidth}
% % 		\\
		
% % 		\footnotesize{(e)}
% % 		&
% % 		\footnotesize{(f)}
% % 		&
% % 		\footnotesize{(g)}
% % 		&
% % 	    \footnotesize{(h)}
% % 		\\
% % \end{tabular}
% % \caption {\textbf{Multi-Obstacle \& Clutter Scenario. } a) In the initial state, an RFID tagged item is occluded under clutter inside one of the boxes. There is no line-of-sight to the item from camera or antennas. b) The robot moves directly above the item. d) The robot grasps an item. However, since the RFID location doesn't change, it concludes that the recently grasped item is a clutter. e) The robot removes more clutter.  
% %  f) Robot tries grasping the tagged item. However, it misses the item as the box slippes in the process and changes the item location. e) \name\ updates the tagged item location, and tries grasping again. g) The robot confirms that it grasped the item of interest because the RFID location changes with accordingly.}
% % \label{fig:res-qual-fig}
% % \end{figure*}



==> results-3.tex <==
 
\section{Results}

%\fa{Section needs smoothing English.}

%We first evaluated \name’s performance qualitatively and then quantitatively. We analyzed the quantitative results in terms of the traveled distance, completion rate, and grasp efficiency.

\subsection{Performance Results}

\begin{figure}[t]
\begin{tikzpicture}
\begin{axis}[ymin=0, ymax=5, height=5cm, width=0.45\textwidth, 
  ytick={0,1,...,5}, ytick align=outside, ytick pos=left,
  xtick={0,1,...,6}, xtick align=outside, xtick pos=left,
  xlabel= \footnotesize{\# occlusions},
  ylabel={\footnotesize{Avg. Traveled Distance [m]}},
  legend pos=north west,
  legend style={draw=none},
  yticklabel style={font=\small},
  xticklabel style={font=\small}]
\addplot+[
  blue, mark options={blue, scale=0.75}, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.95,    0.38
    1,  1.80,    0.68
    2,  2.43,    0.77
    3,  3.2,    1.57
    4,  3.42,    1.1
    5,  2.93,    0.96
    
};
\addplot+[
  red, mark options={red, scale=0.75},
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.96,    0.44
    1,  1.42,    0.22
    2,  1.40,    0.26
    3,  1.8,     0.37
    4,  1.82,    0.54
    5,  1.57,    0.45
    
};
\addlegendentry{\footnotesize{Baseline}}
\addlegendentry{\footnotesize{\name}}
\end{axis}
\end{tikzpicture}

\noindent
\caption{\textbf{Average Traveled Distance.} The figure plots the average traveled distance of the gripper's tip for baseline (blue) and \name\ (red) in scenarios with 0-5 occlusion. The error bars represent the standard deviation for traveled distance in each scenario.}
\label{fig:travel}
\end{figure}

\begin{figure*}[t]
	\centering
	\begin{tabular}{ccc}
%	\begin{minipage}{.63\columnwidth}
%		\centering
		\epsfig{file=res1.jpeg,width=0.3\textwidth}
		&
		\epsfig{file=res2.jpeg,width=0.3\textwidth}
		&
		\epsfig{file=res3.jpeg,width=0.3\textwidth}
		\\
		
		\footnotesize{(a) Clutter scenario}
		&
		\footnotesize{(b) Multi-obstacle and clutter scenario.  }
		&
		\footnotesize{(c) Sorting Scenario} \vspace{0.2cm}
		\\
\end{tabular}
\caption{\textbf{Generalized Mechanical Search.} We show 3 challenging tasks which the baseline cannot perform. (a) The first is grasping from under clutter. (b) The second is grasping in the presence of multiple piles and obstacles. (c) The third is a prioritized sorting task.}
\label{fig:res-qual-fig}
\end{figure*}

We evaluated \name\ and the baseline quantitatively by varying the number of large occlusions and distractor objects in the environment. Each large occlusions $M$ hides a different region of the workspace from the wrist-mounted camera. In all except $M=0$, the target object is not in the line-of-sight of the camera.  In the scenario with no occlusion, there is no need for exploration since there is no occlusion in the work space as the item of interest is in the line-of-sight of the wrist mounted camera. We also vary the initial position of the robot across experimental trials, but ensure that the baseline and \name\ share the same initial position.

\noindent
\textbf{(a) Traveled Distance:} 
We recorded the robot's end-effector position and computed the average traveled distance of end-effector in every scenario for our system and the baseline. We had six scenarios with 0-5 occluded regions ($M=0-5$) (each with 1-15 distractor objects) and ran $\sim 10-11$ trials per system and scenarios. 
We placed the robot in an initial pose where the wrist-mounted camera can partially see a frontier. As a result, there is initially one or more occluded regions in the robot's workspace. The robot will find the other frontiers and occluded regions as it explores the environment to minimize its cost function. 

Figure~\ref{fig:travel} plots the average traveled distance of gripper tip in each of the scenarios for both \name\ and the baseline. For all except $M=0$, our results show that \name\ travels shorter distances (by up to 50\%) to grasp the target item; moreover, \name\ significantly outperforms the baseline as the number of occlusions increases. This result is excepted because \name\ is guided by the RFID's location (in the cost function) and moves in the direction of the RFID-tagged object. This reduces the traveled distance and the time spent on exploring the environment searching for the tagged item in comparison to the baseline. Note that the average traveled distance plateaus after four occlusions because the workspace of the robot is limited by its arm size and mobility (and all occluded regions are within that workspace). This result demonstrates the value of \name's first core component (RF-visual servoing) in enabling efficient exploration and trajectory optimization.

\noindent
\textbf{(b) Task Completion Rate:}
Next, we are interested in evaluating \name’s completion rate across the same experiments described above. A task is considered complete if the robot successfully maneuvers toward the target object and picks it up.  For a trial to be considered successful, the system should find a line of sight to the item within 5 meters of traveled distance in the exploration phase, and a successful grasp should be completed within 10 grasping attempts. 
%We use the same experimental trials performed above experiments are the same as ones carried out for average traveled distance.

Table~\ref{tabCompletion} shows the results. \name\ was able to complete the task in 60 out of 60 trials, while the baseline was unable to complete the task in 8 out of 61 trials. The baseline completion rate decreases as the number of occlusions and complexity in experiments increases.

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lbababa}

& \multicolumn{6}{c}{\textbf{Scenario (M=\#occlusions, N=\#objects)}}\\
\cmidrule{2-7}
\textbf{System}& M=0 N=5 & M=1 N=1 & M=2 N=5 & M=3 N=10 & M=4 N=13 & M=5 N=15\\
\hline
Baseline &    $10_{/10}$  & $10_{/10}$ & $10_{/10}$  & $8_{/10}$  & $7_{/10}$  & $8_{/11}$  \\
RF-Grasp &    $10_{/10}$  &   $10_{/10}$   &  $10_{/10}$ &    $10_{/10}$ &  $10_{/10}$  &  $10_{/10}$ \\
\end{tabular}
\caption{\textbf{Completion rate.} In each scenario, M denotes number of occlusions, N number of blocks. The results are reported as the number of successfully completed trials out of the total number of experimental trials.}
\label{tabCompletion}
\end{table}

\subsection{Generalized Mechanical Search}

Next, we show that \name\ can also successfully grasp fully-occluded objects, in challenging scenarios where the state-of-the-art baseline is not capable of completing. We consider three such scenarios, shown in Fig.~\ref{fig:res-qual-fig}.

\noindent
\textbf{Scenario 1: Under Clutter:} First, in a cluttered scenario, we randomly placed more than 20 distractor objects along with tagged item in the workspace and covered them with package filling sheets (as shown in Fig.~\ref{fig:res-qual-fig}(a)).. Because of the cover, there is no line-of-sight to the item from wrist-mounted camera or antennas to the item. \name\ localizes the RFID and moves directly above the covered item. The camera RGB-D data is fed to the grasping network and an action point and gripper orientation is chosen according to estimated Q-values. Because the target itself is occluded, the robot picks up the cover in step,\textcolor{red}{ha?!} and realizes it hasn't picked the target object since the RFID location has not change. It puts the clutter aside and goes back above the tagged item location. The new RGB-D data is fed to grasping network, and \name\ tries grasping again. This time the RFID location changes with robot's end-effector movements, and \name\ confirms it has grasped the requested item. We tested \name\ in this scenario for 5 times. The average travelled distance was 2.68m with standard deviation of 0.98. \name\ was successful in all 5 trials.

It is worth noting that, in contrast to \name, our baseline is incapable of successfully completing such a task because the green-tagged object would remain fully-occluded; thus, neither its exploration phase would be completed nor the grasping phase can efficiently pick up the object of interest. It is also worth noting that some recent mechanical search system could, in principle, succeed in such a scenario~\cite{ICRA2019search}, but not in the ones discussed next.

\noindent
\textbf{Scenario 2: Multi-obstacle and clutter:}
Secondly, we tested \name\ in a scenario that has both large obstacles and clutter (as shown in Fig.~\ref{fig:res-qual-fig}(b)). We placed two boxes in the workspace, thus occluding two regions from camera.  We placed 5 items in each box, and one tagged item in one of the boxes. Similar to the above scenario, \name\ was successful in exploring the environment using RF-guided optimization, maneuvering toward to the target object, and successfully grasping it. We tested \name\ in this scenario for 3 times. The average travelled distance was 4.13 with standard deviation of 1.91. \name\ was successful across all 3 trials. It is worth noting that, to the best of our knowledge, this is a novel task that existing robotic systems cannot perform.

\noindent
\textbf{Scenario 3: Multiple piles and multiple target objects:} Our final scenario of interest is one that involves mechanical search for \textit{all} objects belonging to a semantic class. One such scenario is shown in Fig.~\ref{fig:res-qual-fig}(c), where the robot needs to extract all RFID-tagged items that have a certain semantic feature (e.g., all green blocks)\textcolor{red}{(We are not doing grasping similar blocks in the video)} and sort them into a separate bin. Since the RF perception module can read all RFID-tagged items in the environments, it can identify and locate them, and determine which of these it needs to grasp. Subsequently, the robot performs mechanical search for each of the items, picks them up, and drops them in the white bin to the bottom right. \name\ succeeded in the task and declared task completion once it localized all target objects to the final bin. The travelled  distance for this scenario was  16.18m. 
\fa{Failure modes? Limitations}


% \begin{figure*}
% 	\centering
% 	\begin{tabular}{ccc}
% %	\begin{minipage}{.63\columnwidth}
% %		\centering
% 		\epsfig{file=res_1p_1.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_2.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_3.jpeg,width=0.3\textwidth}
% 		\\
		
% 		\footnotesize{(a) Localization through obstacles}
% 		&
% 		\footnotesize{(b) Moving directly  above  the  item.  }
% 		&
% 		\footnotesize{(c) Decluttering} \vspace{0.2cm}
% 		\\
		
% 		\epsfig{file=res_1p_4.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_5.jpeg,width=0.3\textwidth}
% 		&
% 		\epsfig{file=res_1p_6.jpeg,width=0.3\textwidth}
% 		\\
		
% 		\footnotesize{(d) Moving  directly  above  the  item.  }
% 		&
% 		\footnotesize{(e) Grasping attempt}
% 		&
% 		\footnotesize{(f)Grasp success confirmation}
% 		\\ 
% 		&
% 		&
% 		\footnotesize{by RFID location change}
% 		\\ 
% \end{tabular}
% \caption {\textbf{Scenario 1: Clutter} a) In the initial state, an RFID tagged item is occluded under clutter. There is no line-of-sight to the item from camera or antennas. b) The robot moves directly above the item. c) The robot grasps an item. However, since the RFID location doesn't change, it concludes that the recently grasped item is a clutter.  d)  The robot returns directly above the item to try again. e) \name\ attempts grasping another item. f) The robot confirms that it grasped the item of interest because the RFID location changes accordingly.}
% \label{fig:res-qual-fig}
% \end{figure*}
% \vspace{0.3cm}
% % \begin{figure*}
% % 	\centering
% % 	\begin{tabular}{cccc}
% % %	\begin{minipage}{.63\columnwidth}
% % %		\centering
% % 		\epsfig{file=res_1p_1.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_2.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_3.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_4.jpeg,width=0.23\textwidth}
% % 		\\
		
% % 		\footnotesize{(a)}
% % 		&
% % 		\footnotesize{(b) }
% % 		&
% % 		\footnotesize{(c)}  
% % 		& 
% % 		\footnotesize{(d)} 
% % 		\\
		
% % 		\epsfig{file=res_3_5.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_6.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_7.jpeg,width=0.23\textwidth}
% % 		&
% % 		\epsfig{file=res_3_8.jpeg,width=0.23\textwidth}
% % 		\\
		
% % 		\footnotesize{(e)}
% % 		&
% % 		\footnotesize{(f)}
% % 		&
% % 		\footnotesize{(g)}
% % 		&
% % 	    \footnotesize{(h)}
% % 		\\
% % \end{tabular}
% % \caption {\textbf{Multi-Obstacle \& Clutter Scenario. } a) In the initial state, an RFID tagged item is occluded under clutter inside one of the boxes. There is no line-of-sight to the item from camera or antennas. b) The robot moves directly above the item. d) The robot grasps an item. However, since the RFID location doesn't change, it concludes that the recently grasped item is a clutter. e) The robot removes more clutter.  
% %  f) Robot tries grasping the tagged item. However, it misses the item as the box slippes in the process and changes the item location. e) \name\ updates the tagged item location, and tries grasping again. g) The robot confirms that it grasped the item of interest because the RFID location changes with accordingly.}
% % \label{fig:res-qual-fig}
% % \end{figure*}



==> results-4.tex <==
\begin{figure}[t]
\begin{tikzpicture}
\begin{axis}[ymin=0, ymax=5, height=4cm, width=0.45\textwidth, 
  ytick={0,1,...,5}, ytick align=outside, ytick pos=left,
  xtick={0,1,...,6}, xtick align=outside, xtick pos=left,
  xlabel= \footnotesize{\# occlusions},
  ylabel={\footnotesize{Traveled Distance [m]}},
  legend pos=north west,
  legend style={draw=none},
  yticklabel style={font=\small},
  xticklabel style={font=\small}]
\addplot+[
  blue, mark options={blue, scale=0.75}, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.95,    0.38
    1,  1.80,    0.68
    2,  2.43,    0.77
    3,  3.2,    1.57
    4,  3.42,    1.1
    5,  2.9,    1.05
    
};
\addplot+[
  red, mark options={red, scale=0.75},
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {
    x,  y,       error
    0,  0.96,    0.44
    1,  1.42,    0.22
    2,  1.40,    0.26
    3,  1.8,     0.37
    4,  1.82,    0.54
    5,  1.57,    0.45
    
};
\addlegendentry{\footnotesize{Baseline}}
\addlegendentry{\footnotesize{\name}}
\end{axis}
\end{tikzpicture}
\vspace{-0.05in}
\caption{\textbf{Traveled Distance.} The figure plots the average traveled distance of the gripper's tip for baseline (blue) and \name\ (red) in successful trials across 0-5 occlusion. Error bars represent the standard deviation.}
\label{fig:travel}
\vspace{-0.15in}
\end{figure}

\begin{figure*}[thp]
	\centering
	\begin{tabular}{ccc}
%	\begin{minipage}{.63\columnwidth}
%		\centering
		\epsfig{file=res1.jpeg,width=0.29\textwidth}
		&
		\epsfig{file=res2.jpeg,width=0.29\textwidth}
		&
		\epsfig{file=res3.jpeg,width=0.29\textwidth}
		\\
		
		\footnotesize{(a) Under Soft Cover}
		&
		\footnotesize{(b) Multi-obstacle and Multi-pile }
		&
		\footnotesize{(c) Prioritized Sorting} \vspace{0.2cm}
		\\
\end{tabular}
\vspace{-0.1in}
\caption{\textbf{Generalized Mechanical Search.} We demonatrate \name\ in 3 challenging tasks which the baseline cannot perform.} %(a) The first is grasping from under clutter. (b) The second is grasping in the presence of multiple piles and obstacles. (c) The third is a prioritized sorting task.}
\label{fig:res-qual-fig}
\vspace{-0.15in}
\end{figure*}

\vspace{-0.08in}
\section{Results}
\vspace{-0.1in}
\subsection{Performance Results}
\vspace{-0.05in}


We evaluated \name\ and the baseline quantitatively by varying the number of large occlusions ($M$) and distractor objects ($N$). Each large occlusion hides a different region of the workspace from the camera. We also varied the initial position of the robot across experimental trials, but ensured the baseline and \name\ shared the same initial position.

\noindent
\textbf{(a) Traveled Distance:} 
We recorded the robot's end-effector position and computed its traveled distance for \name\ and the baseline. We tested six scenarios with 0-5 occluded regions (each with 1-15 distractor objects) and ran 10 trials per system and scenario. 
We placed the robot in an initial pose where the wrist-mounted camera partially sees a frontier, i.e., with one or more occluded regions in its initial observation. As the robot explored the environment to minimize its cost function, it found other frontiers and occluded regions. 

Fig.~\ref{fig:travel} plots the average traveled distance of the gripper for both \name\ and the baseline. For all except $M=0$, our results show that \name\ travels shorter distances (by up to 50\%); moreover, \name\ significantly outperforms the baseline as the number of occlusions increases. This result is expected because \name\ is guided by the RFID's location (in the cost function), which reduces the traveled distance and the time spent on exploring the environment searching for the tagged item in comparison to the baseline. Note that the average traveled distance plateaus beyond four occlusions because the workspace of the robot is limited by its arm size and mobility (and all occluded regions are within that workspace). This result demonstrates the value of \name's first core component (RF-visual servoing) in enabling efficient exploration and trajectory optimization.

\noindent
\textbf{(b) Task Completion Rate:}
Next, we evaluated \name’s completion rate (defined in~\ref{sec:eval}) across the same experiments described above. %A task is considered complete if the robot successfully maneuvers toward the target object and picks it up.  %For a trial to be considered successful, the system should find a line of sight to the item within 5 meters of traveled distance in the exploration phase, and a successful grasp should be completed within 10 grasping attempts. 
%We use the same experimental trials performed above experiments are the same as ones carried out for average traveled distance.
%
Table~\ref{tabCompletion} shows the results. \name\ was able to complete the task in 60 out of 60 trials, while the baseline was unable to complete the task in 7 out of 60 trials. The baseline completion rate decreases as the number of occlusions and complexity in experiments increases.

\begin{table}[h]
\vspace{-0.1in}
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lbababa}

& \multicolumn{6}{c}{\textbf{Scenario (M=\#occlusions, N=\#objects)}}\\
\cmidrule{2-7}
\textbf{System}& M=0 N=5 & M=1 N=1 & M=2 N=5 & M=3 N=10 & M=4 N=13 & M=5 N=15\\
\hline
Baseline &    $10_{/10}$  & $10_{/10}$ & $10_{/10}$  & $8_{/10}$  & $7_{/10}$  & $8_{/10}$  \\
RF-Grasp &    $10_{/10}$  &   $10_{/10}$   &  $10_{/10}$ &    $10_{/10}$ &  $10_{/10}$  &  $10_{/10}$ \\
\end{tabular}
\caption{\textbf{Completion Rate.} In each scenario, M denotes number of occlusions, N number of blocks. Results are reported as the number of successfully completed trials out of the total number of experimental trials.}
\label{tabCompletion}
\end{table}
\vspace{-0.05in}
\subsection{Generalized Mechanical Search}
\vspace{-0.05in}
Next, we show that \name\ can successfully perform mechanical search in challenging scenarios where the state-of-the-art baseline is unsuccessful. We consider three such scenarios, shown in Fig.~\ref{fig:res-qual-fig} (see video for demonstration).

\noindent
\textbf{Scenario 1: Under Soft Cover:} We consider scenarios with more than 20 distractor objects along with the target item, covered with soft package filling sheets (Fig.~\ref{fig:res-qual-fig}(a)). There is no line-of-sight from the wrist-mounted camera or antennas to the item. \name\ localizes the RFID and moves directly above the covered item. 
%The camera RGB-D data is fed to the grasping network and an action point and gripper orientation is chosen according to estimated Q-values. 
Because the target is occluded, the robot's attention mechanism biases it to first pick up the cover, but realizes it hasn't picked the target object since the RFID's location has not changed. It puts the cover aside and makes a second grasping attempt. This time, the tracked RFID location changes with the robot's end-effector, and \name\ confirms it has grasped the requested item. We tested \name\ in this scenario 5 times. The average travelled distance was 2.68m with standard deviation of 0.98. \name\ was successful in all 5 trials.

In contrast to \name, our baseline is incapable of successfully completing this task because the green-tagged object would remain fully-occluded; thus, it can neither complete its exploration nor efficiently grasp the target object. It is also worth noting that some recent mechanical search system could, in principle, succeed in such a scenario~\cite{ICRA2019search}.

\noindent
\textbf{Scenario 2: Multiple piles and multiple obstacles:}
Next, we tested \name\ in a scenario with large obstacles and a cover (Fig.~\ref{fig:res-qual-fig}(b)). We used two boxes, occluding two regions from camera.  We placed 5 items in each box, and a tagged item in one of them. Similar to the above scenario, \name\ was successful in exploring the environment using RF-guided optimization, maneuvering toward the target, removing the cover, and successfully grasping. We tested \name\ in this scenario 3 times. The average travelled distance was 4.13 with standard deviation of 1.91. \name\ was successful across all 3 trials. To the best of our knowledge, this is a novel task that existing robotic systems cannot perform.

\noindent
\textbf{Scenario 3: Multiple piles and multiple target objects:} Our final scenario is involves mechanical search for \textit{all} objects belonging to a semantic class. An example is shown in Fig.~\ref{fig:res-qual-fig}(c), where the robot needs to extract all RFID-tagged items that have a certain feature (e.g., the same dimensions) and sort them into a separate bin. The RF perception module reads and locates all RFID-tagged items, and determines which it needs to grasp. Subsequently, the robot performs mechanical search for each of the items, picks them up, and drops them in the white bin to the bottom right. \name\ succeeded and declared task completion once it localized all target objects to the final bin. The total travelled distance (for 3 objects) was 16.18m. To the best of our knowledge, this is also a novel task that existing systems cannot perform.

==> servoing-1.tex <==
\section{Radio Visual Servoing}\label{sec:servoing}

Things to cover: RF Positioning, Gaussian Belief Space Planning,
Biasing the Planner (weights), probabilistic constraint on trajectory
and initial/final position, Active Exploration, Trajectory
Optimization (function)


In this section, we describe how \name$_$ explores the environment to enable grasping occluded objects. We assume the environment is static, and the robot base is stationary. The process consists of several step as depicted in Figure \ref{fig:diagram}. The camera continuously updates the TSDF (Truncated Signed Distance Function) volume, and the RFID localization system constantly gets the coordinates of the targeted object. Occlusion frontiers and occluded regions are extracted from the TSDF volume, and occluded regions are modeled by 3D Gaussian distributions. \name$_$ performs radio-visual trajectory optimization. It assesses the amount of uncertainty in the occluded region of interest after executing the trajectory. If the uncertainty is below a threshold, system moves to grasping phase. Otherwise, the system continues to trajectory optimization and exploration.

\begin{figure}[H]
	\begin{center}
		\includegraphics[width =\textwidth/2]{Grasping_Paper/figures/diagram.001.jpeg}
		\caption{\textbf{Exploration system overview.}}
		\label{fig:diagram}
	\end{center}
\end{figure}


\subsection{Parameterizing the Uncertainties}
During the exploration, \name$_$ maintains a map of the environment using a 3D voxel grid which is stored in a TSDF volume. The system assumes the obstacles and items are placed on a large table top, and removes the largest plane (table top) from its model of the environment. The occlusion frontiers are extracted by clustering and fitting oriented bounding boxes in the rest of the surface point cloud. The inverse point cloud is computed from the unobserved voxels in TSDF volume, and is truncated against the camera frustum to get the occluded regions point cloud by each frontier. Lastly, M Gaussians distributions are fit on M largest occluded regions where M is a user-defined parameter. The mean and covariance of the m-th Gaussian are denoted by $(\mathbf{x}^{m},\mathbf{\Sigma}_0^{m})$ at the initial time. The environment is assumed to be static and hence the means remain the same over time; however, the covariances $\mathbf{\Sigma}_t^{m}$ get updated as system explores the environment.  

\subsection{RF-Guided Objective Function}

\name\ aims to minimize its trajectory (control signal) while at the same time minimizing its uncertainty of the surrounding environment. Mathematically, the overall cost at time $t$ can be expressed as:
{
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\begin{align}
c_t (\mathbf{x}_t^{R}, \Sigma_t^{1:M},\mathbf{u}_t) &= \alpha||\mathbf{u}_t||_2^2+\sum\limits_{m=1}^M\beta_t^m\text{tr}(\Sigma_t^m) %\\%[0.03in]
%c_T (\mathbf{x}_T^{R}, \Sigma_T^{1:M},\mathbf{u}_T) &= \sum\limits_{m=1}^M\beta_T^m\tr(\Sigma_T^m)
\end{align}
}

\noindent
where $\mathbf{u}$ is the control signal applied to the joint state $\mathbf{x}^{R}$. $\alpha$ and $\beta_t^m$ are scalar weighting parameters. 
In order to bias the controller to explore the occluded region surrounding the RFID, we set the $\beta_t^m$ of the corresponding occluded region to be significantly larger than others. Moreover, to give the robot more flexibility at the beginning to explore, we start with a lower $\beta_t^m$ and increase it over time. 

Given the above cost function, we can now formulate the trajectory optimization problem as a minimization function over the planning horizon~\cite{BerkeleyGraspOcclusion} and solve it using standard optimization solvers.


\subsection{System and Belief Dynamics}

The system dynamics of the 6 DoF manipulator can be represented as $\mathbf{x}_{t+1}^{R}=\mathbf{f}(\mathbf{x}_{t}^{R},\mathbf{u}_{t},\mathbf{q}_t)$ where $\mathbf{q}_t$ is the the dynamics noise. The observation is modeled as,
$$\mathbf{z}_t=\mathbf{h}(\mathbf{x}_t^R,\mathbf{x}_t^m,\mathbf{r}_t) =\left[\begin{array}{c}
\mathbf{x}_t^R \\
\mathbf{x}_t^m - \text{IK}(\mathbf{x}_R^m)\end{array}\right]+\mathbf{r}_t$$ where $\mathbf{z}_t$ denotes observation, $\mathbf{r}_t$ is measurement noise and IK is inverse-kinematic function. For belief dynamics, \name\ follows standard Gaussian belief space planning techniques that propagates belief states using an Extended Kalman Filter (EKF) \cite{XX}. The EKF update equations for each occluded region are:
\begin{equation}
\Sigma_{t+1} = (I- K_t H_t)\Sigma_{t+1}^{-}\\
\end{equation}
\begin{equation}
K_t=\Sigma_{t+1}^{-} H_t^T \Delta_t [\Delta_t H_t \Sigma_{t+1}^{-} H_t^T \Delta_t + R_t R_t^T ]^{-1}\Delta_t
\end{equation}
\begin{equation}
\Sigma_{t+1}^{-} = A_t \Sigma_t A_t^T + Q_tQ_t^T\\
\end{equation}
\begin{equation}
A_t = \left[\begin{array}{cc}
                \frac{\partial\mathbf{f} }{\partial\mathbf{x}^R} (\mathbf{x}_{t}^{R},\mathbf{u}_{t},0) & 0\\
                0 & I\end{array}\right]\\
\label{eq:At}
\end{equation}
\begin{equation}             
Q_t =\left[\begin{array}{cc}
            \frac{\partial\mathbf{f} }{\partial\mathbf{q}} (\mathbf{x}_{t}^{R},\mathbf{u}_{t},0) & 0\\
            0 & 0\end{array}\right]\\
\label{eq:qt}
 \end{equation}
\begin{equation}           
H_t =\left[ \frac{\partial\mathbf{h}}{\partial\mathbf{x}^{R}}(\mathbf{x}_{t+1}^R,\mathbf{x}^m,0),   \frac{\partial\mathbf{h}}{\partial\mathbf{x}^{m}}(\mathbf{x}_{t+1}^R,\mathbf{x}^m,0)\right]\\
% \label{eq:sig}
\end{equation}
\begin{equation}
R_t=\frac{\partial\mathbf{h}}{\partial\mathbf{r}}(\mathbf{x}_{t+1}^R,\mathbf{x}_t^m,0) , \Delta_t = \left[\begin{array}{cc}
                I & 0\\
                0 & \Delta_t^m\end{array}\right]\\
 \end{equation}
\begin{equation}             
\Sigma_0 = \left[\begin{array}{cc}
                \Sigma_0^R & 0\\
                0 & \Sigma_0^m \end{array}\right] 
                \label{eq:sig}
\end{equation}

In Eq.\ref{eq:sig} the initial covariance are created by diagonally concatenating the robot joint state uncertainty with the
occluded region covariances. Eq. \ref{eq:At} and \ref{eq:qt} are changed because the environment is assumed to be static\cite{BerkeleyGraspOcclusion}. $H_t$ and $R_t$ are approximated numerically.\textcolor{red}{(double check)}

\subsection{Sensing Domain Discontinuity}
In \name\ the potential unobservability due to occlusions and vision sensor field-of-view is taken care of by $\Delta_t$ in the modified EKF update. $\Delta_t^m$ can be defined as:
\begin{equation}
\Delta_t^m =\left[\begin{array}{ccc}
                \varphi_{t}^m & 0 & 0\\
                0 & \varphi_{t}^m & 0\\
                0 & 0 & \varphi_{t}^m\end{array}\right]
\end{equation}
where $\varphi_{t}^m $ is 1 where $x^m$ is observable and is 0 otherwise. However, such a step function is not differentiable, so it is approximated by 
\begin{equation}
    \varphi_t^m = \frac{1}{1+\exp(-\alpha(\text{sd}(\mathbf{x}_t^{R},\mathbf{x}^{m},\prod_t)+\rho(\mathbf{x}^{m})))}
\end{equation}
where $\alpha$ is the slope of the sigmoidal approximation, $\prod_t$ denotes the frontiers, and $\rho(\mathbf{x}^{m})$ is the distance in image plane of $\mathbf{x}^{m}$ to the principal axis of camera\cite{in brekely paper}. Lastly, $\text{sd}(\mathbf{x}_t^{R},\mathbf{x}^{m},\prod_t)$ is the signed-distance from $\mathbf{x}^{m}$ to camera’s frustum.
The camrera field-of-view is represented as a set of convex regions by truncating the view frustum against the frontiers. The magnitude of the signed-distance is $\mathbf{x}^{m}$'s distance to the nearest convex region border. Its sign is positive if $\mathbf{x}^{m}$ is outside a convex regions and negative otherwise. 

==> servoing-2.tex <==
\section{RF-Visual Servoing}\label{sec:servoing}

%Things to cover: RF Positioning, Gaussian Belief Space Planning,
%Biasing the Planner (weights), probabilistic constraint on trajectory
%and initial/final position, Active Exploration, Trajectory
%Optimization (function)

\fa{The techniques are finalized but the writing needs significant smoothing/re-org.}

In this section, we describe how \name\ explores the environment to enable grasping occluded objects. We assume the environment is static, and the robot base is stationary. We frame the servoing problem as a Partially Observable Markov Decision Process (POMDP) defined by a 7-tuple $\mathcal{(S,A,T,R,}\Omega\mathcal{,O,\gamma)}$:
\begin{itemize}
    \item \textbf{States $\mathcal{(S)}$:} The state of the environment consists of obstacles and occlusions, objects, clutters, and robot joint state. 
    \item \textbf{Actions $\mathcal{(A)}$:} The  control  signal, $\mathbf{u}_t$,  applies  to  the  joint  state $\mathbf{x}_t^R$ and changes the robot pose.
    \item \textbf{Transition Function $\mathcal{(T)}$:} When objects and the robot come to rest after action execution, the new state is determined. The transition model is $T(s_{t+1} | s_t , a_t )$.
    \item \textbf{Reward $\mathcal{(R)}$:} Lets $\Lambda_t$ denote the uncertainty in the environment at time $t$. Reward function  increases as uncertainties decrease in the environment. It can be noted by $r_t = \Lambda_t - \Lambda_{t+1}$. In this paper, we do not directly optimize this function.  
    \item \textbf{Observations $(\Omega)$:} Joint state $\mathbf{x}_t^R$, RFID tagged item location $\mathbf{p}_t$, and RGB-D data from wrist-mounted camera are observed by \name.
    \item \textbf{Observation Model $\mathcal{(O)}$:} The observation $o_t\in\Omega$ at time $t$ depend on the state of the environment and the action taken with probability of $\mathcal{O}(o_t|s_{t+1},a_t)$. 
    \item \textbf{Discount Factor $\mathcal{(\gamma)}$:} It determines how much distant reward are taken into consideration.
\end{itemize}
\noindent
Given the problem definition, the goals is to choose a sequence of actions to minimize the uncertainties of the environment around the RFID tagged item using the observations.  

The process consists of several step as depicted in Figure \ref{fig:exploration}. The camera continuously updates the TSDF (Truncated Signed Distance Function) volume \cite{XX}, and the RFID localization system constantly gets the coordinates of the targeted object. In the second step, occlusion frontiers and occluded regions are extracted from the TSDF volume, and occluded regions are modeled by 3D Gaussian distributions. It assesses the amount of uncertainty in the occluded region of interest after executing the trajectory. If the uncertainty is below a threshold, or there is a line of sight to the tagged item, system moves to grasping phase. Otherwise, the system continues to trajectory optimization and exploration.

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width =0.45\textwidth]{Grasping_Paper/figures/exploration.jpeg}
% 		\caption{\textbf{Exploration System Overview.} \name\ creates a 3D model of the environment using the RGB-D date stream from camera. Then, it extracts the occluded regions and models them with a 3D Gaussian distribution. If a exploration stopping criterion is met, the system moves to grasping phase. Otherwise, \name\ optimizes trajectory using RFID location and executes it. The process repeats again. }
% 		\label{fig:exploration}
% 	\end{center}
% \end{figure}


\subsection{Parameterizing the Uncertainties}
During the exploration, \name\ maintains a map of the environment using a 3D voxel grid which is stored in a TSDF volume. After removing table top, the occlusion frontiers are extracted by clustering. M Gaussian distributions are fitted on M largest occluded regions where M is a user-defined parameter. The mean and covariance of the m-th Gaussian are denoted by $(\mathbf{x}^{m},\mathbf{\Sigma}_0^{m})$ at the initial time. The environment is assumed to be static and hence the means remain the same over time; however, the covariances $\mathbf{\Sigma}_t^{m}$ get updated as the system explores the environment.  

\subsection{RF-Guided Objective Function}

\name\ aims to minimize its trajectory (control signal) while at the same time minimizing its uncertainty of the surrounding environment. Mathematically, the overall cost at time $t$ can be expressed as:
{
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\begin{align}
c_t (\mathbf{x}_t^{R}, \Sigma_t^{1:M},\mathbf{u}_t) &= \alpha||\mathbf{u}_t||_2^2+\sum\limits_{m=1}^M\beta_t^m\text{tr}(\Sigma_t^m) %\\%[0.03in]
%c_T (\mathbf{x}_T^{R}, \Sigma_T^{1:M},\mathbf{u}_T) &= \sum\limits_{m=1}^M\beta_T^m\tr(\Sigma_T^m)
\end{align}
}

\noindent
where $\mathbf{u}$ is the control signal applied to the joint state $\mathbf{x}^{R}$. $\alpha$ and $\beta_t^m$ are scalar weighting parameters. 
In order to bias the controller to explore the occluded region surrounding the RFID, we set the $\beta_t^m$ of the corresponding occluded region to be significantly larger than others. Moreover, to give the robot more flexibility at the beginning to explore, we start with a lower $\beta_t^m$ and increase it over time. 

Given the above cost function, we can now formulate the trajectory optimization problem as a minimization function over the planning horizon~\cite{BerkeleyGraspOcclusion} and solve it using standard optimization solvers.

\begin{figure}[t] \vspace{-0.15in}
\centering
\epsfig{file=occluded-regions.png,width=2.3in}
\captionof{figure}{\footnotesize \textbf{RF-Visual Servoing.} \name\ encodes occluded regions as a mixture of Gaussians and biases its active exploration toward the region that has the RFID-tagged item of interest.}
\label{fig:MoG}
%\vspace{-0.1in}
\end{figure}


\subsection{RF-Guided Initial Trajectory}
Since \name\ is capable of accurately localizing the RFID-tagged object position, an initial trajectory toward the item of interest can be created. This RF-guided initial trajectory is used as initial point for the optimization solver to aid the exploration.

\subsection{System and Belief Dynamics}

The system dynamics of the 6 DoF manipulator can be represented as $\mathbf{x}_{t+1}^{R}=\mathbf{f}(\mathbf{x}_{t}^{R},\mathbf{u}_{t},\mathbf{q}_t)$ where $\mathbf{q}_t$ is the the dynamics noise. The observation is modeled as,
$$\mathbf{z}_t=\mathbf{h}(\mathbf{x}_t^R,\mathbf{x}_t^m,\mathbf{r}_t) =\left[\begin{array}{c}
\mathbf{x}_t^R \\
\mathbf{x}_t^m - \text{IK}(\mathbf{x}_R^m)\end{array}\right]+\mathbf{r}_t$$ where $\mathbf{z}_t$ denotes observation, $\mathbf{r}_t$ is measurement noise and IK is inverse-kinematic function. For belief dynamics, \name\ follows standard Gaussian belief space planning techniques that propagates belief states using an Extended Kalman Filter (EKF) \cite{XX}. 
% The EKF update equations for each occluded region are:
% \begin{equation}
% \Sigma_{t+1} = (I- K_t H_t)\Sigma_{t+1}^{-}\\
% \end{equation}
% \begin{equation}
% K_t=\Sigma_{t+1}^{-} H_t^T \Delta_t [\Delta_t H_t \Sigma_{t+1}^{-} H_t^T \Delta_t + R_t R_t^T ]^{-1}\Delta_t
% \end{equation}
% \begin{equation}
% \Sigma_{t+1}^{-} = A_t \Sigma_t A_t^T + Q_tQ_t^T\\
% \end{equation}
% \begin{equation}
% A_t = \left[\begin{array}{cc}
%                 \frac{\partial\mathbf{f} }{\partial\mathbf{x}^R} (\mathbf{x}_{t}^{R},\mathbf{u}_{t},0) & 0\\
%                 0 & I\end{array}\right]\\
% \label{eq:At}
% \end{equation}
% \begin{equation}             
% Q_t =\left[\begin{array}{cc}
%             \frac{\partial\mathbf{f} }{\partial\mathbf{q}} (\mathbf{x}_{t}^{R},\mathbf{u}_{t},0) & 0\\
%             0 & 0\end{array}\right]\\
% \label{eq:qt}
%  \end{equation}
% \begin{equation}           
% H_t =\left[ \frac{\partial\mathbf{h}}{\partial\mathbf{x}^{R}}(\mathbf{x}_{t+1}^R,\mathbf{x}^m,0),   \frac{\partial\mathbf{h}}{\partial\mathbf{x}^{m}}(\mathbf{x}_{t+1}^R,\mathbf{x}^m,0)\right]\\
% % \label{eq:sig}
% \end{equation}
% \begin{equation}
% R_t=\frac{\partial\mathbf{h}}{\partial\mathbf{r}}(\mathbf{x}_{t+1}^R,\mathbf{x}_t^m,0) , \Delta_t = \left[\begin{array}{cc}
%                 I & 0\\
%                 0 & \Delta_t^m\end{array}\right]\\
%  \end{equation}
% \begin{equation}             
% \Sigma_0 = \left[\begin{array}{cc}
%                 \Sigma_0^R & 0\\
%                 0 & \Sigma_0^m \end{array}\right] 
%                 \label{eq:sig}
% \end{equation}

% In Eq.\ref{eq:sig} the initial covariance are created by diagonally concatenating the robot joint state uncertainty with the
% occluded region covariances. Eq. \ref{eq:At} and \ref{eq:qt} are changed because the environment is assumed to be static\cite{BerkeleyGraspOcclusion}. $H_t$ and $R_t$ are approximated numerically.\textcolor{red}{(double check)}

% \subsection{Sensing Domain Discontinuity}
% In \name\ the potential unobservability due to occlusions and vision sensor field-of-view is taken care of by $\Delta_t$ in the modified EKF update. $\Delta_t^m$ can be defined as:
% \begin{equation}
% \Delta_t^m =\left[\begin{array}{ccc}
%                 \varphi_{t}^m & 0 & 0\\
%                 0 & \varphi_{t}^m & 0\\
%                 0 & 0 & \varphi_{t}^m\end{array}\right]
% \end{equation}
% where $\varphi_{t}^m $ is 1 where $x^m$ is observable and is 0 otherwise. However, such a step function is not differentiable, so it is approximated by 
% \begin{equation}
%     \varphi_t^m = \frac{1}{1+\exp(-\alpha(\text{sd}(\mathbf{x}_t^{R},\mathbf{x}^{m},\prod_t)+\rho(\mathbf{x}^{m})))}
% \end{equation}
% where $\alpha$ is the slope of the sigmoidal approximation, $\prod_t$ denotes the frontiers, and $\rho(\mathbf{x}^{m})$ is the distance in image plane of $\mathbf{x}^{m}$ to the principal axis of camera\cite{in brekely paper}. Lastly, $\text{sd}(\mathbf{x}_t^{R},\mathbf{x}^{m},\prod_t)$ is the signed-distance from $\mathbf{x}^{m}$ to camera’s frustum.
% The camrera field-of-view is represented as a set of convex regions by truncating the view frustum against the frontiers. The magnitude of the signed-distance is $\mathbf{x}^{m}$'s distance to the nearest convex region border. Its sign is positive if $\mathbf{x}^{m}$ is outside a convex regions and negative otherwise. 


\subsection{Exploration Termination Criteria}
The system stops exploration and moves to grasping phase as soon as one of the following criteria is met.

a) Insignificant covariance matrix trace: The system assesses the covariance of the  3D Gaussian associated with the tagged item which is denoted by $\Sigma^1$. The exploration is halted if $$\text{trace}(\Sigma^1) < 0.005$$ as the uncertainty around the item is very small. 

b) Line of Sight to the tagged item vicinity: Since the exact location of RFID tag is known, it can be easily inferred which voxels in the TSDF volume are near the RFID tag. We defined item vicinity,$\mathbf{\nu}$, to be a $5\text{cm}\times5\text{cm}\times5\text{cm}$ cube centered at RFID location. $\forall \upsilon \in \mathbf{\nu}: \digamma(\upsilon) = 1 \iff$


The system presumes there is a line of sight to item when it can see more than 10\% of voxels in the cube.

When the environment is cluttered and the item is under a cover, the trace of covariance won't be below threshold since the cover and other items hide the table top. However, enough voxels in the vicinity of the item will be visible to the camera that the second criterion is met and system will move to grasping phase in the right time.

==> servoing-3.tex <==
\section{RF-Visual Servoing}\label{sec:servoing}

%Things to cover: RF Positioning, Gaussian Belief Space Planning,
%Biasing the Planner (weights), probabilistic constraint on trajectory
%and initial/final position, Active Exploration, Trajectory
%Optimization (function)

Given the RFID’s location and an RGB-D image, \name\ needs to maneuver the robotic arm toward the target object. A key difficulty in this process is that the environment is not known a priori and the direct path may be occluded by obstacles. Thus, RF-Grasp needs to actively explore the environment as it tries to determine the optimal path around obstacles toward the target object. 

In this section, we describe how \name\ formulates this as a POMDP and extends past work in Gaussian Belief Space Planning (GBSP) to enable efficient active exploration while minimizing the trajectory toward the object of interest.

\subsection{Problem Definition}
We frame the servoing problem as a Partially Observable Markov Decision Process (POMDP) defined by a 7-tuple $\mathcal{(S,A,T,R,}\Omega\mathcal{,O,\gamma)}$:
\begin{itemize}
    \item \textbf{States $\mathcal{(S)}$:} The state of the environment consists of obstacles and occlusions, objects, %clutters, 
    and robot joint state. 
    \item \textbf{Actions $\mathcal{(A)}$:} The  control  signal, $\mathbf{u}_t$,  applies  to  the  joint  state $\mathbf{x}_t^R$ and changes the robot pose.
    \item \textbf{Transition Function $\mathcal{(T)}$:} When objects and the robot come to rest after action execution, the new state is determined. The transition model is $T(s_{t+1} | s_t , a_t )$.
    \item \textbf{Reward $\mathcal{(R)}$:} Let $\Lambda_t$ denote the uncertainty in the environment at time $t$. The reward function increases as uncertainties decrease in the environment. It can be noted as $r_t = \Lambda_t - \Lambda_{t+1}$. In this paper, we do not directly optimize this function.  
    \item \textbf{Observations $(\Omega)$:} Joint state $\mathbf{x}_t^R$, RFID-tagged item's location $\mathbf{p}_t$, and RGB-D data from wrist-mounted camera are observed by \name.
    \item \textbf{Observation Model $\mathcal{(O)}$:} The observation $o_t\in\Omega$ at time $t$ depend on the state of the environment and the action taken with probability of $\mathcal{O}(o_t|s_{t+1},a_t)$. 
    \item \textbf{Discount Factor $\mathcal{(\gamma)}$:} It determines how much distant rewards are taken into consideration.
\end{itemize}
\noindent

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width =0.45\textwidth]{Grasping_Paper/figures/exploration.jpeg}
% 		\caption{\textbf{Exploration System Overview.} \name\ creates a 3D model of the environment using the RGB-D date stream from camera. Then, it extracts the occluded regions and models them with a 3D Gaussian distribution. If a exploration stopping criterion is met, the system moves to grasping phase. Otherwise, \name\ optimizes trajectory using RFID location and executes it. The process repeats again. }
% 		\label{fig:exploration}
% 	\end{center}
% \end{figure}


\subsection{Modeling Environmental Uncertainties}
In order to optimize the exploration and navigation process, we need to model the uncertainty of the 3D environment. Similar to past work on GBSP~\cite{BerkeleyGraspOcclusion}, \name\ encodes uncertainty in occluded regions using a mixture of Gaussians. Specifically, each occluded region is modeled as a 3D Gaussian as shown in Fig.~\ref{fig:MoG}. The mean and covariance of the m-th Gaussian are denoted by $(\mathbf{x}^{m},\mathbf{\Sigma}_0^{m})$ at the initial time. The environment is assumed to be static and hence the means remain the same over time; however, the covariances $\mathbf{\Sigma}_t^{m}$ get updated as the system explores the environment.  

\begin{figure}[t] \vspace{-0.15in}
\centering
\epsfig{file=occluded-regions.png,width=2.3in}
\captionof{figure}{\footnotesize \textbf{RF-Visual Servoing.} \name\ encodes occluded regions as a mixture of Gaussians and biases its active exploration toward the region that has the RFID-tagged item of interest.}
\label{fig:MoG}
%\vspace{-0.1in}
\end{figure}

\subsection{RF-Biased Objective Function}

To efficiently maneuver toward the target object, \name\ aims to minimize its trajectory (control signal) while at the same time minimizing its uncertainty of the surrounding environment. Mathematically, the overall cost at time $t$ can be expressed as:
{
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\begin{align}
C_{t=0:T-1} (\mathbf{x}_t^{R}, \Sigma_t^{1:M},\mathbf{u}_t) &= \alpha||\mathbf{u}_t||_2^2+\sum\limits_{m=1}^M\beta_t^m\text{tr}(\Sigma_t^m) \\%[0.03in]
C_T (\mathbf{x}_T^{R}, \Sigma_T^{1:M}) &= \sum\limits_{m=1}^M\beta_T^m\tr(\Sigma_T^m)
\end{align}
}
\noindent
where $\mathbf{u}_t$ is the control signal applied to the joint state $\mathbf{x}_t^{R}$. $\alpha$ and $\beta_t^m$ are scalar weighting parameters. 

In order to bias the controller to explore \textit{the occluded region surrounding the RFID}, we set weighting parameter of its corresponding occluded region, $\beta_t^1$, to be significantly larger than others. Moreover, to give the robot more flexibility at the beginning to explore, we start with a lower $\beta_t^1$ and increase it over time. 

Given the above cost function, we can now formulate the trajectory optimization problem as a minimization function over the planning horizon as follows:
\vspace{-0.1in}
\begin{equation*}
\begin{array}{rccr}
\displaystyle \min_{\mathbf{x}_{0:T}^{R},\mathbf{u}_{0:T-1}} & \multicolumn{3}{l}{\mathbb{E}[C_T (\mathbf{x}_T^{R}, \Sigma_T^{1:M}) + \sum\limits_{t=0}^{T-1} C_t (\mathbf{x}_t^{R}, \Sigma_t^{1:M},\mathbf{u}_t)]} \\
\textrm{s.t.} & \mathbf{x}_{t+1}^{R} =  \mathbf{f}(\mathbf{x}_{t}^{R},\mathbf{u_t},0) & & \\
 & \mathbf{x}_{t}^{R} \in \mathbb{X}_{\text{feasible}}, & & \\
 & \mathbf{u}_{t}^{R} \in \mathbb{U}_{\text{feasible}},  & & \\
 & \mathbf{x}_{0}^{R} =\mathbf{x}_{\text{init}}^{R}& & \\
\end{array}
\end{equation*}
where  $\mathbb{X}_{\text{feasible}}$ and $\mathbb{U}_{\text{feasible}}$ represent the set of feasible joint states and control signals of the robot arm. $\mathbf{x}_{\text{init}}^{R}$ is the initial joint state of the robot. The dynamics model for the robot is given by differentiable and stochastic function as in $\mathbf{x}_{t+1}^{R} = f(\mathbf{x}_{t}^R,\mathbf{u}_t,\mathbf{q}_t), \mathbf{q}_t \sim N(0,I)$ where $q_t$ is the dynamics noise.

\subsection{RF-Guided Trajectory Optimization}
\name's approach for solving the above problem follows prior work in Gaussian Belief Space Planning, including modeling the environment using 3D voxel grid map,\footnote{The grid map is stored in a TSDF (Truncated Signed Distance Function) volume.} extracting frontiers and occluded regions, dealing with discontinuities in the RGB-D observation model, modeling the observation and dynamics using Gaussians, and propagating beliefs using Extended Kalman Filter (EKF). We refer the interested reader to prior work for details~\cite{BerkeleyGraspOcclusion}, and focus below on two unique features of our solution, aside from the RF-biased objective function described above:

\vspace{0.05in}
\noindent
\textbf{(a) RF-based Initial Trajectory.} To aid the optimization solver and enable faster convergence of the above optimization problem, we seed the optimization function with an RF-based initial trajectory. Specifically, since \name\ is capable of accurately localizing the RFID-tagged object, it can seed the optimizer with an initial trajectory toward the item of interest can be created.

\vspace{0.05in}
\noindent
\textbf{(b) Exploration Termination Criteria.}
The system stops exploration and moves to grasping phase as soon as one of the following criteria is met.

a) Insignificant covariance matrix trace: The system assesses the covariance of the  3D Gaussian associated with the tagged item which is denoted by $\Sigma^1$. The exploration is halted if $$\text{trace}(\Sigma^1) < 0.005$$ as the uncertainty around the item is very small. 

b) Line of sight to the tagged item vicinity: Since the exact location of RFID tag is known, it can be easily inferred which voxels in the TSDF volume are near the RFID tag. We defined item vicinity, $\nu$, to be a $5\text{cm}\times5\text{cm}\times5\text{cm}$ cube centered at RFID location. If voxel $\upsilon$ has been seen by camera, $\digamma(\upsilon)=1$; otherwise, $\digamma(\upsilon)=0$. The exploration is halted if $$\frac{\sum_{\upsilon \in \nu} \digamma(\upsilon)}{|\nu|} > 0.1 $$ as there is a line of sight to the item's vicinity.



When the environment is cluttered and the item is under a cover, the trace of covariance won't be below threshold since the cover and other items hide the table top. However, enough voxels in the vicinity of the item will be visible to the camera that the second criterion is met and system will move to grasping phase in the right time.

%Given the problem definition, the goals is to choose a sequence of actions to minimize the uncertainties of the environment around the RFID tagged item using the observations.  

%The process consists of several step as depicted in Figure \ref{fig:exploration}. The camera continuously updates the TSDF (Truncated Signed Distance Function) volume \cite{XX}, and the RFID localization system constantly gets the coordinates of the targeted object. In the second step, occlusion frontiers and occluded regions are extracted from the TSDF volume, and occluded regions are modeled by 3D Gaussian distributions. It assesses the amount of uncertainty in the occluded region of interest after executing the trajectory. If the uncertainty is below a threshold, or there is a line of sight to the tagged item, system moves to grasping phase. Otherwise, the system continues to trajectory optimization and exploration.

==> servoing-4.tex <==
\section{RF-Visual Servoing}\label{sec:servoing}

%Things to cover: RF Positioning, Gaussian Belief Space Planning,
%Biasing the Planner (weights), probabilistic constraint on trajectory
%and initial/final position, Active Exploration, Trajectory
%Optimization (function)

Given the RFID’s location and an RGB-D image, \name\ needs to maneuver the robotic arm toward the target object. A key difficulty in this process is that the environment is not known a priori and the direct path may be occluded by obstacles. Thus, RF-Grasp needs to actively explore the environment as it tries to determine the optimal path around obstacles toward the target object. 

In this section, we describe how \name\ formulates this as a POMDP and extends past work in Gaussian Belief Space Planning (GBSP) to enable efficient active exploration while minimizing the trajectory toward the object of interest.

\subsection{Problem Definition}
We frame the servoing problem as a Partially Observable Markov Decision Process (POMDP) defined by a 7-tuple $\mathcal{(S,A,T,R,}\Omega\mathcal{,O,\gamma)}$ \textcolor{red}{with a horizon of T}:
\begin{itemize}
    \item \textbf{States $\mathcal{(S)}$:} The state of the environment consists of obstacles and occlusions, objects, %clutters, 
    and robot joint state. 
    \item \textbf{Actions $\mathcal{(A)}$:} The  control  signal, $\mathbf{u}_t$,  applies  to  the  joint  state $\mathbf{x}_t^R$ and changes the robot pose.
    \item \textbf{Transition Function $\mathcal{(T)}$:} When objects and the robot come to rest after action execution, the new state is determined. The transition model is $T(s_{t+1} | s_t , a_t )$.
    \item \textbf{Reward $\mathcal{(R)}$:} Let $\Lambda_t$ denote the uncertainty in the environment at time $t$. The reward function increases as uncertainties decrease in the environment. It can be noted as $r_t = \Lambda_t - \Lambda_{t+1}$. In this paper, we do not directly optimize this function.  
    \item \textbf{Observations $(\Omega)$:} Joint state $\mathbf{x}_t^R$, RFID-tagged item's location $\mathbf{p}_t$, and RGB-D data from wrist-mounted camera are observed by \name.
    \item \textbf{Observation Model $\mathcal{(O)}$:} The observation $o_t\in\Omega$ at time $t$ depends on the state of the environment and the action taken with probability of $\mathcal{O}(o_t|s_{t+1},a_t)$. 
    \item \textbf{Discount Factor $\mathcal{(\gamma)}$:} It determines how much distant rewards are taken into consideration.
\end{itemize}
\noindent

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width =0.45\textwidth]{Grasping_Paper/figures/exploration.jpeg}
% 		\caption{\textbf{Exploration System Overview.} \name\ creates a 3D model of the environment using the RGB-D date stream from camera. Then, it extracts the occluded regions and models them with a 3D Gaussian distribution. If a exploration stopping criterion is met, the system moves to grasping phase. Otherwise, \name\ optimizes trajectory using RFID location and executes it. The process repeats again. }
% 		\label{fig:exploration}
% 	\end{center}
% \end{figure}


\subsection{Modeling Environmental Uncertainties}
In order to optimize the exploration and navigation process, we need to model the uncertainty of the 3D environment. Similar to past work on GBSP~\cite{BerkeleyGraspOcclusion}, \name\ encodes uncertainty in occluded regions using a mixture of Gaussians. Specifically, each occluded region is modeled as a 3D Gaussian as shown in Fig.~\ref{fig:MoG}. The mean and covariance of the m-th Gaussian are denoted by $(\mathbf{x}^{m},\mathbf{\Sigma}_0^{m})$ at the initial time. The environment is assumed to be static and hence the means remain the same over time; however, the covariances $\mathbf{\Sigma}_t^{m}$ get updated as the system explores the environment.  

\begin{figure}[t] \vspace{-0.15in}
\centering
\epsfig{file=rviz.jpeg,width=2.5in}
\captionof{figure}{\footnotesize \textbf{RF-Visual Servoing.} \name\ encodes occluded regions as a mixture of Gaussians and biases its active exploration toward the region that has the RFID-tagged item of interest.}
\label{fig:MoG}
%\vspace{-0.1in}
\end{figure}

\subsection{RF-Biased Objective Function}

To efficiently maneuver toward the target object, \name\ aims to minimize its trajectory (control signal) while at the same time minimizing its uncertainty of the surrounding environment. Mathematically, the overall cost at time $t$ can be expressed as:
{
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\begin{align}
C_{t=0:T-1} (\mathbf{x}_t^{R}, \Sigma_t^{1:M},\mathbf{u}_t) &= \alpha||\mathbf{u}_t||_2^2+\sum\limits_{m=1}^M\beta_t^m\text{tr}(\Sigma_t^m) \\%[0.03in]
C_T (\mathbf{x}_T^{R}, \Sigma_T^{1:M}) &= \sum\limits_{m=1}^M\beta_T^m\tr(\Sigma_T^m)
\end{align}
}

\noindent
where $\mathbf{u}_t$ is the control signal applied to the joint state $\mathbf{x}_t^{R}$and $M$ is the total number of occluded regions. \textred{(Is the notation $t=0:T-1$ correct?)} $\alpha$ and $\beta_t^m$ are scalar weighting parameters. 

In order to bias the controller to explore \textit{the occluded region surrounding the RFID}, we set weighting parameter of its corresponding occluded region, $\beta_t^1$, to be significantly larger than others. Moreover, to give the robot more flexibility at the beginning to explore, we start with a lower $\beta_t^1$ and increase it over time. 

Given the above cost function, we can now formulate the trajectory optimization problem as a minimization function over the planning horizon as follows:
\vspace{-0.1in}
\begin{equation}\label{eq:obj1}
\begin{array}{rccr}
\displaystyle \min_{\mathbf{x}_{0:T}^{R},\mathbf{u}_{0:T-1}} & \multicolumn{3}{l}{\mathbb{E}[C_T (\mathbf{x}_T^{R}, \Sigma_T^{1:M}) + \sum\limits_{t=0}^{T-1} C_t (\mathbf{x}_t^{R}, \Sigma_t^{1:M},\mathbf{u}_t)]} \\
\textrm{s.t.} & \mathbf{x}_{t+1}^{R} =  \mathbf{f}(\mathbf{x}_{t}^{R},\mathbf{u_t},0) & & \\
 & \mathbf{x}_{t}^{R} \in \mathbb{X}_{\text{feasible}}, & & \\
 & \mathbf{u}_{t}^{R} \in \mathbb{U}_{\text{feasible}},  & & \\
 & \mathbf{x}_{0}^{R} =\mathbf{x}_{\text{init}}^{R}& & \\
\end{array}
\end{equation}
where  $\mathbb{X}_{\text{feasible}}$ and $\mathbb{U}_{\text{feasible}}$ represent the set of feasible joint states and control signals of the robot arm. $\mathbf{x}_{\text{init}}^{R}$ is the initial joint state of the robot. The dynamics model for the robot is given by differentiable and stochastic function as in $\mathbf{x}_{t+1}^{R} = f(\mathbf{x}_{t}^R,\mathbf{u}_t,\mathbf{q}_t), \mathbf{q}_t \sim N(0,I)$ where $q_t$ is the dynamics noise.

\subsection{RF-Guided Trajectory Optimization}
\name's approach for solving the above problem follows prior work in Gaussian Belief Space Planning, including modeling the environment using 3D voxel grid map,\footnote{The grid map is stored in a TSDF (Truncated Signed Distance Function) volume.} extracting frontiers and occluded regions, dealing with discontinuities in the RGB-D observation model, modeling the observation and dynamics using Gaussians, and propagating beliefs using Extended Kalman Filter (EKF). We refer the interested reader to prior work for details~\cite{BerkeleyGraspOcclusion}, and focus below on two unique features of our solution, aside from the RF-biased objective function described above:

\vspace{0.05in}
\noindent
\textbf{(a) RF-based Initial Trajectory.} To aid the optimization solver and enable faster convergence of the above optimization problem, we seed the optimization function with an RF-based initial trajectory. Specifically, since \name\ is capable of accurately localizing the RFID-tagged object, it can seed the optimizer with an initial trajectory toward the item of interest.

\vspace{0.05in}
\noindent
\textbf{(b) Exploration Termination Criteria.}
The system stops exploration when it determines that there is no major obstacle that the robot needs to maneuver around, and thus it needs to move to the manipulation/grasping phase (described in the next section). In the absence of clutter above the target object, this happens when the robot has a direct line-of-sight to the object~\cite{BerkeleyGraspOcclusion}. However, in the presence of clutter, we need to relax this criterion to scenarios where the robot has a near-line-of-sight to the item of interest so that it might need to declutter the environment before grasping. 

To capture both of these scenarios, we formulate the exploration termination criteria as a function of the uncertainty region around the target object. Such uncertainty is encoded both in the covariance of the 3D Gaussian around the object $\Sigma^1$ and in visibility of the voxels $\upsilon$ in the vicinity of $\nu$ the target object's location $\mathbf{p}$. Mathematically, the termination criteria can be expressed as:
\vspace{-0.05in}
\begin{equation}\label{eq:criterion}
\text{trace}(\Sigma^1) < \rho_{\sigma} \quad \text{or} \quad \frac{\sum_{\upsilon \in \nu} \digamma(\upsilon)}{|\nu(\mathbf{p})|} > \rho_{\upsilon}
\end{equation}

\vspace{-0.05in}
\noindent 
where $\digamma(\upsilon)=1$ if voxel $\upsilon$ has been seen by camera and $\digamma(\upsilon)=0$ otherwise. The first criterion signifies that the uncertainty around the object is smaller than a threshold $\rho_{\sigma}$, or the fraction of the visible region surrounding the RFID is larger than a threshold $\rho_{\upsilon}$.\footnote{In our implementation, $\rho_{\sigma} = 0.005$ and $\rho_{\upsilon}=0.1$, and the vicinity, $\nu(\mathbf{p_t})$, is set to a $5\text{cm}\times5\text{cm}\times5\text{cm}$ cube centered at RFID location. } 

The combination of the above criteria is necessary to deal with the diversity of clutter scenarios. For example, when the environment is cluttered and the item is under a cover, the trace of covariance won't be below threshold since the cover and other items hide the table top. However, enough voxels in the vicinity of the item will be visible to the camera that the second criterion is met and system will move to grasping phase in the right time.

Finally, it is worth noting that \name's active exploration formulation as per Eq.~\ref{eq:obj1} automatically perform collision avoidance. This is because if the camera is too close to a large occlusion, the covariances $\Sigma^m_t$ become larger, thus penalizing the expected cost and biasing the decision trajectory away from the large obstruction.

%Given the problem definition, the goals is to choose a sequence of actions to minimize the uncertainties of the environment around the RFID tagged item using the observations.  

%The process consists of several step as depicted in Figure \ref{fig:exploration}. The camera continuously updates the TSDF (Truncated Signed Distance Function) volume \cite{XX}, and the RFID localization system constantly gets the coordinates of the targeted object. In the second step, occlusion frontiers and occluded regions are extracted from the TSDF volume, and occluded regions are modeled by 3D Gaussian distributions. It assesses the amount of uncertainty in the occluded region of interest after executing the trajectory. If the uncertainty is below a threshold, or there is a line of sight to the tagged item, system moves to grasping phase. Otherwise, the system continues to trajectory optimization and exploration.
